BUGSPHP: A dataset for Automated Program Repair in PHP

Automated Program Repair (APR) improves developer productivity by saving debugging and bug-fixing time. While APR has been extensively explored for C/C++ and Java programs, there is little research on bugs in PHP programs due to the lack of a benchmark PHP bug dataset. This is surprising given that PHP has been one of the most widely used server-side languages for over two decades, being used in a variety of contexts such as e-commerce, social networking, and content management. This paper presents a benchmark dataset of PHP bugs on real-world applications called BUGSPHP, which can enable research on analysis, testing, and repair for PHP programs. The dataset consists of training and test datasets, separately curated from GitHub and processed locally. The training dataset includes more than 600,000 bug-fixing commits. The test dataset contains 513 manually validated bug-fixing commits equipped with developer-provided test cases to assess patch correctness.

==> listings/responses.tex <==
\begin{figure}[t]

\begin{subfigure}[t]{0.47\textwidth}
\begin{lstlisting}[numbers=none, basicstyle=\scriptsize\ttfamily,
columns=flexible,
breaklines=true,
keepspaces=true, 
frame=tb,]
Topic:
denominatorDegreeOfFreedom in FDistribution leads 
to IllegalArgumentsException in
UnivariateRealSolverUtils.bracket

Description:
The problem is the 'initial' parameter to that 
function, wich is POSITIVE_INFINITY and therefore not 
within the boundaries. I already pinned down 
the problem to the FDistributions 
getInitialDomain()-method, wich goes like:

return getDenominatorDegreesOfFreedom() /
(getDenominatorDegreesOfFreedom() - 2.0);

Obviously, in case of  denominatorDegreesOfFreedom 
is 2, this must lead to a division-by-zero, resulting 
in POSTIVE_INFINITY. 

\end{lstlisting}

\caption{bug report for MATH-227}
\label{lst:example-bug-report}
\end{subfigure}

\vspace{0.1in}

\begin{subfigure}[t]{0.47\textwidth}
\centering
\begin{lstlisting}[language=java, floatplacement=b, frame=tb, basicstyle=\scriptsize\ttfamily]
double getInitialDomain(double p, double d) {
   double ret;
   ret = d / (d - 2.0);
   return ret;
}
\end{lstlisting}
\caption{buggy code in MATH-227}
\label{lst:example-bug}
\end{subfigure}

\vspace{0.1in}

\begin{subfigure}[t]{0.47\textwidth}
\centering
\begin{lstlisting}[language=java,floatplacement=b, frame=tb, basicstyle=\scriptsize\ttfamily]
T wrapper_method(Parameters p ...) {
  if (instrumentation_enabled) {
    T result = original_method(p);
    if (<condition_for_buggy_behavior>) {
      throw new RuntimeException("[Defects4J_BugReport_Violation]");
    }
      return result;
   } else {
      return original_method(p);
   }
}
\end{lstlisting}
\caption{oracle instrumentation template for MATH-227}
\label{lst:instrumentation-template}
\end{subfigure}

\vspace{0.1in}

\begin{subfigure}[t]{0.47\textwidth}
\centering
\begin{lstlisting}[language=java, floatplacement=tbp, frame=tb, basicstyle=\scriptsize\ttfamily]
double getInitialDomain(double p, double d) {
   if (Boolean.parseBoolean(System.getProperty("defects4j.instrumentation.enabled"))) {
      double init = getInitialDomain_original(p, d);
      double lowerBound = 0;
      double upperBound = Double.MAX_VALUE;
      if (init < lowerBound || init > upperBound) {
         throw new RuntimeException("[Defects4J_BugReport_Violation]");
      }
      return init;
   } else {
      return getInitialDomain_original(p, d);
   }
}
\end{lstlisting}
\caption{instrumentation for MATH-227}
\label{lst:math227-instrumentation}
\end{subfigure}

\vspace*{-0.05in}
\caption{Illustration of the oracle-generation from a developer provided bug-report and the buggy function, based on MATH-227 in Defects4J benchmark}
\label{tab:types-of-changes}
\vspace*{-0.2in}
\end{figure}

==> sections-old/analysis.tex <==
\section{Experiment Design}

We perform an empirical study using our \bugsphp testing dataset, with LLMs and existing state-of-the-art learning-based APR tools. For this purpose, we train two existing learning-based repair tools with our \bugsphp training dataset and query two pre-trained LLMs. 


\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{./figures/process-flow.pdf}
    \caption{High-level workflow to generate and validate patches for bugs in our \bugsphp test dataset using LLMs. First, we extract the context for the bug and create prompts. Then, using the OpenAI API, we retrieve model responses for each prompt. Finally, we automatically obtain a PHP patch by prepossessing the model response and validate it using the developer test suite. Plausible patches are manually verified against the developer fix.}
    \label{fig:llms-evaluation-process}
\end{figure*}


\subsection{Using Large Language Models}
We use two pre-trained models to evaluate the efficacy of LLMs in generating fixes for PHP bugs in our test dataset. Namely TextDavinci (text-DaVinci-003) and ChatGPT(gpt-3.5-turbo). OpenAI develops both models, and both are part of the GPT-3.5 family. In this section, we explain the process of generating patches using the selected LLMs and detail the setup for our experiments. 


% With 175 billion parameters, TextDavinci is one of the biggest language models ever developed. This model is intended to be a sophisticated NLP system capable of comprehending and producing human-like language in various contexts. It was trained on a massive dataset of internet text, including books, articles, and websites, and it can generate a wide range of responses to prompts and questions.

% TextDavinci can handle various linguistic activities, including translation, text completion, question answering, summarizing, and more. Its performance on these tasks is frequently seen to be on par with or greater than that of humans.

% The ability of the TextDavinci model to generate highly creative and coherent responses to prompts makes it well-suited for creative writing, story generation, and chatbot development. This text generation ability of this language model might be prominent to patch generation tasks. This is what we evaluated using our novel PHP benchmark. 

% \textbf{TextDavinci:} is an advanced Natural Language Processing model that uses a variant of the GPT architecture and has 2.7 trillion parameters, making it one of the largest and most powerful language models available today. This model is designed to understand and produce human-like language in various contexts. It was trained on a massive dataset of internet text, including books, articles, and websites, and it can generate a wide range of responses to prompts and questions. TextDavinci can perform various linguistic tasks, such as translation, text completion, question answering, summarizing, and more, with a performance that is often comparable to or better than that of humans. Its unique ability to produce creative and coherent responses to prompts makes it ideal for creative writing, story generation, and chatbot development. In our empirical study, we evaluate the text generation ability of this language model for patch generation. 

\textbf{TextDavinci:} is one of the largest and most powerful language models, with 175 billion parameters ~\cite{microsoftConceptsOverview}. It can handle various natural language and multimodal tasks, including image captioning, style transfer, and visual reasoning. With its advanced training using reinforcement learning and reward models from human comparisons, TextDavinci can generate creative and coherent texts on virtually any topic. It has been fine-tuned on a vast corpus of text and code from before Q4 2021, resulting in better output quality, longer text, and consistent instruction. TextDavinci also allows for easy insertion of completions within the text ~\cite{openaiOpenAI}.  

% \textbf{ChatGPT:} is the most capable and cost-effective model in the GPT-3.5 family and is optimized for a chat at 1/10th the cost of TextDavinci. This model has been optimized for chat but works well for traditional completion tasks. We can use this model for patch generation tasks like the TextDavinci model. However, output retrieval is different since this model acts as a chatbot.  

% \textbf{ChatGPT:} has advanced NLP capabilities that enable it to comprehend and produce human-like text~\cite{chatgpt}. When analyzing code, this can be helpful because it enables the model to comprehend the code's purpose and find potential errors based on the language used. A sizable amount of text data, including details on software development and programming languages, was used to train ChatGPT. As a result, it has a richer representation of the knowledge and ideas in software development that may be used to identify and correct problems in code. This can help with code debugging since it enables the model to find errors in new code using its prior knowledge. Automating the debugging process can shorten the time and effort needed to detect and repair errors. In our empirical study, we evaluate the text generation ability of this language model for patch generation. 

\textbf{ChatGPT:}  is an AI chatbot developed by OpenAI built on top of GPT-3.5 and has been fine-tuned using supervised and reinforcement learning techniques~\cite{wikipediaChatGPTWikipedia}. ChatGPT has been trained on various sources of text data, including programming languages, internet phenomena like bulletin board systems, and man pages. As a result, it has advanced natural language processing capabilities that enable it to comprehend and generate text that resembles human language. This feature is beneficial in analyzing code because the model can recognize and interpret the code's intent and detect potential errors based on the language used. ChatGPT's extensive training on texts related to software development and programming languages has provided it with a wealth of knowledge and concepts, which it can use to identify and resolve bugs in code ~\cite{chatgpt}.

\textbf{Prompt Generation}: we select the context of the bug by extracting a maximum of 40 lines above the buggy line as prefix context and a maximum of 40 lines below the buggy lines as suffix context. The buggy line is identified using the developer fix location(s). If the context can be encapsulated within a function procedure, we reduce the context to the scope of the modified function. We generate two types of queries, to investigate the impact of providing additional information such as the exact line to fix. Therefor, we generate one prompt (Type-I) without providing the developer fixed line, and a second prompt (Type-II) by providing the exact line to modify. Listing~\ref{lst:input-promt-1} shows the skeleton for a query of Type-I. In this prompt we provide the buggy context and request the model to fix the bug. Listing~\ref{lst:input-promt-2} shows the skeleton for a query of Type-II. In this prompt, we additionally provide information of the line to modify. If the developer fix does not modify existing lines but insert new lines, we keep this field empty. 

\vspace{0.1in}

\begin{lstlisting}[caption=Query Type-I, label={lst:input-promt-1}, numbers=none, frame=single, basicstyle=\scriptsize\ttfamily]
Context: <context>
Given "Context" has a bug.
Fix the bug and give only the correct code "Context".
\end{lstlisting}

\begin{lstlisting}[caption=Query Type-II, label={lst:input-promt-2}, numbers=none, frame=single,basicstyle=\scriptsize\ttfamily]
Context: <context>
Buggy: <buggy lines>
"Buggy" lines contained in the "Context" has bug.
Fix it and give fixed lines.
\end{lstlisting}


% \textbf{Model Configuration}: TextDavinci and ChatGPT has an upper limit of 4096 maximum tokens for context length. %Use other API parameters such as temperature (control randomness of the output), top\_p (an alternative to sampling with temperature, called nucleus sampling, where the model considers the results of the tokens with top\_p probability mass), same during the evaluation and max\_tokens (maximum number of tokens can be generated in completion). 
% We use the default values for the configurable parameters during patch generation for the above two LLMs as shown in 

% For both models, temperature, max\_tokens, top\_p, and model are the standard parameters to be provided when calling the API. The temperature value must be between 0 and 1; lowering the value results in less random completion and repetition. We use a temperature of 0.7, a higher value, to get different kinds of patches in 3 rounds. max\_tokens value set to 800 after we find out the largest token count of the developer patch for a bug in the test dataset is about 800. top\_p is set to 1, which is the default value, and finally passed model names 'text-davinci-003' or 'gpt-3.5-turbo' as value for the model parameter. Figure~\ref{fig:llms-evaluation-process} refers to the high-level evaluation process of LLMs. 



\textbf{Patch Prepossessing}
LLMs does not always generate patches as code, which might include comments in Natural Language. Hence, a prepossessing step is necessary to extract the code from the response. Figure~\ref{fig:response-taxonomy} depicts a categorization we used to classify model responses into different classes. We list 3 types of model responses which can be expected for a prompt. Listing~\ref{lst:response-1} is a typical output generated by the model if its not able to generate a patch. Listing~\ref{lst:response-2} is a example of a correct code generated as the fix for the bug provided in a request prompt. Finally, Listing~\ref{lst:response-3} shows a correct code mixed with comments/explanation in natural language, which makes it difficult to automatically extract the code. In order to correctly recognize the success of the model response, we classify the responses based on the  taxonomy shown in Figure~\ref{fig:response-taxonomy}. 

First we partition the responses into two classes based on the model explicitly stating that a patch was not found. For the response in which a patch is provided, we then categorize if the response include any PHP syntax code. For responses without any code we classify them as "Natural Language Patches" , typically consist of instruction in natural language on how to fix the bug. If the model response provide a PHP code that can be automatically extracted, we collect it as a candidate patch for validation. Such candidate patches are applied to the buggy program and validated using the developer test-suite. 


\begin{figure}[h]
\centering
% \scriptsize
\begin{tikzpicture}[level distance=1.5cm,
  level 1/.style={sibling distance=3.3cm},
  level 2/.style={sibling distance=3cm}]
  level 3/.style={sibling distance=3cm}]
  \node {Model Response}
    child {node {Patch Provided}
      child {node {PHP Code}
        % child{node {PHP Patch}}
        % child{node {PHP Patch with Noise}}
      }
      child {node {Natural Language}}
    }
    child {node {Patch Not Provided}
    };

\end{tikzpicture}
\caption{Taxonomy for model responses}
\label{fig:response-taxonomy}
\end{figure}


\begin{lstlisting}[language=php, caption=Response Type-I, label=lst:response-1, numbers=none, frame=single,basicstyle=\scriptsize\ttfamily]
"There is no bug in the given context."
\end{lstlisting}


\begin{lstlisting}[language=php, caption=Response Type-II, label={lst:response-2}, numbers=none, frame=single,basicstyle=\scriptsize\ttfamily]
Fixed: if ($record->getLevel() < $this->getLevel()) {
\end{lstlisting}

% \begin{lstlisting}[language=php, caption=Response Type-III, label={lst:response-3}, numbers=none, frame=single,basicstyle=\scriptsize\ttfamily]
% "Fixed: !is_numeric($timeLimit) || 0 >= $timeLimit) {"
% \end{lstlisting}

\begin{lstlisting}[language=php, caption=Response Type-III, label={lst:response-3}, numbers=none, 
frame=single,basicstyle=\scriptsize\ttfamily]
"Fixed: if ($hour < 13) {The line should compare the $hour variable with 13 instead of 15, as the 'tengah hari' period should be from 12:00 PM to 1:59 PM, which is before 2:00 PM (14:00) and after 11:59 AM (11:00)"
\end{lstlisting}





% In this example, \texttt{Fixed:} word needs removed to extract the patch. We remove this kind of keyword and extract the code that needs to replace with the buggy code.




% \textbf{Experimental Setup}: we used Google Colab\footnote{https://colab.research.google.com/} to run our experiments with LLMs. Using a virtual machine with 13GB memory and 4vCPUs we queried OpenAI API\footnote{openai_api_ref} to generate patches for the bugs in our test dataset. Listing~\ref{lst:text-davinci-config} depicts the configuration used for \textit{TextDavinci}, Listing~\ref{lst:gpt-turbo-config} shows the configuration used for \textit{ChatGPT}. For each model and for each bug we generated two types of queries as discussed previously, and aggregate the results for 3 repetitions. 


% % \begin{lstlisting}[language=Python, caption=TextDavinci configuration, label={lst:text-davinci-config}]
% % response = openai.Completion.create(
% %         model="text-davinci-003",
% %         prompt = prompt,
% %         temperature=0.7,
% %         max_tokens=800,
% %         top_p=1,
% %         frequency_penalty=0,
% %         presence_penalty=0,
% %         stop=["###"]
% %         )
% % \end{lstlisting}


% % \begin{lstlisting}[language=Python, caption=ChatGPT configuration, label={lst:gpt-turbo-config}]
% % response = openai.ChatCompletion.create(
% %         model="gpt-3.5-turbo",
% %         temperature=0.7,
% %         max_tokens=800,
% %         top_p=1,
% %         messages=[{"role": "user", "content": prompt}]
% %         )
% % \end{lstlisting}







% \textbf{Experimental Setup}: we used Google Colab\footnote{https://colab.research.google.com/} to run our experiments with LLMs. Using a virtual machine with 13GB memory and 4vCPUs we queried OpenAI API\footnote{openai_api_ref} to generate patches for the bugs in our test dataset.


% \subsubsection{Patch Validation}

% To validate the candidate patches, whether correct or not, we ran test cases in two ways and collected the results.
% \begin{itemize}
%     \item Run only failing test cases.
%     \item Run all the related test cases.
% \end{itemize}

% \subsubsection{Patch Results and Manual Validation}





% We analyze the patch Results according to whether it was a "Giving Patch" or "Not Giving Patch." For some bugs, the model responses are like, "There is no bug in the given context." The model says there is no bug in the code. Those responses are categorized under the "Not Giving Patch." 

% \vspace{5mm}
% \noindent \texttt{"There is no bug in the given context."}
% \vspace{5mm}

% The rest of the responses are categorized under the "Giving Patch." Models give patches as PHP code or natural language explanation. Some responses model explain how to fix the bug without giving an exact PHP code. Those responses are categorized under the "Natural Language." 



% The rest of the responses are categorized under the ”PHP Code.” Again we analyze how many patches could extract or not from the given PHP code patches. Table~\ref{tab:model-responses-results} included those details. Some patches include some noisy words before and after the patch. So we have to extract patches from those kinds of results. The "PHP Patch" consists of the number of patches that extract like that. 



% The rest of the patches are categorized under "PHP Patch with Noise." There is some manual effort needed to extract that patches. We did this categorization manually. 


\subsection{Using State of the Art Repair Models}

\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{./figures/apr_tool_experiment_flow.pdf}
    \caption{High-level overview of the process to evaluate state-of-the-art learning-based repair tools using our training and test data in \bugsphp. First part depicts the training process and the second part depicts the inference process. Plausible patches generated by each tool is manually compared against the developer fix to determine semantic equivalence.}
    \label{fig:apr-evaluation-process}
\end{figure*}

We select two existing state-of-the-art learning-based  program repair tools to evaluate the capabilities in fixing PHP bugs from our dataset. For this purpose, we select CURE~\cite{jiang2021cure} and RewardRepair~\cite{ye2022neural} which have been shown to outperform existing state of the art tools for bugs in Defects4J~\cite{just2014defects4j}. We retrain the models using our training dataset and evaluate the efficacy using the test dataset. 


\textbf{CURE:} is a new NMT-based APR technique with three significant improvements. CURE consists of two models with two different architectures CoNuT and FConv \cite{gehring2017convolutional}. The Pre-trained Programming language (PL) model is trained to predict the subsequent tokens in code sequences and learns to generate developer-like code. The code-aware beam-search strategy did more correct fixes by inducing more compilable patches and similar lengths to the buggy line. CURE used the byte-pair encoding sub-word tokenization technique to tokenize compound and rare words to address the Out of Vocabulary (OOV) problem. CURE uses word-level tokenization to separate code lines by spaces, camel case letters, underscores, strings, and numbers.

\textbf{RewardRepair:} is a new repair model built on a mix of syntactic and semantic training objectives. This model combines semantic training based on program execution with token-level syntactic training. It uses program compilation and test execution-based loss functions to improve Neural Machine Translation (NMT)-based program repair. They use discriminators to compile and run test cases to generate patches and provide high-quality feedback about patch quality. The neural network weight is updated according to feedback.

% \subsubsection{Experimental Setup}
\textbf{Training:} we trained CURE and RewardRepair models with our newly created PHP training dataset. We extract 500k samples of buggy context data to train the models. Context in CURE induces a maximum of 40 lines of prefix context, buggy lines, and 40 lines of suffix context. If the buggy function is within that line limit, we extract only the buggy function. In RewardRepair we used maximum token length to 512 which is default value use in this tool. Then we prepare the data input format file for each tool using the buggy context, buggy lines, and patch. then we trained the tools. RewardRepair tool has two training steps syntactic training and semantic training. In our experiments we train the model using only syntactic training step which is typical training process for program repair tools. 

% \subsection{Patch Generation and Validation}
\textbf{Patch Generation:} using \bugsphp test dataset of 513 PHP bugs, to evaluate the APR tools. First, we extract the buggy context and buggy lines, and then prepare the input format for the tools. We generate 100 candidate patches for each bug in our dataset using the PHP-trained CURE and RewardRepair tools. Figure~\ref{fig:apr-evaluation-process} show the high-level workflow of APR tools training and inference processes.

% \subsection{Results}

==> sections-old/bug-data.tex <==
\section{Bug Data Set Construction}
In this section, we discuss the methodology of curating our dataset and analysis of our proposed benchmark \bugsphp. We collect 513 bugs from 15 open-source PHP applications based on the \phpunit testing framework. \bugsphp contains each bug’s buggy version, fixed version, and related test cases. \bugsphp also provides a simple interface to use the dataset. Our dataset can be used to evaluate program repair techniques as well as software testing and program analysis techniques. 

% \begin{figure*}[!htb]
%     \centering
%     \includegraphics[width=1\linewidth]{./figures/benchmark_flow_diagram.pdf}
%     \caption{High-level process for curating a list of 513 bugs in PHP applications. We generate a dataset of PHP bugs from top-75 most popular PHP applications in GitHub. Manually filtering repositories that does not include a developer provided test-suite and test-cases incompatible with the latest stable PHP version 8.1 }
%     \label{fig:benchmark_flow}
% \end{figure*}

\begin{figure*}[!htb]
    \centering
    \includegraphics[width=1\linewidth]{./figures/benchmark_flow_diagram.pdf}
    \caption{High-level process for curating a list of 513 bugs in PHP applications and training dataset. We generate a BugsPHP dataset of PHP bugs from the top-75 most popular PHP applications and a training dataset from 4k PHP applications in GitHub. BugsPHP dataset manually filtering repositories that do not include a developer provided test-suite and test cases incompatible with the latest stable PHP version 8.1 }
    \label{fig:benchmark_flow}
\end{figure*}

For bug collection, we queried for PHP projects on GitHub. We used the history in the git version control system for the subject programs to find bugs and the corresponding patches offered by developers to curate our benchmark of real PHP bugs. Developers manually mark the program revisions where reported bugs are fixed (bug-fixing commits or patches). The version before the bug-fixing commit is considered as the buggy commit. This allowed us to extract a combination pair of the buggy program version and the fixed program version. We filtered our results further for the purpose of removing unusable data by applying the following criteria:


\begin{itemize}
    \item Developer fix should be restricted to PHP files.
    \item A fix commit must contain one or more test cases that can be used to validate the bug fix. The same test case(s) can also be used to identify the existence of the bug. 
    \item The developer patch should not contain file addition, deletion, or renaming. Such modifications to the source files are usually refactoring effects and can obfuscate the relevant fix. 
 
\end{itemize}

% \begin{figure}[!htb]
%   \centering
%   \includegraphics[width=0.5\linewidth]{figures/benchmark_flow_diagram.png}
%   \caption{High-level flow diagram of benchmark bug collection process.}
%   \label{fig:benchmark_flow}
% \end{figure}



Figure~\ref{fig:benchmark_flow} depicts the high-level overview of the process for curating the dataset of PHP bugs. We systematically crawl open-source PHP projects hosted in GitHub, extract all commit history to identify bug-fixing commits and filter potential bug-fixing commits using the above criteria. For each potential bug-fixing commit we manually validated the fix commit and the test cases for inclusion in our dataset. Table~\ref{table:data-set} shows the details of the curated subject list.

\input{tables/table-subjects}

\textbf{Subject Systems Selection}: We used GitHub REST API \footnote{https://docs.github.com/en/rest?apiVersion=2022-11-28} to retrieve the repositories for PHP. First, we sort the repositories based on the popularity, measured using the stargazers count (i.e. number of stars) and we set the latest commit date greater than 2021 to make sure that the repositories are recently updated. From the ranked list of repositories, we select the top-75 repositories to collect commits. For each repository, we manually inspected the code for the availability of developer test cases and removed those which do not have such test suites readily available. 

\textbf{Collection of Bugs}: For each filtered repository we collect commits ranging from 2020 Jan to 2023 March. We search for commits with commit messages that include terms like \texttt{"fix"}, \texttt{"solve"}, \texttt{"bug"}, \texttt{"issue"}, \texttt{"problem"} or \texttt{"error"}. We note that this process can be incomplete but such approximations have been shown to be useful for curating bug datasets in previous studies~\cite{tufano2019empirical}. We further filter out and remove commits with source file addition, deletion, and renaming, which we consider to be part of refactoring and irrelevant for the bug fix. Finally, we filter commits with changes of lines larger than 50 and changes of files larger than 3 similar to previous work~\cite{gyimesi2019bugsjs}.  

\textbf{Test Validation}: Once we curate the list of commits, we manually checked that the test cases can be used to validate the fix. We chose PHP version 8.1 because currently, it is the latest stable PHP version, and we removed the repositories that could not run test cases due to PHP version incompatibility. 
We manually run all the test cases on the fixed version of the program (i.e. fix commit) and generate the test coverage report. Using the test coverage report, we identify the relevant test cases that reach the modified location(s) of the commit. We select the appropriate passing test cases covering the modified fix locations within a neighborhood of 10 lines. We run selected relevant test cases on the buggy version of the program (i.e. the parent commit) to identify at least one failing test case. We select commits that have at least one failing test case from its parent commit, which constitutes a program pair of (buggy version, fixed version). Our evaluation finds 513 bugs listed in Table~\ref{table:data-set}. 




% \vspace{5mm}
% \noindent 5. Infrastructure and Implementation of the Final Benchmark
% \vspace{5mm}

% \bugsphp supports common activities related to the bug benchmarks, such as checking out buggy or fixed versions of the specific commit and running the test cases.
% \vspace{5mm}

% \noindent \textbf{Infrastructure.} The following commands are available in the CLI:

% \begin{itemize}
%     \item -p: Project name - project name should give as a combination of repository owner and repository name Ex - \begin{verbatim}
%  <owner-name>--<repository-name>
% \end{verbatim}
%     \item -b: Bug number 
%     \item -t: task
%         \begin{itemize}
%         \item checkout: Checks out the source code into the given output path.
%         \item install: Install the composer and necessary packages.
%         \item test: Run all the test cases
%         \end{itemize}
%     \item -v: Bug version
%         \begin{itemize}
%         \item buggy: The original buggy code
%         \item fixed: Bug fixed code with updated test cases
%         \end{itemize}
%     \item -c: Test case number (optional). If we input the test case number with the task test. It will run only that particular test case.
%     \item -o: Output path where the source code should be checkout
% \end{itemize}

% \vspace{5mm}
% \noindent \textbf{Example Commands}

% 1. Checks out the source code for a given bug
% \begin{itemize}
%     \item python3 main.py -p composer--composer -b 1 -t checkout -v fixed -o /content/tmp/
% \end{itemize}

% 2. Install the necessary packages
% \begin{itemize}
%     \item python3 main.py -p composer--composer -b 1 -t install -v fixed -o /content/tmp/
% \end{itemize}

% 3. Run all the test cases
% \begin{itemize}
%     \item python3 main.py -p composer--composer -b 1 -t test -v fixed -o /content/tmp/
% \end{itemize}

% 4. Run only a given test case
% \begin{itemize}
%     \item python3 main.py -p composer--composer -b 1 -t test -v fixed -c 1 -o /content/tmp/
% \end{itemize}

% \vspace{5mm}

\vspace{5mm}
\noindent 6. Benchmark Bug Distribution
\vspace{5mm}

BugsPHP benchmark contains 513 bugs from 15 projects. All bugs are mainly classified into two categories. They are bug distribution by the number of file changes and the number of line changes. Figure~\ref{fig:file-distribution} and Figure~\ref{fig:line-distribution} listed the distribution of the bugs.


\begin{figure*}[h!]
\captionsetup[subfigure]{justification=centering}
    \centering
    \begin{subfigure}[]{0.30\textwidth}
        \centering
       \includegraphics[width=0.9\textwidth]{./figures/number_of_file_changes.pdf}
       \caption{file changes in bug data-set}
       \label{fig:file-distribution}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[]{0.30\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]
        {./figures/bug_lines_distribution.pdf}
       \caption{line changes in bug data-set}
       \label{fig:file-distribution}

    \end{subfigure}
    ~
    \begin{subfigure}[]{0.30\textwidth}
        \centering
       \includegraphics[width=0.9\textwidth]{./figures/bug_categories.pdf}
       \caption{patch types in bug data-set}
       \label{fig:file-distribution}
    \end{subfigure}%

    
    \begin{subfigure}[]{0.30\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{./figures/number_of_file_changes_training.pdf}
       \caption{file changes in training data-set}
       \label{fig:file-distribution}
    \end{subfigure}
    ~
     \begin{subfigure}[]{0.30\textwidth}
        \centering
       \includegraphics[width=0.9\textwidth]{./figures/number_of_line_changes_training.pdf}
        \caption{line changes in training data-set}
       \label{fig:file-distribution}
    \end{subfigure}%
    % ~ 
    % \begin{subfigure}[]{0.30\textwidth}
    %     \centering
    %     \includegraphics[width=0.9\textwidth]{./figures/number_of_file_changes.pdf}
    %     \caption{patch types in training data-set}
    %    \label{fig:file-distribution}
    % \end{subfigure}
     \caption{Statistical analysis of the bug data-set and training data-set in \bugsphp: }
    \label{fig:file-distribution}
\end{figure*}



% \begin{figure}[!htb]
% \centering
%   \includegraphics[width=0.4\textwidth]{./figures/number_of_file_changes.pdf}
%   \caption{Bugs distribution by number of file changes}
%   \label{fig:file-distribution}
% \end{figure}

% \begin{table}[!htb]
% \centering
%  \caption{Bugs distribution by number of file changes}
% \begin{tabular}{|l|r|}
%     \hline
%     \textbf{Number of File Changes} & \textbf{Number Of Bugs}\\
%     \hline
%     1 file & 473\\
%     \hline
%     2 file & 30\\
%     \hline
%     3 file & 10\\
%     \hline
%     \hline
%     Total & 513\\
%     \hline
%     \end{tabular}
% \label{tab:bugsphp-bugs-categorization-file}
% \end{table}


% \begin{table}[!htb]
% \centering
%  \caption{Bugs distribution by number of line changes}
% \begin{tabular}{|l|r|}
%     \hline
%     \textbf{Number of Line Changes} & \textbf{Number Of Bugs}\\
%     \hline
%     1 - 10 & 349\\
%     \hline
%     10 - 20 & 89\\
%     \hline
%     20 - 30 & 50\\
%     \hline
%     30 - 40 & 13\\
%     \hline
%     40 - 50 & 12\\
%     \hline
%     \hline
%     Total & 513\\
%     \hline
%     \end{tabular}
% \label{tab:bugsphp-bugs-categorization-line}
% \end{table}

\vspace{5mm}
\noindent 7. Benchmark Patch Distribution
\vspace{5mm}

The developer patch for each bug has been categorized manually. Patches of all bugs are mainly classified under three categories. They are Lines Insertion, Lines Deletion, and Lines Modification, as shown in Figure~\ref{fig:main-categories}. Every bug has a secondary category, as shown in Figure~\ref{fig:sub-categories}. (Note: some bugs can be categorized into multiple categories)

% \begin{figure}[!htb]
% \centering
%   \includegraphics[width=0.4\textwidth]{./figures/line-distribution.pdf}
%   \caption{Bugs distribution by number of line changes}
%   \label{fig:line-distribution}
% \end{figure}

% \begin{table}[!htb]
% \centering
%  \caption{Main Patch Categories}
% \begin{tabular}{|l|r|}
%     \hline
%     \textbf{Category} & \textbf{Number Of Bugs}\\
%     \hline
%     Modifying statement & 263\\
%     \hline
%     Inserting statement & 243\\
%     \hline
%     Deleting statement & 7\\
%     \hline
%     \end{tabular}
% \label{tab:bugsphp-main-patch-categories}
% \end{table}

% \begin{figure}[!htb]
% \centering
%   \includegraphics[width=0.4\textwidth]{./figures/main-categories.pdf}
%   \caption{Main Patch Categories}
%   \label{fig:main-categories}
% \end{figure}

% \begin{table}[!htb]
% \centering
%  \caption{Secondary Patch Categories}
% {\begin{tabular}{|l|r|}
%     \hline
%     \textbf{Category} & \textbf{Number Of Bugs}\\
%     \hline
%     Add break, continue statement & 1\\
%     \hline
%     Add new case in Switch statement & 1\\
%     \hline
%     Add parentheses & 1\\
%     \hline
%     Adding conditional block & 134\\
%     \hline
%     Adding foreach loop & 19\\
%     \hline
%     Adding function call & 4\\
%     \hline
%     Adding new function & 3\\
%     \hline
%     Adding try catch & 7\\
%     \hline
%     Adding while loop & 3\\
%     \hline
%     Assignment & 59\\
%     \hline
%     Casting variable & 2\\
%     \hline
%     Change Message & 6\\
%     \hline
%     Change operator & 2\\
%     \hline
%     Declare new function & 17\\
%     \hline
%     Deleting existing condition & 2\\
%     \hline
%     Exception handling & 1\\
%     \hline
%     Function argument change & 31\\
%     \hline
%     Function call & 50\\
%     \hline
%     Function return type modification & 1\\
%     \hline
%     Implements super class & 1\\
%     \hline
%     Modify conditional block & 65\\
%     \hline
%     Modify function parameter & 16\\
%     \hline
%     Regex & 20\\
%     \hline
%     Return value change & 28\\
%     \hline
%     SQL query change & 1\\
%     \hline
%     Variable/object declaration & 33\\
%     \hline
%     \end{tabular}
%  }{}
%  \label{tab:bugsphp-secondary-patch-categories}
% \end{table}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]
    {./figures/sub-categories.pdf}
    \caption{Secondary Patch Categories}
    \label{fig:sub-categories}
\end{figure*}

% \begin{figure*}[!htb]
%     \centering
%     \includegraphics[width=0.9\linewidth]{./figures/benchmark_flow_diagram.pdf}
%     \caption{High-level flow diagram of benchmark bug collection process.}
%     \label{fig:benchmark_flow}
% \end{figure*}









==> sections-old/bug-data_v2.tex <==
\section{\bugsphp Data Set}
In this section, we present the methodology we followed to curate a dataset of PHP bugs and provide an statistical overview. Our new dataset, \bugsphp, includes a training dataset of 653,606 PHP bugs and a test dataset of 513 bugs from the most popular open-source applications collected from GitHub between January 2021 and March 2023. Each bug in the test dataset includes its buggy version, fixed version, and related test cases. Our dataset can be useful to evaluate program repair techniques, software testing, and program analysis techniques.

\subsection{\bugsphp Test Dataset}

\begin{figure*}[!htb]
    \centering
    \includegraphics[width=1\linewidth]{./figures/benchmark_flow_diagram.pdf}
    \caption{High-level process for curating a list of 513 bugs in PHP applications and training dataset. We generate a BugsPHP dataset of PHP bugs from the top-75 most popular PHP applications and a training dataset from 4k PHP applications in GitHub. BugsPHP dataset manually filtering repositories that do not include a developer provided test-suite and test cases incompatible with the latest stable PHP version 8.1 }
    \label{fig:benchmark_flow}
\end{figure*}

For bug collection, we queried for PHP projects on GitHub. We used the history in the git version control system for the subject programs to find bugs and the corresponding patches offered by developers to curate our test dataset of real PHP bugs. Developers manually mark the program revisions where reported bugs are fixed (bug-fixing commits or patches). The version before the bug-fixing commit is considered as the buggy commit. This allowed us to extract a combination pair of the buggy program version and the fixed program version. We filtered our results further for the purpose of removing unusable data by applying the following criteria:


\begin{itemize}
    \item Developer fix should be restricted to PHP files.
    \item A fix commit must contain one or more test cases that can be used to validate the bug fix. The same test case(s) can also be used to identify the existence of the bug. 
    \item The developer patch should not contain file addition, deletion, or renaming. Such modifications to the source files are usually refactoring effects and can obfuscate the relevant fix. 
\end{itemize}

% \begin{figure}[!htb]
%   \centering
%   \includegraphics[width=0.5\linewidth]{figures/benchmark_flow_diagram.png}
%   \caption{High-level flow diagram of benchmark bug collection process.}
%   \label{fig:benchmark_flow}
% \end{figure}



Figure~\ref{fig:benchmark_flow} depicts the high-level overview of the process for curating the dataset of PHP bugs. We systematically crawl open-source PHP projects hosted in GitHub, extract all commit history to identify bug-fixing commits and filter potential bug-fixing commits using the above criteria. For each potential bug-fixing commit we manually validated the fix commit and the test cases for inclusion in our dataset. Table~\ref{table:data-set} shows the details of the curated subject list.

\input{tables/table-subjects}

\textbf{Subject Systems Selection}: We used GitHub REST API \footnote{https://docs.github.com/en/rest?apiVersion=2022-11-28} to retrieve the repositories for PHP. First, we sort the repositories based on the popularity, measured using the stargazers count (i.e. number of stars) and we set the latest commit date greater than 2020 Jan to make sure that the repositories are recently updated. From the ranked list of repositories, we select the top-75 repositories to collect commits. For each repository, we manually inspected the code for the availability of developer test cases and removed those which do not have such test suites readily available. 

\textbf{Collection of Bugs}: For each filtered repository we collect commits ranging from 2020 Jan to 2023 March. We search for commits with commit messages that include terms like \texttt{"fix"}, \texttt{"solve"}, \texttt{"bug"}, \texttt{"issue"}, \texttt{"problem"} or \texttt{"error"}. We note that this process can be incomplete but such approximations have been shown to be useful for curating bug datasets in previous studies~\cite{tufano2019empirical}. We further filter out and remove commits with source file addition, deletion, and renaming, which we consider to be part of refactoring and irrelevant for the bug fix. Finally, we filter commits with changes of lines larger than 50 and changes of files larger than 3 similar to previous work~\cite{gyimesi2019bugsjs}.  

\textbf{Test Validation}: Once we curate the list of commits, we manually checked that the test cases can be used to validate the fix. We chose PHP version 8.1 because currently, it is the latest stable PHP version, and we removed the repositories that could not run test cases due to PHP version incompatibility. 
We manually run all the test cases on the fixed version of the program (i.e. fix commit) and generate the test coverage report. Using the test coverage report, we identify the relevant test cases that reach the modified location(s) of the commit. We select the appropriate passing test cases covering the modified fix locations within a neighborhood of 10 lines. We run selected relevant test cases on the buggy version of the program (i.e. the parent commit) to identify at least one failing test case. We select commits that have at least one failing test case from its parent commit, which constitutes a program pair of (buggy version, fixed version). Our evaluation finds 513 bugs listed in Table~\ref{table:data-set}. 


\subsection{\bugsphp Training Data Set}

Figure~\ref{fig:benchmark_flow} depicts the high-level overview of the process for curating the training dataset of PHP bugs. We used GitHub REST API to retrieve the repositories for the training dataset. First, we sort the repositories based on popularity, using the stargazers count. We search for commits with commit messages that include terms like \texttt{"fix"}, \texttt{"solve"}, \texttt{"bug"}, \texttt{"issue"}, \texttt{"problem"} or \texttt{"error"}. Then we systematically crawl open-source PHP projects hosted in GitHub, extract all commit history to identify bug-fixing commits and filter potential bug-fixing commits using the below criteria.

\begin{itemize}
    \item Developer fix should be restricted to PHP files.
    \item The developer patch should not contain file addition, deletion, or renaming. 
    \item Number of file changes should be less than or equal to 3
    \item Number of line changes should be less than or equal to 50
\end{itemize}

We selected the first 5000 repositories and filtered out the repositories used in our test dataset construction. Following the criteria for filtering commits we collected 653,606 bugs from 4483 PHP applications. 

\subsection{Overview of the Data Set}
BugsPHP test dataset contains a total of 654,119 bug fixing commits divided into two subsets; training and testing. The training data-set consist of 653,606 commits and test data-set with 513 commits. We analyze the size of the fix commits in terms of number of line changes and number of file changes to provide an high-level overview of the complexities of the fix commits. Figure~\ref{fig:commit-distribution} depicts the complexity of the commits in both training and test datasets. In terms of number of file changes,  majority of the commits only modify a single file, where 437034 (74.2\%) in training data and 349 (92.2\%) in test data represent single file changes. 




\begin{figure*}[h!]
\captionsetup[subfigure]{justification=centering}
    \centering
    \begin{subfigure}[]{0.23\textwidth}
        \centering
       \includegraphics[width=0.9\textwidth]{./figures/number_of_file_changes.pdf}
       \caption{file changes in test data}
       \label{fig:file-distribution-bug-dataset}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[]{0.23\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]
        {./figures/bug_lines_distribution.pdf}
       \caption{line changes in test data}
       \label{fig:line-distribution-bug-dataset}

    \end{subfigure}
    ~
    % \begin{subfigure}[]{0.30\textwidth}
    %     \centering
    %    \includegraphics[width=0.9\textwidth]{./figures/bug_categories.pdf}
    %    \caption{patch types in bug dataset}
    %    \label{fig:patch-distribution}
    % \end{subfigure}%
    \begin{subfigure}[]{0.23\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{./figures/number_of_file_changes_training.pdf}
       \caption{file changes in training data}
       \label{fig:file-distribution}
    \end{subfigure}
    ~
     \begin{subfigure}[]{0.23\textwidth}
        \centering
       \includegraphics[width=0.9\textwidth]{./figures/number_of_line_changes_training.pdf}
        \caption{line changes in training data}
       \label{fig:file-distribution}
    \end{subfigure}%

    % ~ 
    % \begin{subfigure}[]{0.30\textwidth}
    %     \centering
    %     \includegraphics[width=0.9\textwidth]{./figures/number_of_file_changes.pdf}
    %     \caption{patch types in training data-set}
    %    \label{fig:file-distribution}
    % \end{subfigure}
     \caption{Statistical analysis of the bug data-set and training data-set in \bugsphp: }
    \label{fig:commit-distribution}
\end{figure*}



% \begin{figure}[!htb]
% \centering
%   \includegraphics[width=0.4\textwidth]{./figures/number_of_file_changes.pdf}
%   \caption{Bugs distribution by number of file changes}
%   \label{fig:file-distribution}
% \end{figure}

% \begin{table}[!htb]
% \centering
%  \caption{Bugs distribution by number of file changes}
% \begin{tabular}{|l|r|}
%     \hline
%     \textbf{Number of File Changes} & \textbf{Number Of Bugs}\\
%     \hline
%     1 file & 473\\
%     \hline
%     2 file & 30\\
%     \hline
%     3 file & 10\\
%     \hline
%     \hline
%     Total & 513\\
%     \hline
%     \end{tabular}
% \label{tab:bugsphp-bugs-categorization-file}
% \end{table}


% \begin{table}[!htb]
% \centering
%  \caption{Bugs distribution by number of line changes}
% \begin{tabular}{|l|r|}
%     \hline
%     \textbf{Number of Line Changes} & \textbf{Number Of Bugs}\\
%     \hline
%     1 - 10 & 349\\
%     \hline
%     10 - 20 & 89\\
%     \hline
%     20 - 30 & 50\\
%     \hline
%     30 - 40 & 13\\
%     \hline
%     40 - 50 & 12\\
%     \hline
%     \hline
%     Total & 513\\
%     \hline
%     \end{tabular}
% \label{tab:bugsphp-bugs-categorization-line}
% \end{table}

% \vspace{5mm}
% \noindent 7. Benchmark Patch Distribution
% \vspace{5mm}

% The developer patch for each bug has been categorized manually. Patches of all bugs are mainly classified under three categories. They are Lines Insertion, Lines Deletion, and Lines Modification, as shown in Figure~\ref{fig:patch-distribution}. Every bug has a secondary category, as shown in Figure~\ref{fig:sub-categories}. (Note: some bugs can be categorized into multiple categories)

% \begin{figure}[!htb]
% \centering
%   \includegraphics[width=0.4\textwidth]{./figures/line-distribution.pdf}
%   \caption{Bugs distribution by number of line changes}
%   \label{fig:line-distribution}
% \end{figure}

% \begin{table}[!htb]
% \centering
%  \caption{Main Patch Categories}
% \begin{tabular}{|l|r|}
%     \hline
%     \textbf{Category} & \textbf{Number Of Bugs}\\
%     \hline
%     Modifying statement & 263\\
%     \hline
%     Inserting statement & 243\\
%     \hline
%     Deleting statement & 7\\
%     \hline
%     \end{tabular}
% \label{tab:bugsphp-main-patch-categories}
% \end{table}

% \begin{figure}[!htb]
% \centering
%   \includegraphics[width=0.4\textwidth]{./figures/main-categories.pdf}
%   \caption{Main Patch Categories}
%   \label{fig:main-categories}
% \end{figure}

% \begin{table}[!htb]
% \centering
%  \caption{Secondary Patch Categories}
% {\begin{tabular}{|l|r|}
%     \hline
%     \textbf{Category} & \textbf{Number Of Bugs}\\
%     \hline
%     Add break, continue statement & 1\\
%     \hline
%     Add new case in Switch statement & 1\\
%     \hline
%     Add parentheses & 1\\
%     \hline
%     Adding conditional block & 134\\
%     \hline
%     Adding foreach loop & 19\\
%     \hline
%     Adding function call & 4\\
%     \hline
%     Adding new function & 3\\
%     \hline
%     Adding try catch & 7\\
%     \hline
%     Adding while loop & 3\\
%     \hline
%     Assignment & 59\\
%     \hline
%     Casting variable & 2\\
%     \hline
%     Change Message & 6\\
%     \hline
%     Change operator & 2\\
%     \hline
%     Declare new function & 17\\
%     \hline
%     Deleting existing condition & 2\\
%     \hline
%     Exception handling & 1\\
%     \hline
%     Function argument change & 31\\
%     \hline
%     Function call & 50\\
%     \hline
%     Function return type modification & 1\\
%     \hline
%     Implements super class & 1\\
%     \hline
%     Modify conditional block & 65\\
%     \hline
%     Modify function parameter & 16\\
%     \hline
%     Regex & 20\\
%     \hline
%     Return value change & 28\\
%     \hline
%     SQL query change & 1\\
%     \hline
%     Variable/object declaration & 33\\
%     \hline
%     \end{tabular}
%  }{}
%  \label{tab:bugsphp-secondary-patch-categories}
% \end{table}

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]
%     {./figures/sub-categories.pdf}
%     \caption{Secondary Patch Categories}
%     \label{fig:sub-categories}
% \end{figure*}

% \begin{figure*}[!htb]
%     \centering
%     \includegraphics[width=0.9\linewidth]{./figures/benchmark_flow_diagram.pdf}
%     \caption{High-level flow diagram of benchmark bug collection process.}
%     \label{fig:benchmark_flow}
% \end{figure*}



==> sections-old/bug-data_v3.tex <==
\section{\bugsphp Data Set}
In this section, we present the methodology we followed to curate a dataset of PHP bugs and provide a statistical overview. Our new dataset, \bugsphp, includes a training dataset of 653,606 PHP bugs and a test dataset of 513 bugs from the most popular open-source applications collected from GitHub between January 2021 and March 2023. This dataset can be valuable for evaluating software testing, program analysis techniques, and program repair methods.

The process of curating the \bugsphp dataset is outlined in Figure~\ref{fig:benchmark_flow}. Based on their stargazers count, we use the GitHub Rest API to retrieve the top 5000 PHP repositories with at least one commit after 2021.01.01. Bugs are then collected from these repositories and filtered based on their number of file and line changes. After filtering, the top 75 repositories' bugs are used for the testing dataset, while the remaining 4483 are used for the training dataset. For the bugs in the training dataset, we extract the buggy and fixed versions files for the \bugsphp training dataset. Meanwhile, we conduct a dynamic validation for the bugs in the testing dataset to obtain each bug's corresponding buggy version, fixed version, and test cases.

\subsection{\bugsphp Training Dataset}

% \begin{figure*}[!htb]
%     \centering
%     \includegraphics[width=1\linewidth]{./figures/benchmark_flow_diagram.pdf}
%     \caption{High-level process for curating a list of 513 bugs in PHP applications and training dataset. We generate a BugsPHP dataset of PHP bugs from the top-75 most popular PHP applications and a training dataset from 4k PHP applications in GitHub. BugsPHP dataset manually filtering repositories that do not include a developer provided test-suite and test cases incompatible with the latest stable PHP version 8.1 }
%     \label{fig:benchmark_flow}
% \end{figure*}


\begin{figure*}[!htb]
    \centering
    \includegraphics[width=1\linewidth]{./figures/benchmark_flow_diagram.pdf}
    \caption{The overview of the process curating \bugsphp dataset. }
    \label{fig:benchmark_flow}
\end{figure*}

For bug collection, we queried for PHP projects on GitHub. We used the history in the git version control system for the subject programs to find bugs and the corresponding patches developers offer to curate our training dataset of PHP bugs. Developers manually mark the program revisions where reported bugs are fixed (bug-fixing commits or patches). The version before the bug-fixing commit is considered as the buggy commit. This allowed us to extract a combination pair of the buggy program version and the fixed program version. We filtered our results further to remove unusable data by applying the following criteria:


\begin{itemize}
    \item Developer fix should be restricted to PHP files.
    \item The developer patch should not contain file addition, deletion, or renaming. Such modifications to the source files are usually refactoring effects and can obfuscate the relevant fix. 
\end{itemize}

\textbf{Subject Systems Selection}: We used GitHub REST API \footnote{https://docs.github.com/en/rest?apiVersion=2022-11-28} to retrieve the repositories for PHP. First, we sort the repositories based on the popularity, measured using the stargazers count (i.e. number of stars), and we set the latest commit date greater than 2020 Jan to ensure that the repositories are recently updated. We select the top 5,000 repositories to collect commits from the ranked list of repositories.

\textbf{Collection of Bugs}: We search for commits with commit messages that include terms like \texttt{"fix"}, \texttt{"solve"}, \texttt{"bug"}, \texttt{"issue"}, \texttt{"problem"} or \texttt{"error"}. This process can be incomplete but such approximations are helpful for curating bug datasets in previous studies~\cite{tufano2019empirical}. Finally, we filter and remove commits with changes of lines larger than 50 and changes of files larger than three, similar to previous work~\cite{gyimesi2019bugsjs}.  

We selected the first 5000 repositories and filtered out the repositories used in our test dataset construction. Following the criteria for filtering commits we collected 653,606 bugs from 4483 PHP applications. 

\subsection{\bugsphp Test Dataset}

% Each bug in the test dataset includes its buggy version, fixed version, and related test cases.

For bug collection, we queried for PHP projects on GitHub. We used the history in the git version control system for the subject programs to find bugs and the corresponding patches offered by developers to curate our test dataset of real PHP bugs. We filtered our results further for the purpose of removing unusable data by applying the following criteria:


\begin{itemize}
    \item Developer fix should be restricted to PHP files.
    \item A fix commit must contain one or more test cases that can be used to validate the bug fix. The same test case(s) can also be used to identify the existence of the bug. 
    \item The developer patch should not contain file addition, deletion, or renaming.  
\end{itemize}

% \begin{figure}[!htb]
%   \centering
%   \includegraphics[width=0.5\linewidth]{figures/benchmark_flow_diagram.png}
%   \caption{High-level flow diagram of benchmark bug collection process.}
%   \label{fig:benchmark_flow}
% \end{figure}



Figure~\ref{fig:benchmark_flow} depicts the high-level overview of the process for curating the test dataset of PHP bugs. For each potential bug-fixing commit we manually validated the fix commit and the test cases for inclusion in our dataset. Table~\ref{table:data-set} shows the details of the curated subject list.

\input{tables/table-subjects}

\textbf{Subject Systems Selection}: We used GitHub REST API \footnote{https://docs.github.com/en/rest?apiVersion=2022-11-28} to retrieve the repositories for PHP. First, we sort the repositories based on the popularity, measured using the stargazers count, and we set the latest commit date greater than 2020 Jan to make sure that the repositories are recently updated. From the ranked list of repositories, we select the top-75 repositories to collect commits. For each repository, we manually inspected the code for the availability of developer test cases and removed those which do not have such test suites readily available. 

\textbf{Collection of Bugs}: For each filtered repository we collect commits ranging from 2020 Jan to 2023 March. We search for commits with commit messages that include terms like \texttt{"fix"}, \texttt{"solve"}, \texttt{"bug"}, \texttt{"issue"}, \texttt{"problem"} or \texttt{"error"}. We further filter out and remove commits with source file addition, deletion, and renaming. Finally, we filter and remove commits with changes of lines larger than 50 and changes of files larger than 3.

\textbf{Test Validation}: Once we curate the list of commits, we manually checked that the test cases can be used to validate the fix. We chose PHP version 8.1 because currently, it is the latest stable PHP version, and we removed the repositories that could not run test cases due to PHP version incompatibility. 
We manually run all the test cases on the fixed version of the program (i.e. fix commit) and generate the test coverage report. Using the test coverage report, we identify the relevant test cases that reach the modified location(s) of the commit. We select the appropriate passing test cases covering the modified fix locations within a neighborhood of 10 lines. We run selected relevant test cases on the buggy version of the program (i.e. the parent commit) to identify at least one failing test case. We select commits that have at least one failing test case from its parent commit, which constitutes a program pair of (buggy version, fixed version). Our evaluation finds 513 bugs listed in Table~\ref{table:data-set}.

\subsection{Overview of the Dataset}
BugsPHP dataset contains a total of 654,119 bug fixing commits divided into two subsets; training and testing. The training dataset consist of 653,606 commits and test dataset with 513 commits. We analyze the size of the fix commits in terms of number of line changes and number of file changes to provide an high-level overview of the complexities of the fix commits. Figure~\ref{fig:commit-distribution} depicts the complexity of the commits in both training and test datasets. In terms of number of file changes,  majority of the commits only modify a single file, where 437034 (74.2\%) in training data and 349 (92.2\%) in test data represent single file changes. 2 and 3 file changes in training dataset are 92868 (15.7\%) and 61798 (10.4\%), in the test dataset 30 (5.8\%) and 10 (1.9\%). Same for the number of line changes, 498940 (76.33\%) commits in the training dataset only have 1-10 line changes and 473 (92.2\%) commits in the test dataset have 1-10 line changes as the majority in both datasets. Also, the training dataset contains 101776 (15.6\%) 11-20 line changes, 50195 (7.6\%) 21-30 line changes, 31081 (4.7\%) 31-40 line changes, and 30760 (4.7\%) 41-50 line changes commits.

\begin{figure*}[h!]
\captionsetup[subfigure]{justification=centering}
    \centering
    \begin{subfigure}[]{0.23\textwidth}
        \centering
       \includegraphics[width=0.9\textwidth]{./figures/number_of_file_changes.pdf}
       \caption{file changes in test data}
       \label{fig:file-distribution-bug-dataset}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[]{0.23\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]
        {./figures/bug_lines_distribution.pdf}
       \caption{line changes in test data}
       \label{fig:line-distribution-bug-dataset}

    \end{subfigure}
    ~
    \begin{subfigure}[]{0.23\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{./figures/number_of_file_changes_training.pdf}
       \caption{file changes in training data}
       \label{fig:file-distribution}
    \end{subfigure}
    ~
     \begin{subfigure}[]{0.23\textwidth}
        \centering
       \includegraphics[width=0.9\textwidth]{./figures/number_of_line_changes_training.pdf}
        \caption{line changes in training data}
       \label{fig:file-distribution}
    \end{subfigure}%
     \caption{Statistical analysis of the bug dataset and training dataset in \bugsphp: }
    \label{fig:commit-distribution}
\end{figure*}


==> sections-old/bug-data_v4.tex <==
\section{\bugsphp Dataset}
In this section, we present the methodology we followed to curate a dataset of PHP bugs and provide a statistical overview. Our new dataset, \bugsphp, includes a training dataset of 653,606 PHP bugs and a test dataset of 513 bugs from the most popular open-source applications collected from GitHub between 01 Jan 2021 and March 2023. This dataset can be valuable for evaluating software testing, program analysis techniques, and program repair methods.

\begin{figure*}[!htb]
    \centering
    \includegraphics[width=1\linewidth]{./figures/benchmark_flow_diagram.pdf}
    \caption{The overview of the process curating \bugsphp dataset. }
    \label{fig:benchmark_flow}
\end{figure*}

The process of curating the \bugsphp dataset is outlined in Figure~\ref{fig:benchmark_flow}. Based on their stargazers count, we use the GitHub REST API to retrieve the top 5000 PHP repositories with at least one commit after 01 Jan 2021 (indicating recent development activities). We avoid repositories that are not maintained by filtering those which do not have recent development activities. 
Bugs are then collected from these repositories and filtered based on their number of file and line changes. After filtering, the top 75 repositories' bugs are used for the testing dataset, while the remaining 4483 are used for the training dataset. For the bugs in the training dataset, we extract the buggy and fixed versions files for the \bugsphp training dataset. Meanwhile, we conduct a dynamic validation for the bugs in the testing dataset to obtain each bug's corresponding buggy version, fixed version, and test cases. Below we elaborate each step of the process of curating our dataset. 

\textbf{Repository Selection:} To collect commits, we retrieve PHP repositories using the GitHub REST API \footnote{https://docs.github.com/en/rest?apiVersion=2022-11-28}. Then, we sort them by popularity, measured using the stargazers count (e.g., the number of stars) and the latest commit date. We select only repositories with at least one commit date after 01 Jan 2021 to ensure that we collect bugs from recently updated repositories. Finally, we collect commits from the top 5,000 repositories.

\textbf{Bug Collection:} To collect bugs, we search for PHP projects on GitHub and use the git version control system's history to locate issues and the corresponding solutions developers provided. We follow previous studies (e.g., ~\cite{tufano2019empirical}) and look for commits with messages containing words like ``fix", ``solve", ``bug", ``issue", ``problem" or ``error". Finally, we apply the following criteria similar to those in~\cite{gyimesi2019bugsjs} to filter out unusable data.

\begin{itemize}
    \item The developer fix is applied only to PHP files.
    \item The developer patch should not contain file addition, deletion, or renaming, as such modifications to the source files are usually refactoring effects and can obfuscate the relevant fix. 
\item The number of file changes should be 3 or fewer.
\item The number of line changes should be equal or less than 50. 
\end{itemize}

We sort through repositories containing the bugs that meet the above criteria and have bug fixes committed after 01 Jan 2020. Then, we choose the top 75 most popular repositories from this list to create the \textit{\bugsphp testing dataset}. The rest of the 4483 repositories are used to select bugs for the \textit{\bugsphp training dataset}. 

\textbf{Dataset Labeling:} We obtain the developer commits from the set of repositories selected and designate the commit before the bug-fixing commit as the \textit{buggy version} of the program and the current version as the \textit{fixed version} of the program.

Based on the labeled developer commits, we extract the corresponding buggy version and fixed version files from the repositories designated to obtain the training commits to create the \textit{\bugsphp training dataset}.

The labeled developer commits obtained from the test dataset repositories are fed to the validation process. In creating the \textit{\bugsphp testing dataset}, we perform manual and dynamic validations on the bugs selected for the testing dataset.

\textbf{Manually Validation:} In this step, we examine the latest bug to validate a repository and see if its fixed version has accompanying test cases that can verify the fix. We use the latest stable PHP version, 8.1, to validate fixed versions with these test cases. We select PHP version 8.1 since it is the latest stable PHP version at the time of writing. If the latest bug passes this step, we move that repository to the dynamic validation. If not, we repeat the process with the following bug with the next lower PHP version until we find a bug that passes. This validation is done for each repository until we find at least one bug that successfully pass the validation. Thus, we remove repositories for which we do not find at least one bug that can successfully run the validation. 

\textbf{Dynamic Validation:} we run all the test cases on the fixed version of the program and generate the test coverage report. Then, using the test coverage report, we identify the relevant test cases that reach the fixed version's modified location(s). Next, we select the appropriate passing test cases covering the modified fix locations within a neighborhood of 10 lines. Next, we run selected relevant test cases on the buggy version of the program to identify at least one test case that fails for that buggy version. Finally, we choose the bugs with at least one failing test case. 

\input{tables/table-subjects}

These validation steps result in a testing dataset of 513 bugs, each consisting of the buggy version, the fixed version, and the corresponding test cases. The details of the \textit{\bugsphp testing dataset} are shown in Table~\ref{table:data-set}.



% Table~\ref{table:data-set} shows the details of the curated subject list. 

% Once we curate the list of commits, we manually checked that the test cases can be used to validate the fix. We chose PHP version 8.1 because currently, it is the latest stable PHP version, and we removed the repositories that could not run test cases due to PHP version incompatibility. 

% We manually run all the test cases on the fixed version of the program (i.e. fix commit) and generate the test coverage report. Using the test coverage report, we identify the relevant test cases that reach the modified location(s) of the commit. We select the appropriate passing test cases covering the modified fix locations within a neighborhood of 10 lines. We run selected relevant test cases on the buggy version of the program (i.e. the parent commit) to identify at least one failing test case. We select commits that have at least one failing test case from its parent commit, which constitutes a program pair of (buggy version, fixed version). Our evaluation finds 513 bugs listed in Table~\ref{table:data-set}.

% A fix commit must contain one or more test cases that can be used to validate the bug fix. The same test case(s) can also be used to identify the existence of the bug.

% For each potential bug-fixing commit we manually validated the fix commit and the test cases for inclusion in our dataset. 
% Table~\ref{table:data-set} shows the details of the curated subject list. 
% We set the latest commit date greater than 2020 Jan to make sure that the repositories are recently updated. From the ranked list of repositories, we select the top-75 repositories to collect commits. For each repository, we manually inspected the code for the availability of developer test cases and removed those which do not have such test suites readily available. 

% \textbf{Test Validation}: 


% \subsection{\bugsphp Training Dataset}

% \begin{figure*}[!htb]
%     \centering
%     \includegraphics[width=1\linewidth]{./figures/benchmark_flow_diagram.pdf}
%     \caption{High-level process for curating a list of 513 bugs in PHP applications and training dataset. We generate a BugsPHP dataset of PHP bugs from the top-75 most popular PHP applications and a training dataset from 4k PHP applications in GitHub. BugsPHP dataset manually filtering repositories that do not include a developer provided test-suite and test cases incompatible with the latest stable PHP version 8.1 }
%     \label{fig:benchmark_flow}
% \end{figure*}


\subsection{Overview of the \bugsphp Dataset}
BugsPHP's training dataset has 653,606 fix commits, while the testing dataset has 513 bugs. We analyzed the size of the fix commits in terms of the number of line and file changes to understand the complexities of the fix commits in BugsPHP. Figure~\ref{fig:commit-distribution} shows the complexity of the commits in both the training and test datasets. 

% Most commits modify only one file, with 74.2\% of the training dataset (437034 fix commits) and 92.2\% of the testing dataset (349 bugs) representing single file changes. The percentage of fix commits with 2 and 3 file changes in the training dataset are 15.7\% and 10.4\%, respectively. In the test dataset, 5.8\% of the dataset (30 bugs) have two file changes, whereas 1.9\% of the dataset (10 bugs) have three file changes. We also notice a similar pattern for the number of lines of the commits. In the training dataset, 76.33\% of commits have 1-10 line changes; in the testing dataset, 92.2\% of bugs fall within this range. Also, the training dataset contains 101776 fix commits (15.6\%)  with 11-20 line changes, 50195 fix commits (7.6\%) with 21-30 line changes, 31081 fix commits (4.7\%) with 31-40 line changes, and 30760 fix commits (4.7\%) 41-50 line changes.

Most commits modify only 1 file, with 76.3\% of the training dataset (498940 fix commits) and 92.2\% of the testing dataset (473 bugs) representing single file changes. The percentage of fix commits with 2 and 3 file changes in the training dataset are 14.2\% and 9.5\%, respectively. In the test dataset, 5.8\% of the dataset (30 bugs) have two file changes, whereas 2\% of the dataset (10 bugs) have three file changes. We also notice a similar pattern for the number of lines of the commits. In the training dataset, 67.1\% of commits have 1-10 line changes; in the testing dataset, 68\% of bugs fall within this range. Also, the training dataset contains 101776 fix commits (15.6\%)  with 11-20 line changes, 50195 fix commits (7.7\%) with 21-30 line changes, 31081 fix commits (4.8\%) with 31-40 line changes, and 30760 fix commits (4.8\%) 41-50 line changes.

\begin{figure}[h!]
\captionsetup[subfigure]{justification=centering}
    \centering
    \begin{subfigure}[]{0.45\columnwidth}
        \centering
       \includegraphics[width=0.9\textwidth]{./figures/number_of_file_changes.pdf}
       \caption{file changes in test data}
       \label{fig:file-distribution-bug-dataset}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[]{0.45\columnwidth}
        \centering
        \includegraphics[width=0.9\textwidth]
        {./figures/bug_lines_distribution.pdf}
       \caption{line changes in test data}
       \label{fig:line-distribution-bug-dataset}

    \end{subfigure}
    ~
    \begin{subfigure}[]{0.45\columnwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{./figures/number_of_file_changes_training.pdf}
       \caption{file changes in training data}
       \label{fig:file-distribution}
    \end{subfigure}
    ~
     \begin{subfigure}[]{0.45\columnwidth}
        \centering
       \includegraphics[width=0.9\textwidth]{./figures/number_of_line_changes_training.pdf}
        \caption{line changes in training data}
       \label{fig:file-distribution}
    \end{subfigure}%
     \caption{Statistical analysis of the test dataset and training dataset in \bugsphp, in terms of number of lines and file changes. }
    \label{fig:commit-distribution}
\end{figure}


==> sections-old/conclusion.tex <==
\section{Conclusion}
% PHP has been the most popular server-side language for over two decades but yet there is no  dataset to study logical errors appearing in PHP applications. We curate a dataset of bug fixing commits from most popular open-source PHP applications for the purpose of training learning-based repair tool and evaluating program repair techniques. \bugsphp,  contains 513 bugs from 15 popular open-source PHP applications, which maintains developer written test using the PHPUnit testing framework. 

% We perform an empirical study in fixing logical errors of PHP applications, using the test dataset of \bugsphp. For this purpose, we leverage two Large Language Models: \textit{TextDavinci}, \textit{ChatGPT}, and two state-of-the-art learning-based program repair tools: \textit{CURE} and \textit{RewardRepair}. Our study indicates program repair tools have competitive performance in finding a correct patch compared to pre-trained models which have large number of training data. Furthermore, the number of bugs fixed by both repair techniques and large language models is less than 10\% of the total bugs in our dataset, indicating further research is needed to improve the state-of-the-art program repair techniques for PHP errors. 

PHP has been the most popular server-side language for over two decades, but yet there is no dataset to study logical errors appearing in PHP applications. Hence, we have curated a dataset of bug-fixing commits from the most popular open-source PHP applications to train learning-based repair tools and evaluate program repair techniques. \bugsphp,  contains a training dataset of 653,606 PHP bugs and a test dataset of 513 bugs, which maintains developer-written tests using the PHPUnit testing framework. 

We performed an empirical study in fixing logical errors of PHP applications using the test dataset of \bugsphp. For this purpose, we leveraged two Large Language Models: \textit{TextDavinci}, \textit{ChatGPT}, and two state-of-the-art learning-based program repair tools: \textit{CURE} and \textit{RewardRepair}. Our study indicates program repair tools have competitive performance in finding a correct patch compared to pre-trained Large Language models, which have been trained on vast amounts of data. Furthermore, the number of bugs fixed by repair techniques and large language models is less than 10\% of the total bugs in our dataset, indicating that further research is needed to improve the state-of-the-art program repair techniques for PHP errors.

\begin{tcolorbox}[boxrule=1pt,left=1pt,right=1pt,top=1pt,bottom=1pt]
\textbf{Data Set:}
Our dataset can be accessed via GitHub from the following repository: https://github.com/bugsphp/bugsPHP.git
\end{tcolorbox}

% Researchers can make PHP APR tools to provide more correct patches than these Large Language Models by addressing those issues in their tools. 

==> sections-old/discussion.tex <==
\section{Discussion}

This section analyzes the findings of the empirical study we conducted to assess the effectiveness of LLMs and the state-of-the-art APR tools for automated bug repair in PHP using the newly introduced \bugsphp dataset. 

First, we discuss the effectiveness of LLMs for APR in PHP. Figure~\ref{fig:results-comparison-between-two-method} shows the number of bugs that pass all the test cases for each query type in the model. We observe that Query Type-II performs better in both models than Type-I, indicating that giving the buggy lines to the model is more effective.


\begin{figure}[!htb]
\centering
  \includegraphics[width=0.4\textwidth]{./figures/llm_num_of_uniq.pdf}
  \caption{Number of Bugs Fixes in Each Query Type}
  \label{fig:results-comparison-between-two-method}
\end{figure}



% \begin{figure}[!htb]
%   \includegraphics[width=0.5\textwidth]{./figures/Results Comparison Between Two Methods.png}
%   \caption{Results of the two methods}
%   \label{fig:results-comparison-between-two-method}
% \end{figure}


% \begin{figure}[!htb]
% \begin{tikzpicture}
% \centering
% \begin{axis}[
% 	x tick label style={/pgf/number format/1000 sep=},
% 	ylabel=Number of Bugs,
%     symbolic x coords={Query Type I, Query Type II, tmp},
% 	enlargelimits=0.05,
% 	legend style={at={(0.5,-0.12)},
% 	anchor=north,legend columns=-1},
% 	ybar interval=0.7,
%     xtick=data,  
%     % nodes near coords,
%     % nodes near coords align={vertical},
%  ]
% \addplot coordinates {(Query Type I,5) (Query Type II,41) (tmp,10) };
% \addplot coordinates {(Query Type I,4) (Query Type II,19) (tmp,10) };
% \legend{TextDavinci,ChatGPT}
% \end{axis}
% \end{tikzpicture}
% \caption{Number of Bugs Fixes in Each Query Type}
% \label{fig:results-comparison-between-two-method}
% \end{figure}


After analyzing the results of both models, TextDavinci outperformed ChatGPT even though it is a new model. For query type I TextDavinci generates 5 unique plausible patches, but ChatGPT only generates 4. TextDavinci generates 41 unique plausible patches for query type II, while ChatGPT only generates 19 patches. According to these results, We can say TextDavinci performs better than ChatGPT. Training the model on a given task or dataset to enhance performance is fine-tuning. The TextDavinci model may have been fine-tuned better than the ChatGPT for patch generation of PHP bugs.
% As shown in Table~\ref{tab:all-related-testcase-results} TextDavinci generated 41 patches, which passed all the test cases, while ChatGPT generated only 19 patches for passing all the test cases. This shows the ability of the TextDavinci model in patch generation tasks. Also, from the generated patches, more than 85\% times the TextDavinci model generates the same patches for all three attempts, but the ChatGPT model generates only 75\% as an average. This means TextDavinci is more consistent than ChatGPT. Venn diagram in figure ~\ref{fig:venn_digram} indicates that ChatGPT can generate only eight unique patches while TextDavinci generates 30 unique patches, and it can generate patches that ChatGPT cannot.

Sometimes, ChatGPT generates some noise with a patch, but the TextDavinci model doesn't. Sometimes ChatGPT provides some instruction along with the patch. Below we have included examples of buggy lines in the project and patches generated by the two models. 

\begin{itemize}
    \item buggy line
        \begin{itemize}
        \item  \texttt{if (!is\_numeric(\$timeLimit) || 0 >= \$limit) \{}
        \end{itemize}
    \item TextDavinci model patch
        \begin{itemize}
        \item  \texttt{if (!is\_numeric(\$timeLimit) || 0 >= \$timeLimit) \{}
        \end{itemize}
    \item ChatGPT model patch
        \begin{itemize}
        \item  \texttt{The buggy line is checking the \$limit variable 
        instead of \$timeLimit. Here's the fixed line: Fixed: if (!is\_numeric(\$timeLimit) || 0 >= \$timeLimit) \{}
        \end{itemize}
\end{itemize}

Regarding the overall patch generation for both models, TextDavinci could only generate proper fixes for about 8\% for all bugs. In contrast, ChatGPT generated lesser than that, which is 4\% for all bugs. One reason for this result might be that the training data used for both models is up to 2021 and doesn't include information on some new bugs. The last commit date we use to filter out the bug commit date $ \geq $ 01 Jan 2020, and there can be bugs included in our test dataset after 2021. This might be the reason for not showing many good patch generation results for both models.

In addition to LLMs, we evaluate our test dataset with two state-of-the-art learning-based APR tools. They are CURE and RewardRepair. In the CURE tool, they have generated 5000 candidate patches for each bug; for RewardRepair, they have generated 200 candidate patches. But due to memory limitations, we could generate 100 candidate patches for each bug in both APR tools. After analyzing the results of both APR tools, we can conclude that RewardRepair outperformed CURE for PHP bug repairing even though it is better for Java bug fixing. Venn diagram in figure ~\ref{fig:venn_digram} indicates that CURE can generate only four unique patches while RewardRepair generates 29 unique patches and can generate patches that CURE cannot.

When we consider the overall patch generation for both tools, RewardRepair could generate proper fixes for about 7\% for all bugs, while CURE generated lesser than that, which is 2\% for all bugs. We can say RewardRepair performs better than CURE. Both APR tools generate more patches that pass failing and all the relevant test cases than LLMs. Regarding the overall patch generation for both LLMs, TextDavinci could generate proper fixes for about 5.8\% for all bugs, while ChatGPT generated less than that, which is 2\% for all bugs. We can say TextDavinci performs better than ChatGPT. So by comparing the RewardRepair APR tool and the TextDavinci LLM, we can conclude that still, APR tools are more suitable for patch generation for PHP program bugs. 

==> sections-old/discussion_v1.tex <==
\section{Discussion}

This section analyzes the findings of the empirical study we conducted to assess the effectiveness of LLMs and the state-of-the-art APR tools for automated bug repair in PHP using the newly introduced \bugsphp dataset. 

% First, we discuss the effectiveness of LLMs for APR in PHP. Figure~\ref{fig:results-comparison-between-two-method} shows the number of bugs that pass all the test cases for each query type in the model. We observe that Query Type-II performs better in both models than Type-I, indicating that giving the buggy lines to the model is more effective.


% \begin{figure}[!htb]
% \centering
%   \includegraphics[width=0.4\textwidth]{./figures/llm_num_of_uniq.pdf}
%   \caption{Number of Bugs Fixes in Each Query Type}
%   \label{fig:results-comparison-between-two-method}
% \end{figure}

Analyzing the responses provided by TextDavinci and ChatGPT, we observe that ChatGPT sometimes generates noisy patches: ChatGPT provides some instructions along with the patch. In contrast, TextDavinci always generates candidate patches. For example, below, we show a sample buggy line in a PHP program and the responses provided by two LLMs.  

\begin{itemize}
    \item Buggy line
        \begin{itemize}
        \item  \texttt{if (!is\_numeric(\$timeLimit) || 0 >= \$limit) \{}
        \end{itemize}
    \item TextDavinci model response
        \begin{itemize}
        \item  \texttt{if (!is\_numeric(\$timeLimit) || 0 >= \$timeLimit) \{}
        \end{itemize}
    \item ChatGPT model response
        \begin{itemize}
        \item  \texttt{The buggy line is checking the \$limit variable 
        instead of \$timeLimit. Here's the fixed line: Fixed: if (!is\_numeric(\$timeLimit) || 0 >= \$timeLimit) \{}
        \end{itemize}
\end{itemize}

After analyzing the results of both models, it was found that TextDavinci outperforms ChatGPT even though it is the newer model. For example, when it comes to Query Type-I, TextDavinci can generate five unique plausible patches, while ChatGPT can only generate four. Additionally, for Query Type-II, TextDavinci can generate 41 unique plausible patches, while ChatGPT can only generate 19 patches. ChatGPT's underperformance may be due to its optimization for chat and conversational applications. However, providing feedback to ChatGPT in a conversational manner could help correct its mistakes and generate more accurate patches~\cite{xia2023automated}.

Nevertheless, none of the LLMS is very effective in generating correct patches for PHP bugs. TextDavinci manages to generate proper fixes for only 8\% of the bugs, while ChatGPT generates fixes for just 4\%. One possible explanation for this is that both models have been trained on data that only goes up to 2021, meaning they do not have information on new programs and bugs. The last commit date we used to filter out the bug commit date was set to January 1, 2020, and there may be bugs in our test dataset that were included after 2021. 

% In addition to LLMs, we evaluate our test dataset with two state-of-the-art learning-based APR tools. They are CURE and RewardRepair. In the CURE tool, they have generated 5000 candidate patches for each bug; for RewardRepair, they have generated 200 candidate patches. But due to memory limitations, we could generate 100 candidate patches for each bug in both APR tools. After analyzing the results of both APR tools, we can conclude that RewardRepair outperformed CURE for PHP bug repairing even though it is better for Java bug fixing. Venn diagram in figure ~\ref{fig:venn_digram} indicates that CURE can generate only four unique patches while RewardRepair generates 29 unique patches and can generate patches that CURE cannot.

% When we consider the overall patch generation for both tools, RewardRepair could generate proper fixes for about 7\% for all bugs, while CURE generated lesser than that, which is 2\% for all bugs. We can say RewardRepair performs better than CURE. Both APR tools generate more patches that pass failing and all the relevant test cases than LLMs. Regarding the overall patch generation for both LLMs, TextDavinci could generate proper fixes for about 5.8\% for all bugs, while ChatGPT generated less than that, which is 2\% for all bugs. We can say TextDavinci performs better than ChatGPT. So by comparing the RewardRepair APR tool and the TextDavinci LLM, we can conclude that still, APR tools are more suitable for patch generation for PHP program bugs. 

Next, we analyze the results of the two state-of-the-art APR tools evaluated on our \bugsphp dataset. The results indicate that CURE can only generate four unique patches, while RewardRepair generates 29 unique patches, including those that CURE cannot generate. When looking at the overall patch generation of both tools, RewardRepair was able to generate proper fixes for about 7\% of all bugs, while CURE only generated 2\% of all bugs. From this, we can conclude that RewardRepair is better than CURE for PHP bug repairing, even though CURE is better suited for Java bug fixing.

==> sections-old/introduction.tex <==
% \section{Introduction}
% The exciting area of research and development known as Automated Program Repair (APR) aims to automate resolving software bugs. APR has recently received a lot of attention from the software engineering community because of its potential to cut down on the expense and duration of bug fixes. Using program analysis~\cite{propr}, program synthesis~\cite{angelix, cpr}, evolutionary algorithms~\cite{genprog,arja} and  machine learning algorithms~\cite{jiang2021cure,lutellier2020coconut} to automatically develop patches for software bugs is the state-of-the-art in APR. These techniques involve evaluating the code to determine the root cause of the bug and then creating a patch that fixes the bug while preserving the original program functionality. Genetic programming, which entails developing a population of candidate patches and evolving them over several generations until a good patch is identified, is one of the most initial methods for program repair~\cite{genprog12}. More recently, with the rapid development of Large Language Models(LLMs), more active interest lies if LLMs can be used for the problem of program repair. 
% Learning-based techniques, which entail training models on a large corpus of code and natural language descriptions, can produce semantically meaningful patches and are understandable by humans~\cite{xia2023automated}.


% Hypertext Preprocessor (PHP) is the web applications' most popular server-side scripting language. It was introduced in 1994 and is now powering many large-scale e-commerce applications. PHP is an open-source and general-purpose language. According to W3Techs \cite{W3Techs}, PHP is used by 77.5\% of websites as the server-side scripting language. Since the easy use of PHP, it is still among the top choices for web development. Despite its popularity, weak typing, poor performance, and lack of debugging tools cause errors in PHP web applications. However, there is little attention to applications written in PHP from the research community. A well-organized labeled PHP bugs dataset is missing to facilitate further studies of the software evolution, maintenance and repair of PHP applications. 


% This paper proposes \bugsphp,  a benchmark of 513 bugs in 15 open-source PHP applications based on the PHPUnit testing framework. We curate our benchmark for PHP bugs, similar to those recent work in curating benchmarks of bugs proposed and widely used for program repair tasks, such as BugsJS \cite{gyimesi2019bugsjs}, Defects4J \cite{just2014defects4j}, QuixBugs \cite{lin2017quixbugs}, and Bugs.jar \cite{bugsjar}. \bugsphp contains each bug's buggy version, fixed version, and related test cases. Overall this work aims to benefit the community by offering a valuable data-set for PHP bug identification and prevention, enhancing the reliability and security of PHP applications. Mainly this paper makes the following contributions:

% \begin{itemize}
%     \item \bugsphp, a benchmark of 513 PHP bugs in 15 popular open-source projects, validated them on the PHPUnit testing framework. 
%     \item A quantitative and qualitative analysis of the types of errors in PHP applications captured in \bugsphp
%     \item Preliminary study on the effectiveness of Large Language Models for repairing logical-errors in PHP applications
% \end{itemize}

% In the later sections, this paper discussed our methodology to construct the benchmark \bugsphp, a data-set representation, and the result we obtained after evaluating with LLMs, namely \textit{text-davinci-003} (i.e. TextDavinci) and \textit{gpt-3.5-turbo} (i.e. ChatGPT).

% Automated Program Repair (APR) aims to automate resolving software bugs. APR has recently received a lot of attention from the software engineering community due to its potential to cut down on the expense and duration of bug fixes. Using program analysis~\cite{propr}, program synthesis~\cite{angelix, cpr}, evolutionary algorithms~\cite{genprog,arja} and  machine learning algorithms~\cite{jiang2021cure,lutellier2020coconut} to automatically develop patches for software bugs is the state-of-the-art in APR. These techniques involve evaluating the code to determine the root cause of the bug and then creating a patch that fixes the bug while preserving the original program functionality. Genetic programming, which entails developing a population of candidate patches and evolving them over several generations until a good patch is identified, is one of the most initial methods for program repair~\cite{genprog12}. More recently, with the rapid development of Large Language Models(LLMs), more active interest lies if LLMs can be used for the problem of program repair. Learning-based techniques, which entail training models on a large corpus of code and natural language descriptions, can produce semantically meaningful patches and are understandable by humans~\cite{xia2023automated}.


% Hypertext Preprocessor (PHP) is the web applications' most popular server-side scripting language. It was introduced in 1994 and is now powering many large-scale e-commerce applications. PHP is an open-source and general-purpose language. According to W3Techs \cite{W3Techs}, PHP is used by 77.5\% of websites as the server-side scripting language. Since the easy use of PHP, it is still among the top choices for web development. Despite its popularity, weak typing, poor performance, and lack of debugging tools cause errors in PHP web applications. However, there is little attention to applications written in PHP from the research community. A well-organized labeled PHP bugs dataset is missing to facilitate further studies of the software evolution, maintenance and repair of PHP applications. 


% This paper proposes \bugsphp,  a benchmark of 513 bugs in 15 open-source PHP applications based on the PHPUnit testing framework. We curate our benchmark for PHP bugs, similar to those recent work in curating benchmarks of bugs proposed and widely used for program repair tasks, such as BugsJS \cite{gyimesi2019bugsjs}, Defects4J \cite{just2014defects4j}, QuixBugs \cite{lin2017quixbugs}, and Bugs.jar \cite{bugsjar}. \bugsphp contains each bug's buggy version, fixed version, and related test cases. Overall this work aims to benefit the community by offering a valuable data-set for PHP bug identification and prevention, enhancing the reliability and security of PHP applications. Mainly this paper makes the following contributions:

% \begin{itemize}
%     \item \bugsphp, a benchmark of 513 PHP bugs in 15 popular open-source projects, validated them on the PHPUnit testing framework. 
%     \item A quantitative and qualitative analysis of the types of errors in PHP applications captured in \bugsphp
%     \item Preliminary study on the effectiveness of Large Language Models for repairing logical-errors in PHP applications
% \end{itemize}

% In the later sections, this paper discussed our methodology to construct the benchmark \bugsphp, a data-set representation, and the result we obtained after evaluating with LLMs, namely \textit{text-davinci-003} (i.e. TextDavinci) and \textit{gpt-3.5-turbo} (i.e. ChatGPT).

% Over 77\% of all websites utilize PHP, making it a popular programming language for web development \cite{W3Techs}. PHP is susceptible to bugs, just like any other piece of software. Bugs can range from trivial problems to significant security flaws that could harm users and companies that depend on web apps. Thus, one of the most critical research areas is the investigation of PHP bugs.
% The stability and security of web applications are significant reasons to examine PHP bugs. Bugs can have severe consequences, ranging from data loss to illegal access by intruders. The most common way for attackers to access data without authorization is through web application vulnerabilities. Researchers can discover prevalent problems and create plans to avoid or mitigate them by investigating PHP bugs, ultimately increasing web applications' stability and security. Analyzing PHP bugs also aims to boost software development's effectiveness and efficiency. Bug fixes can take a long time, cost money, and postpone the introduction of new features or products. Developers can save time and money and concentrate on making better software by understanding the causes of PHP bugs and implementing tools and approaches for finding and fixing them. Research into PHP bugs has the potential to be significant for educational purposes. Teachers can teach students the value of testing and debugging and the need for excellent coding methods and attention to detail by examining real-world instances of PHP errors and their causes. 

% Understanding the size and scope of the issue is a crucial driver for researching the effects of PHP bugs on the present software landscape. While many PHP errors are minor and have little impact on users, others can have severe consequences. Researchers can identify the most critical problems and create mitigation plans by researching how PHP vulnerabilities have affected the present software landscape. Additionally, studying the effects of PHP bugs can aid companies and organizations in comprehending the dangers and expenses related to web application development. Researchers can determine the most frequent causes of defects and create preventative measures by examining the effects of PHP problems on the state of the software industry. The danger of data breaches and other security incidents, which may be expensive and destructive to a company's brand, can be decreased. According to an IBM report from 2022, \cite{IBM_data_breach_2022}, the average cost of a data breach is \$4.35 million, and it takes 277 days to find and stop a breach. According to IBM research, more than three-quarters of a year is required to detect and contain a data breach. Compared to 2021, when the life cycle took 287 days, this is a slight improvement.

% The ability to facilitate research into bug detection and resolution is a critical reason for developing a data-set to study PHP bugs. A large data-set can assist academics in creating new methods and instruments for finding and fixing faults in PHP code, ultimately resulting in more dependable and secure web applications. Researchers can create more precise and successful models for predicting PHP code errors if they can access a more complete and current data-set. Making a data-set will also allow researchers to examine previous PHP bug trends and characteristics. Researchers can find patterns and trends that help guide bug prevention and mitigation measures by looking at the frequency, seriousness, and types of bugs in PHP code. Researchers may update and expand this analysis to include more recent PHP versions and bug-tracking systems if they can access a large data-set. A large data-set could also make it easier to study how PHP bugs affect the security of web applications. Understanding the causes and effects of security flaws in web applications is crucial because they can result in data breaches and other serious consequences. Researchers might determine the most general categories of security vulnerabilities in PHP code and create plans to prevent and mitigate them by studying a data-set of PHP bugs. Finally, a large data-set might help academics to develop new methods for testing and validating software. Researchers could make more efficient testing methods to find and prevent PHP bugs by studying the characteristics of these bugs. 

% In conclusion, a data-set that studies PHP bugs must be created to enhance research in this area. The analysis of patterns and traits of PHP bugs over time, the investigation of the effects of PHP bugs on the security of web applications, and the development of novel methods for software testing and verification could all be facilitated by a comprehensive data-set. 

% Our benchmark will also be handy for comparing the performance of existing APR tools for PHP. This work refers to a benchmark as a collection of PHP programs and test cases used to compare the performance of different APR tools for debugging. This dataset is publicly available at \url{https://github.com/DushanPramod/bugsPHP}. So, researchers can use our work to evaluate APR tools for PHP program repair. This knowledge can be applied to educate best practices for PHP development and create new methods and tools for debugging PHP bugs. Overall this research aims to benefit the community by offering a valuable data-set for PHP bug identification and prevention, enhancing the reliability and security of PHP applications.

% \section{Introduction}

% The exciting area of research and development known as Automated Program Repair (APR) aims to automate resolving software bugs. Using program analysis~\cite{propr}, program synthesis~\cite{angelix, cpr}, evolutionary algorithms~\cite{genprog,arja} and  machine learning algorithms~\cite{jiang2021cure,lutellier2020coconut} to automatically develop patches for software bugs is the state-of-the-art in APR.
% These techniques involve evaluating the code to determine the root cause of the bug and then creating a patch that fixes the bug while preserving the original program functionality. Genetic programming, which entails developing a population of candidate patches and evolving them over several generations until a good patch is identified, is one of the most initial methods for program repair~\cite{genprog12}.
% APR has recently received a lot of attention from the software engineering community because of its potential to cut down on the expense and duration of bug fixes. %According to VentureBeat \cite{Venture_Beat}, software developers typically spend 20\% of their programming time finding and fixing bugs.

% Template-based, semantic-based, search-based, and learning-based methods are types of techniques for APR. These methods often include examining the code, finding the bug's location and root cause, then creating and implementing a fix. Search-based APR utilizes search algorithms to find and automatically correct software bugs. Template-based APR creates candidate patches for software flaws using established templates. Semantic-based APR is an approach to APR that focuses on correcting software problems by reasoning about the program's behavior and correctness using semantic analysis techniques. Learning-based techniques, which entail training models on a large corpus of code and natural language descriptions, can produce semantically meaningful patches and are understandable by humans~\cite{xia2023automated}.  CURE \cite{jiang2021cure}, is a tool that creates patches for Java programs using neural machine translation methods, is one of today's most cutting-edge APR tools. RewardRepair \cite{ye2022neural} is another recent invention that uses reinforcement learning to learn a reward function that directs the search for patches.

% Most repair tools, specifically learning-based tools, are implemented for bug repair in C, Java, Python, and JavaScript due to the dataset availability for those languages. The available datasets Defects4J \cite{just2014defects4j}, Bugs.jar \cite{bugsjar}, Bears \cite{madeiral2019bears} contain bugs for Java programs, ManyBugs, IntroClass \cite{le2015manybugs} are datasets for C language, QuixBugs \cite{lin2017quixbugs} has bugs in both Java and Python languages and for JavaScript there are BugsJS \cite{gyimesi2019bugsjs} and FixJs \cite{csuvik2022fixjs} datasets available. Surprisingly there is no suitable dataset for PHP. The unavailability of a standard dataset for PHP bugs hinders the development of APR tools for PHP program errors.

% Hypertext Preprocessor (PHP) is the web applications' most popular server-side scripting language. It was introduced in 1994 and is now powering many large-scale e-commerce applications. PHP is an open-source and general-purpose language. According to W3Techs \cite{W3Techs}, PHP is used by 77.5\% of websites as the server-side scripting language. Since the easy use of PHP, it is still among the top choices for web development. Despite its popularity, weak typing, poor performance, and lack of debugging tools cause errors in PHP web applications. However, there is little attention to applications written in PHP from the research community. A well-organized labeled PHP bugs dataset is missing to facilitate further studies of the software evolution, maintenance, and repair of PHP applications. 

% To fill the gap of unavailability of the PHP bug dataset, we propose \bugsphp,  a benchmark of 513 bugs in 15 popular open-source PHP applications based on the PHPUnit testing framework. We curate our benchmark for PHP bugs, similar to those recent work in curating benchmarks of bugs proposed and widely used for program repair tasks, such as BugsJS \cite{gyimesi2019bugsjs}, Defects4J \cite{just2014defects4j}, QuixBugs \cite{lin2017quixbugs}, and Bugs.jar \cite{bugsjar}. \bugsphp contains each bug's buggy version, fixed version, and related test cases. Further Command Line Interface (CLI) is also implemented with simple commands for users to make it easy to use. Overall this work aims to benefit the community by offering a valuable dataset for PHP bug identification and prevention, enhancing the reliability and security of PHP applications. 

% Large language models are Artificial Intelligence (AI) systems that produce human-like language using deep learning methods. These models are trained on enormous volumes of data using algorithms that enable them to recognize patterns and connections between various language components. These models can understand and analyze massive volumes of natural language data, including text, speech, and images. More recently, with the rapid development of LLMs, more active interest lies if LLMs can be used for the problem of program repair. LLMs have gained much more attention in the previous decade due to the development of computer hardware, neural networks, and the availability of vast amounts of data for training. After the release of ChatGPT, many communities get exposed to LLMs and gained benefits. Due to LLMs' Natural Language Processing (NLP) capabilities, more and more people interact with LLMs like ChatGPT. With the performance shown by ChatGPT, the community is now curious about APR using LLMs if they can be used to generate patches and do not need specific programming language-related datasets.
% Moreover, LLMs such as OpenAI Codex~\cite{codex}, AlphaCode~\cite{alphacode}, and Galactica~\cite{galactica} can be used for code generation by giving natural language descriptions. Their ability to generate code like humans motivates the community to use LLMs in APR tasks. Recent works look into the capabilities of LLMs for APR~\cite{xia_zhang_2023, Fan_Gao_Mirchev_Roychoudhury_Tan_2023}.

% Due to this gaining interest for LLMs in the community and their capabilities, we evaluated two LLMs developed by OpenAI, which are \textit{text-davinci-003} (i.e. TextDavinci) and \textit{gpt-3.5-turbo} (i.e. ChatGPT). We use two query types (query specifying buggy lines and not specifying buggy lines) and generate patches using those two queries in 3 attempts. Then run related test cases for all the patches after replacing them in related bug locations. Surprisingly TextDavinci model outperformed ChatGPT for bugs in our dataset even though ChatGPT is a new model. TextDavinci correctly fixed 5 out of 513 bugs in the benchmark, which is semantically equivalent to the developer patch.


% Mainly this paper makes the following contributions:

% \begin{itemize}
%     \item \bugsphp, a benchmark of 513 PHP bugs in 15 popular open-source projects, validated them on the PHPUnit testing framework. 
%     \item A quantitative and qualitative analysis of the types of errors in PHP applications captured in \bugsphp
%     \item Preliminary study on the effectiveness of LLMs for repairing errors in PHP applications
% \end{itemize}

% In the later sections, this paper discussed our methodology to construct the benchmark \bugsphp, a dataset representation, and the result we obtained after evaluating with LLMs.



\section{Introduction}

Manually fixing software bugs is a tedious and time-consuming task. Software engineers must invest significant time and effort in finding and fixing bugs in software programs. For example, O'Dell et al. in \cite{O'Dell2017} have mentioned that developers spend 50\% of programming time finding and fixing bugs. As a solution, Automated Program Repair (APR) has been explored to reduce the bug-fixing effort and increase developer productivity. Given the buggy program, APR tools automatically generate potential patches for software bugs. APR tools analyze the buggy program to determine the root cause and create a patch that fixes the bug while preserving the original program functionality \cite{automatic_software_repair_a_survey}. 

The current work in developing APR tools can be broadly categorized as template-based, semantic-based, search-based, and learning-based. Template-based APR tools create candidate patches for software bugs using established templates~\cite{Liu2019TBar},~\cite{FLEXIREPAIR} whereas search-based APR generates program variants that are then assessed using a fitness function on the test suite of the original program~\cite{refining_fitness_functions},~\cite{Jiang2018SimFix}. Semantic-based APR focuses on fixing bugs by reasoning about the program's behavior and correctness using semantic analysis techniques~\cite{Mechtaev2015DirectFix},~\cite{jfix}. Finally, the state-of-the-art APR tools employ learning-based techniques, which entail training machine learning models on a large corpus of code and natural language descriptions. These learning-based methods can produce patches that are semantically meaningful patches and understandable to humans~\cite{xia2023automated}. For example, CURE~\cite{jiang2021cure} creates patches for bugs in Java programs using neural machine translation, whereas RewardRepair~\cite{ye2022neural} uses reinforcement learning to learn a reward function that directs the search for correct patches.

Nevertheless, most of the existing APR tools, particularly the learning-based ones, have been implemented for bug repair in C, Java, Python, and JavaScript languages owing to the availability of large datasets for those languages. For example, datasets such as Defects4J \cite{just2014defects4j}, Bugs.jar \cite{bugsjar}, Bears \cite{madeiral2019bears} contain bugs for Java programs whereas QuixBugs \cite{lin2017quixbugs} consists of bugs in both Java and Python languages. ManyBugs and IntroClass \cite{le2015manybugs} are datasets created for C language. The datasets for JavaScript include BugsJS \cite{gyimesi2019bugsjs} and FixJs \cite{csuvik2022fixjs}. Surprisingly, despite being the most popular server-side scripting language, there is no benchmark dataset for PHP. The unavailability of a benchmark dataset for PHP bugs hinders the development of APR tools for PHP program bugs. 

PHP is an open-source and general-purpose language that powers many large-scale web applications like Facebook, Wikipedia, and WordPress. According to W3Techs \cite{W3Techs}, PHP is used by 77.5\% of websites as the server-side scripting language. Owing to the easiness of programming, PHP is still among the top choices for web development. Despite its popularity, weak typing, poor performance, and lack of debugging tools cause errors in PHP web applications. However, the research community has paid little attention to developing techniques to improve PHP programs. A well-organized labeled PHP bugs dataset must be introduced to facilitate further studies of the software evolution, maintenance, and repair of PHP applications.

Further, with the recent increased interest in Large Language Models (LLMs) like ChatGPT, exploring whether LLMs can generate patches for program bugs has attracted growing attention. LLMs are deep learning-based models trained on large amounts of text data, such as books, articles, and websites, to learn the structure and patterns of natural language. These models can generate human-like text responses to various prompts and questions. With the recent increased interest in LLMs like ChatGPT, there is a growing interest if LLMs can be used to generate patches for program bugs. Suppose LLMs can successfully generate patches for program bugs. In that case, it is a significant advancement in APR as it eliminates the need to develop programming language-specific datasets and developing APR specific complex deep learning models. Recent works look into the capabilities of LLMs for APR~\cite{xia_zhang_2023, Fan_Gao_Mirchev_Roychoudhury_Tan_2023}. Nevertheless, to the best of our knowledge, evaluating LLMs in generating patches for PHP bugs still needs to be done. 

This paper introduces a PHP bug dataset called \bugsphp that can be used to develop and evaluate APR models for PHP programs and conduct an empirical study to assess LLMs and existing APR tools on repairing PHP bugs using the introduced \bugsphp dataset. In our empirical study, we evaluate two LLMs developed by OpenAI, \textit{text-davinci-003} (i.e. TextDavinci) and \textit{gpt-3.5-turbo} (i.e. ChatGPT) and two state-of-the-art APR tools CURE~\cite{jiang2021cure} and RewardRepair~\cite{ye2022neural} on \bugsphp.

\bugsphp consists of a training dataset containing 653,606 PHP bugs from 4,483 PHP applications and a benchmark dataset containing 513 bugs from 15 PHP applications. In curating the benchmark dataset, we first select the most popular 75 GitHub Repositories based on the stargazers count and remove those that do not have developer test-suite. Next, we collect commits from 2021 Jan to 2023 March based on the commit messages from the filtered set of repositories. Following the existing work, we collect commits with a number of lines changes less than 50 and a number of file changes less than 3. Then we carry out a manual test case validation by running all the test cases on the fixed version of the program. Finally, we select the commits with at least one failing test case from its parent commit, resulting in 513 bugs from 15 PHP applications that constitute the buggy version, fixed version, and related test cases. We follow a similar subject selection and bug collection approach to curate the training dataset. Moreover, we implemented a Command Line Interface (CLI) for benchmark, including commands to checkout for buggy or fixed versions, and run only failing test cases and all the test cases. 

% how the dataset is collected
% what is in the dataset
% what can done using the provided commands


% To fill the gap of unavailability of the PHP bug dataset, we propose \bugsphp,  a benchmark of 513 bugs in 15 popular open-source PHP applications \textbf{based on the PHPUnit testing framework}. We curate our benchmark for PHP bugs, similar to those recent work in curating benchmarks of bugs proposed and widely used for program repair tasks, such as BugsJS \cite{gyimesi2019bugsjs}, Defects4J \cite{just2014defects4j}, QuixBugs \cite{lin2017quixbugs}, and Bugs.jar \cite{bugsjar}. \bugsphp contains each bug's buggy version, fixed version, and related test cases. Further Command Line Interface (CLI) is also implemented with simple commands for users to make it easy to use. Overall this work aims to benefit the community by offering a valuable dataset for PHP bug identification and prevention, enhancing the reliability and security of PHP applications. 

% Next, we conduct an empirical study to evaluate the Large Language Models (LLMs) and existing APR tools on repairing PHP bugs using the introduced \bugsphp dataset. LLMs are deep learning based models that have been trained on large amounts of text data, such as books, articles, and websites, to learn the structure and patterns of natural language.  These models can generate human-like text responses to various prompts and questions.  With the recent increased interest in LLMs like ChatGPT, there is a growing interest if LLMs can be used to generate patches for program bugs. If LLMs can successfully generate patches for program bugs then it is a huge advancement in APR as it eliminates the need to develop programming language-specific datasets and developing APR specific complex deep learning models. Recent works look into the capabilities of LLMs for APR~\cite{xia_zhang_2023, Fan_Gao_Mirchev_Roychoudhury_Tan_2023}.

To generate patches for the bugs in \bugsphp benchmark dataset using LLMs, we use two query types: query specifying buggy lines and not specifying buggy lines. The generated patches are applied to the corresponding bug locations and run related test cases. Surprisingly TextDavinci model outperformed ChatGPT for bugs in our dataset despite ChatGPT being the more advanced LLM. TextDavinci fixes 7 out of 513 bugs in \bugsphp, whereas ChatGPT fixes only four bugs for the query type I that passed all the related test cases. For the query type II TextDavinci fixes 41 bugs out of 513, while ChatGPT only fixes 19 bugs. 

% *** Describe how APR was used to generate the patches and include the results for APR tools***. 

For the final evaluation, we used two state-of-the-art APR tools, CURE and RewardRepair, to generate patches for \bugsphp benchmark. Since both the APR tools are implemented for Java bug fixing, we have trained both tools using our novel PHP training dataset. RewardRepair uses Transformer based model (T5) from Hugging Face and is trained with ten syntactic training epochs. The semantic training step was not done due to the unavailability of another PHP benchmark needed for this training process. The CURE tool consists of two models with two different architectures (CoNuT and FConv \cite{gehring2017convolutional}). Both models trained for five epochs. Evaluation for tools we generated 100 candidate patches for each bug in the benchmark using both tools and validated patches with test cases. RewardRepair showed better results than the CURE tool by generating 36 plausible patches, and 13 out of them are correct patches while CURE generate 11 plausible patches and non of them are correct patches. 

Our empirical study demonstrates that *** ***


%Large language models are Artificial Intelligence (AI) systems that produce human-like language using deep learning methods. These models are trained on enormous volumes of data using algorithms that enable them to recognize patterns and connections between various language components. These models can understand and analyze massive volumes of natural language data, including text, speech, and images. More recently, with the rapid development of LLMs, more active interest lies if LLMs can be used for the problem of program repair. LLMs have gained much more attention in the previous decade due to the development of computer hardware, neural networks, and the availability of vast amounts of data for training. After the release of ChatGPT, many communities get exposed to LLMs and gained benefits. Due to LLMs' Natural Language Processing (NLP) capabilities, more and more people interact with LLMs like ChatGPT. With the performance shown by ChatGPT, the community is now curious about APR using LLMs if they can be used to generate patches and do not need specific programming language-related datasets. Moreover, LLMs such as OpenAI Codex~\cite{codex}, AlphaCode~\cite{alphacode}, and Galactica~\cite{galactica} can be used for code generation by giving natural language descriptions. Their ability to generate code like humans motivates the community to use LLMs in APR tasks. Recent works look into the capabilities of LLMs for APR~\cite{xia_zhang_2023, Fan_Gao_Mirchev_Roychoudhury_Tan_2023}.

% Due to this gaining interest for LLMs in the community and their capabilities, we evaluated two LLMs developed by OpenAI, which are \textit{text-davinci-003} (i.e. TextDavinci) and \textit{gpt-3.5-turbo} (i.e. ChatGPT). We use two query types (query specifying buggy lines and not specifying buggy lines) and generate patches using those two queries in 3 attempts. Then run related test cases for all the patches after replacing them in related bug locations. Surprisingly TextDavinci model outperformed ChatGPT for bugs in our dataset even though ChatGPT is a new model. TextDavinci correctly fixed 5 out of 513 bugs in our dataset, which is semantically equivalent to the developer patch.


This paper makes three main contributions:

\begin{itemize}
    \item A PHP bug dataset called \bugsphp consisting of 513 PHP bugs for benchmarking and 653606 for training APR tools from popular open-source projects. % validated them on the PHPUnit testing framework. 
    \item A quantitative and qualitative analysis of the types of errors in PHP applications captured in \bugsphp
    \item An empirical evaluation of the effectiveness of LLMs and existing APR tools for repairing errors in PHP applications
\end{itemize}

% In the later sections, this paper discussed our methodology to construct the dataset of \bugsphp, a dataset representation, and the result we obtained after evaluating with LLMs.



==> sections-old/introduction_v2.tex <==
\section{Introduction}

Manually fixing software bugs is a tedious and time-consuming task. Software engineers must invest significant time and effort in finding and fixing bugs in software programs. For example, O'Dell et al. in \cite{O'Dell2017} have mentioned that developers spend 50\% of programming time finding and fixing bugs. As a solution, Automated Program Repair (APR) has been explored to reduce the bug-fixing effort and increase developer productivity. Given the buggy program, APR tools automatically generate potential patches for software bugs. APR tools analyze the buggy program to determine the root cause and create a patch that fixes the bug while preserving the original program functionality \cite{automatic_software_repair_a_survey}. 

The current work in developing APR tools can be broadly categorized as template-based, semantic-based, search-based, and learning-based. Template-based APR tools create candidate patches for software bugs using established templates~\cite{Liu2019TBar},~\cite{FLEXIREPAIR} whereas search-based APR generates program variants that are then assessed using a fitness function on the test suite of the original program~\cite{refining_fitness_functions},~\cite{Jiang2018SimFix}. Semantic-based APR focuses on fixing bugs by reasoning about the program's behavior and correctness using semantic analysis techniques~\cite{Mechtaev2015DirectFix},~\cite{jfix}. Finally, APR tools also employ learning-based techniques, which entail training machine learning models on a large corpus of code and natural language descriptions. These learning-based methods can produce patches that are semantically meaningful patches and understandable to humans~\cite{xia2023automated}. For example, CURE~\cite{jiang2021cure} creates patches for bugs in Java programs using neural machine translation, whereas RewardRepair~\cite{ye2022neural} uses reinforcement learning to learn a reward function that directs the search for correct patches.

Nevertheless, most of the existing APR tools, particularly the learning-based ones, have been implemented for bug repair in C, Java, Python, and JavaScript languages owing to the availability of large datasets for those languages. For example, datasets such as Defects4J \cite{just2014defects4j}, Bugs.jar \cite{bugsjar}, Bears \cite{madeiral2019bears} contain bugs for Java programs whereas QuixBugs \cite{lin2017quixbugs} consists of bugs in both Java and Python languages. ManyBugs and IntroClass \cite{le2015manybugs} are datasets created for C language. The datasets for JavaScript include BugsJS \cite{gyimesi2019bugsjs} and FixJs \cite{csuvik2022fixjs}. Surprisingly, despite being the most popular server-side scripting language, there is no benchmark dataset for PHP. The unavailability of a benchmark dataset for PHP bugs hinders the development of APR tools for PHP program bugs. 

PHP is an open-source and general-purpose language that powers many large-scale web applications like Facebook, Wikipedia, and WordPress. According to W3Techs \cite{W3Techs}, PHP is used by 77.5\% of websites as the server-side scripting language. Owing to the easiness of programming, PHP is still among the top choices for web development. Despite its popularity, weak typing, poor performance, and lack of debugging tools cause errors in PHP web applications. However, the research community has paid little attention to developing techniques to improve PHP programs. A well-organized labeled PHP bugs dataset must be introduced to facilitate further studies of the software evolution, maintenance, and repair of PHP applications.

Further, with the recent increased interest in Large Language Models (LLMs) like ChatGPT, exploring whether LLMs can generate patches for program bugs has attracted growing attention. LLMs are deep learning-based models trained on large amounts of text data, such as books, articles, and websites, to learn the structure and patterns of natural language. These models can generate human-like text responses to various prompts and questions. With the recent increased interest in LLMs like ChatGPT, there is a growing interest if LLMs can be used to generate patches for program bugs. Suppose LLMs can successfully generate patches for program bugs. In that case, it is a significant advancement in APR as it eliminates the need to develop programming language-specific datasets and developing APR specific complex deep learning models. Recent works look into the capabilities of LLMs for APR~\cite{xia_zhang_2023, Fan_Gao_Mirchev_Roychoudhury_Tan_2023}. Nevertheless, to the best of our knowledge, evaluating LLMs in generating patches for PHP bugs still needs to be done. 

This paper introduces a PHP bug dataset called \bugsphp that can be used to develop and evaluate APR models for PHP programs and conduct an empirical study to assess LLMs and existing APR tools on repairing PHP bugs using the introduced \bugsphp dataset. In our empirical study, we evaluate two LLMs developed by OpenAI, \textit{text-davinci-003} (i.e. TextDavinci) and \textit{gpt-3.5-turbo} (i.e. ChatGPT) and two state-of-the-art APR tools CURE~\cite{jiang2021cure} and RewardRepair~\cite{ye2022neural} on \bugsphp.

\bugsphp consists of a training dataset containing 653,606 PHP bugs from 4,483 PHP applications and a test dataset containing 513 bugs from 15 PHP applications. In curating the test dataset, we first select the most popular 75 GitHub Repositories based on the stargazers count and remove those that do not have developer test-suite. Next, we collect commits from 01 Jan 2020 to Mar 2023 based on the commit messages from the filtered set of repositories. Following the existing work, we collect commits with a number of lines changes less than 50 and a number of file changes less than 3. Then we carry out a manual test case validation by running all the test cases on the fixed version of the program. Finally, we select the commits with at least one failing test case from its parent commit, resulting in 513 bugs from 15 PHP applications that constitute the buggy version, fixed version, and related test cases. We follow a similar subject selection and bug collection approach to curate the training dataset. %Moreover, we implemented a Command Line Interface (CLI) for test dataset, including commands to checkout for buggy or fixed versions, and run only failing test cases and all the test cases.

% Next, we conduct an empirical study to evaluate the effectiveness of LLMs and existing APR tools in repairing PHP bugs using the \bugsphp dataset. We used TextDavinci and ChatGPT to generate patches for the bugs in the test dataset. Two query types were used: one specifying buggy lines and one not specifying buggy lines. The generated patches were then applied to the corresponding bug locations and tested. Surprisingly, the TextDavinci model performed better than ChatGPT, despite ChatGPT being the more advanced LLM. For instance, TextDavinci correctly fixed 41 bugs out of 513 bugs in our dataset, while ChatGPT only fixed 19 bugs.

Next, we conduct an empirical study to evaluate the effectiveness of LLMs and existing APR tools in repairing PHP bugs using the \bugsphp dataset. We used TextDavinci and ChatGPT to generate patches for the bugs in the test dataset. Two query types were used: one specifying buggy lines and one not specifying buggy lines. The generated patches were then applied to the corresponding bug locations and tested. Finally, we utilize two recent learning-based APR tools, CURE~\cite{jiang2021cure} and RewardRepair~\cite{ye2022neural}, to generate patches for the bugs in the \bugsphp test dataset. However, since these tools have been evaluated using bugs in Java programs, we trained them using our newly curated dataset of PHP bugs. We tested the tools by generating 100 candidate patches for each bug through both tools and verified them using developer-provided test cases.

% *** Describe how APR was used to generate the patches and include the results for APR tools***. 

% For the final evaluation, we used two state-of-the-art APR tools, CURE and RewardRepair, to generate patches for \bugsphp benchmark. Since both the APR tools are implemented for Java bug fixing, we have trained both tools using our novel PHP training dataset. RewardRepair uses Transformer based model (T5) from Hugging Face and is trained with ten syntactic training epochs. The semantic training step was not done due to the unavailability of another PHP benchmark needed for this training process. The CURE tool consists of two models with two different architectures (CoNuT and FConv \cite{gehring2017convolutional}). Both models trained for five epochs. Evaluation for tools we generated 100 candidate patches for each bug in the benchmark using both tools and validated patches with test cases. RewardRepair showed better results than the CURE tool by generating 36 plausible patches, and 13 out of them are correct patches while CURE generate 11 plausible patches and non of them are correct patches. 

% Finally, we utilize two recent learning-based APR tools, CURE~\cite{jiang2021cure} and RewardRepair~\cite{ye2022neural}, to generate patches for the bugs in the \bugsphp test dataset. However, since these tools have been evaluated using bugs in Java programs, we trained them using our newly curated dataset of PHP bugs. We tested the tools by generating 100 candidate patches for each bug through both tools and verified them using developer-provided test cases. RewardRepair outperforms CURE by generating 36 plausible patches, of which seven were correct. On the other hand, CURE produces only 11 plausible patches, of which one was correct.

Our empirical study demonstrates that TextDavinci outperforms ChatGPT in repairing PHP bugs, despite ChatGPT being the more advanced LLM. For instance, TextDavinci correctly fixes 41 bugs out of 513 in our dataset, while ChatGPT only fixes 19 bugs. Considering APR tools, RewardRepair performs significantly better than CURE. RewardRepair can generate 36 plausible patches, but CURE can produce only 11. When comparing LLMs and APR tools, the RewardRepair model has comparative performances with the TextDavinci model in generating high-quality patches for PHP bugs in \bugsphp.

% Our empirical study demonstrates that TextDavinci performs significantly better than ChatGPT for PHP bugs. TextDavinci could generate more plausible patches than ChatGPT. In the best-performing round in query type II, TextDavinci was able to generate 30 plausible patches, but ChatGPT could generate 14 plausible patches. almost 2 times better results in the TextDavinci. Considering APR tools, RewardRepair performs significantly better than CURE. RewardRepair could generate 36 plausible patches, but CURE could generate 11 plausible patches, almost 3 times better results in RewardRepair than CURE. comparing LLM and APR tools. RewardRepair is the best-performing tool for PHP bugs.


%Large language models are Artificial Intelligence (AI) systems that produce human-like language using deep learning methods. These models are trained on enormous volumes of data using algorithms that enable them to recognize patterns and connections between various language components. These models can understand and analyze massive volumes of natural language data, including text, speech, and images. More recently, with the rapid development of LLMs, more active interest lies if LLMs can be used for the problem of program repair. LLMs have gained much more attention in the previous decade due to the development of computer hardware, neural networks, and the availability of vast amounts of data for training. After the release of ChatGPT, many communities get exposed to LLMs and gained benefits. Due to LLMs' Natural Language Processing (NLP) capabilities, more and more people interact with LLMs like ChatGPT. With the performance shown by ChatGPT, the community is now curious about APR using LLMs if they can be used to generate patches and do not need specific programming language-related datasets. Moreover, LLMs such as OpenAI Codex~\cite{codex}, AlphaCode~\cite{alphacode}, and Galactica~\cite{galactica} can be used for code generation by giving natural language descriptions. Their ability to generate code like humans motivates the community to use LLMs in APR tasks. Recent works look into the capabilities of LLMs for APR~\cite{xia_zhang_2023, Fan_Gao_Mirchev_Roychoudhury_Tan_2023}.

% Due to this gaining interest for LLMs in the community and their capabilities, we evaluated two LLMs developed by OpenAI, which are \textit{text-davinci-003} (i.e. TextDavinci) and \textit{gpt-3.5-turbo} (i.e. ChatGPT). We use two query types (query specifying buggy lines and not specifying buggy lines) and generate patches using those two queries in 3 attempts. Then run related test cases for all the patches after replacing them in related bug locations. Surprisingly TextDavinci model outperformed ChatGPT for bugs in our dataset even though ChatGPT is a new model. TextDavinci correctly fixed 5 out of 513 bugs in our dataset, which is semantically equivalent to the developer patch.


This paper makes three main contributions:

\begin{itemize}
    \item A PHP bug dataset called \bugsphp consisting of 513 PHP bugs for testing and 653606 for training APR tools from popular open-source projects. % validated them on the PHPUnit testing framework. 
    \item A quantitative and qualitative analysis of the types of errors in PHP applications captured in \bugsphp
    \item An empirical evaluation of the effectiveness of LLMs and existing APR tools for repairing errors in PHP applications
\end{itemize}

% In the later sections, this paper discussed our methodology to construct the dataset of \bugsphp, a dataset representation, and the result we obtained after evaluating with LLMs.



==> sections-old/motivation.tex <==
\section{Motivation}
% Over 77\% of all websites utilize PHP, making it a popular programming language for web development \cite{W3Techs}. PHP is susceptible to bugs, just like any other piece of software. Bugs can range from trivial problems to significant security flaws that could harm users and companies that depend on web apps. Thus, it is imperative to investigate the types of bugs for PHP applications.
% The stability and security of web applications are significant reasons to examine PHP bugs. These bugs can have severe consequences, ranging from data loss to illegal access by intruders. The most common way for attackers to access data without authorization is through web application vulnerabilities. Researchers can discover prevalent problems and create plans to avoid or mitigate them by systematically investigating bugs in PHP applications, ultimately increasing web applications' stability and security. Analyzing PHP bugs also aims to boost software development's effectiveness and efficiency. Bug fixes can take a long time, cost money, and postpone the introduction of new features or products. Developers can save time and money and concentrate on making better software by understanding the causes of PHP bugs and implementing tools and approaches for finding and fixing them. %Research into PHP bugs has the potential to be significant for educational purposes. %Teachers can teach students the value of testing and debugging and the need for excellent coding methods and attention to detail by examining real-world instances of PHP errors and their causes. 

% Since PHP is the most used server-side language, world-famous web applications such as Facebook, Wikipedia, Tumblr, Slack, MailChimp, Etsy, and WordPress also use PHP. Facebook has 2.9 billion worldwide users \cite{Facebook_stats}, Wikipedia has around five billion visits in the first five months of 2022 \cite{Wikipedia_stats}, Tumblr has 547 million monthly users \cite{Tumblr_stats}, Slack is predictive to have 32.3 million monthly users in 2023 \cite{Slack_stats}, Etsy have 94 million active buyers and 7.3 million sellers \cite{Etsy_stats} and 810 million websites created using WordPress which is the 43\% of all the websites in internet \cite{wordpress_stats}. According to those statistics, PHP is used to build web applications that most internet users interact with, and bugs in those PHP web applications can affect billions of users. 

% The Open Web Application Security Project is known as OWASP\footnote{https://owasp.org}. It is a global non-profit organization that prioritizes enhancing software security. Every three years, the nonprofit organization updates a list of the top 10 web application security vulnerabilities and offers advice on reducing such risks. The 2021 edition of OWASP top-10 list ``Broken Access Control'' as the most prevalent type of vulnerabilities in web applications~\cite{owsap_top_10}.

% The following vulnerabilities are listed in the 2021 edition of the OWASP Top 10 \cite{owsap_top_10}.

% \vspace{5mm}
% \begin{itemize}
%     \item A01 - Broken Access Control
%     \item A02 - Cryptographic Failures
%     \item A03 - Injection
%     \item A04 - Insecure Design
%     \item A05 - Security Misconfiguration
%     \item A06 - Vulnerable and Outdated Components
%     \item A07 - Identification and Authentication Failures
%     \item A08 - Software and Data Integrity Failures
%     \item A09 - Security Logging and Monitoring Failures
%     \item A10 - Server-Side Request Forgery
% \end{itemize}

% \vspace{5mm}
% Broken Access Control vulnerabilities are the most prevalent and dangerous web-based application vulnerabilities, according to the OWASP Top 10 list. 

% Web application vulnerabilities can have a significant impact and expense. For instance, the 2017 Equifax data breach \cite{equifax_data_breach} cost the company \$700 million in expenses and lost revenue due to a flaw in the company's web application and affected nearly 150 million clients, about 56\% of Americans. For web applications, PHP is a popular server-side programming language. PHP is not intrinsically insecure, although poorly written PHP code can make web applications more vulnerable. For instance, inappropriate database function use in PHP can result in injection issues. It's critical to adhere to secure coding best practices, uses secure frameworks and libraries, and frequently test and scan web applications for vulnerabilities to prevent web application vulnerabilities. Eighty-seven million records of US resident profiles were obtained through Facebook as the most significant data breaches on online social networks as of 2020, and the data was used to create software that could predict and influence electors \cite{online_social_networks_security_and_privacy}. Another primary photo-sharing website, Flickr (owned by Yahoo Inc.), has experienced severe vulnerabilities \cite{flickr_vulnerable}. The SQL injection vulnerability on the Flickr website was discovered by Egyptian security researcher Ibrahim Raafat. Raafat asserts that he has discovered three susceptible parameters: two for blind SQL injection (page\_id and items) and one for direct SQL injection (Order\_id). The attacker can read the Flickr database thanks to this flaw. By inserting the SQL query, effective SQL exploitation can also give attackers access to databases and MySQL login credentials. Raafat demonstrates how the vulnerability enables him to submit a unique "code execution shell" by writing new files on the server.

% Understanding the size and scope of the issue is a crucial driver for researching the effects of PHP bugs on the present software landscape. While many PHP errors are minor and have little impact on users, others can have severe consequences. Researchers can identify the most critical problems and create mitigation plans by researching how PHP vulnerabilities have affected the present software landscape. Additionally, studying the effects of PHP bugs can aid companies and organizations in comprehending the dangers and expenses related to web application development. Researchers can determine the most frequent causes of defects and create preventative measures by examining the effects of PHP problems on the state of the software industry. The danger of data breaches and other security incidents, which may be expensive and destructive to a company's brand, can be decreased. According to an IBM report from 2022, \cite{IBM_data_breach_2022}, the average cost of a data breach is \$4.35 million, and it takes 277 days to find and stop a breach. According to IBM research, more than three-quarters of a year is required to detect and contain a data breach. Compared to 2021, when the life cycle took 287 days, this is a slight improvement.

% The ability to facilitate research into bug detection and resolution is a critical reason for developing a dataset to study PHP bugs. A large dataset can assist academics in creating new methods and instruments for finding and fixing faults in PHP code, ultimately resulting in more dependable and secure web applications. Researchers can create more precise and successful models for predicting PHP code errors if they can access a more complete and current dataset. Making a dataset will also allow researchers to examine previous PHP bug trends and characteristics. Researchers can find patterns and trends that help guide bug prevention and mitigation measures by looking at the frequency, seriousness, and types of bugs in PHP code. Researchers may update and expand this analysis to include more recent PHP versions and bug-tracking systems if they can access a large dataset. A large dataset could also make it easier to study how PHP bugs affect the security of web applications. Understanding the causes and effects of security flaws in web applications is crucial because they can result in data breaches and other serious consequences. Researchers might determine the most general categories of security vulnerabilities in PHP code and create plans to prevent and mitigate them by studying a dataset of PHP bugs. Finally, a large dataset might help academics to develop new methods for testing and validating software. Researchers could make more efficient testing methods to find and prevent PHP bugs by studying the characteristics of these bugs. 

% In conclusion, a dataset that studies PHP bugs must be created to enhance research in this area. The analysis of patterns and traits of PHP bugs over time, the investigation of the effects of PHP bugs on the security of web applications, and the development of novel methods for software testing and verification could all be facilitated by a comprehensive dataset. 

% In order to study the types of bugs in PHP applications, and to understand the nature of the fixes required to fix these bugs, there is a need for a standard data-set. In this work, we aim to fill this gap by curating a list of PHP bugs from most popular open-source PHP applications. Researchers can use our work to evaluate program repair tools for PHP applications. Furthermore, this data-set can be applied to identify insecure code, detect code-smells and create new methods and tools for debugging PHP bugs. Overall this research aims to benefit the community by offering a valuable dataset for PHP bug identification and prevention, enhancing the reliability and security of PHP applications.


% Revised by Sandareka

PHP is the most popular server-side language used by major web applications, including Facebook, Wikipedia, Tumblr, Slack, MailChimp, Etsy, and WordPress. Facebook alone boasts 2.9 billion users globally, while Wikipedia has received around 5 billion visits in the first 5 months of 2022. Slack is expected to have 32.3 million monthly users by 2023, and WordPress has been used to create 810 million websites, accounting for 43\% of all websites. 

However, like any other software, PHP programs can have bugs ranging from minor issues to major security flaws. These bugs can lead to severe problems such as data loss or unauthorized access by attackers who exploit vulnerabilities in web applications. For instance, the 2017 Equifax data breach \cite{equifax_data_breach} cost the company \$700 million in expenses and lost revenue due to a flaw in the company's web application and affected nearly 150 million clients, about 56\% of Americans. 87 million records of US resident profiles were obtained through Facebook as the most significant data breaches on online social networks as of 2020, and the data was used to create software that could predict and influence electors \cite{online_social_networks_security_and_privacy}.

Since PHP is used to build web applications that are relied upon by billions of internet users, any bugs or issues in PHP web applications can significantly impact many users. Therefore, it is vital to investigate bugs that may occur in PHP applications. By analyzing these bugs, we can improve the stability and security of web applications and increase the effectiveness and efficiency of software development. In addition, studying PHP vulnerabilities can help identify critical issues, develop effective mitigation plans, and prevent costly data breaches and security incidents that damage a company's reputation.

Nevertheless, manually fixing program bugs can be costly and time-consuming, causing delays in releasing new features or products. To save resources and time, developers can use efficient tools and methods to identify and resolve these issues, enabling them to focus on creating high-quality software. To better understand the nature of bugs in PHP applications, there is a need for a standard dataset to study the different types of bugs and their required fixes. Additionally, a comprehensive dataset can facilitate the analysis of patterns and traits of PHP bugs over time, investigating their effects on web application security and developing innovative software testing and verification methods.

This work aims to fill this gap by curating a list of PHP bugs from the most popular open-source PHP applications. Researchers can use our work to evaluate program repair tools for PHP applications. Furthermore, this dataset can be applied to identify insecure code, detect code smells and create new methods and tools for debugging PHP bugs. Overall this research aims to benefit the community by offering a valuable dataset for PHP bug identification and prevention, enhancing the reliability and security of PHP applications.


==> sections-old/related.tex <==
\section{Related Work}

% RunBugRun \cite{prenner_robbes_2023} paper presents a fully executable dataset of 450,000 small buggy/fixed program pairs retrieved from a Project CodeNet (An extensive collection of programming contest submissions mined from two online judge websites AIZU and AtCoder) written in eight different programming languages (C, C++, Java, Python, JavaScript, Ruby, Go, PHP). All the bugs in the RunBugRun dataset come with test cases. They remove all the submissions written in other languages. Then they group rejected and accepted submissions belonging to the same user and the same problem and tokenize those submissions and calculate token level difference using an LCS-based diffing algorithm. Consider rejected and accepted submissions as corresponding buggy and fixed submissions if their token-level difference is less than six. Since CodeNet does not contain the test cases, researchers use a script to extract input/output pairs from the problem descriptions and get more test cases from another dataset, finally using a semi-automatic process to generate further test cases. Then they filter out all pairs (rejected and accepted submissions) and remove them if they contain syntax errors. Also used pre-processing step to convert submissions written in Python 2 converted to Python 3 using code translation. Execute all the submissions on all test cases related to a problem and further filter out and remove pairs if rejected submission passed all related test cases or time out any test case and accepted submission failed or time out a test case. Later they evaluated the dataset with two baselines and provided some statistical information. 

% Defects4J \cite{just2014defects4j} introduces an expandable framework and database that provides genuine software bugs for reproducible research in software testing. The database's initial version includes 357 bugs from five open-source programs. Each bug contains a comprehensive test suite capable of revealing the bug. It allows new bugs to be added to the database with little or no effort once a program has been configured. Defects4J also includes a framework for accessing faulty and fixed program versions and their corresponding test suites and a high-level interface for conducting research in software testing.

% Bugs.jar \cite{bugsjar} was introduced as a sizable collection for researching automated Java program debugging, testing, and patching. This data set includes 1,158 bugs and patches from 8 open-source Java projects, representing eight distinct and significant application categories.

% BEARS \cite{madeiral2019bears} introduced a project focused on gathering and storing bugs to create a flexible benchmark for automatic repair studies in Java. The bug collection relies on building states from Continuous Integration (CI) to identify potential pairs of the buggy and patched program versions from open-source projects on GitHub. The program versions then undergo a pipeline that attempts to reproduce the bug and its corresponding patch. The pipeline includes the execution of the program's test suite on both versions. If a test failure is identified in the buggy version and not in the patched version, the bug, and its patch are considered successfully reproduced. BEARS is designed to be publicly accessible and extendable, enabling researchers to create branches with bugs in a GitHub repository, which can then be used for pull requests in the BEARS repository. Version 1.0 includes 251 reproducible bugs from 72 projects that use the Travis CI and Maven build environment.

% MANYBUGS and INTROCLASS \cite{le2015manybugs} contains 1,183 defects across 15 C programs. Datasets are intended to aid in evaluating automatic repair algorithms and are accompanied by reproducibility and benchmark quality guarantees. ManyBugs consists of bugs from large popular open-source projects. IntroClass consists of bugs from programming assignments written by a small group of students. Each study object is categorized to allow for qualitative evaluation and comparisons based on bug or program category. Also, the paper provides experimental results for three repair methods, GenProg, AE, and TrpAutoRepair.

% BUGSJS \cite{gyimesi2019bugsjs} introduces 453 actual JavaScript bugs that have been manually validated. These bugs are from 10 popular server-side JavaScript programs, totaling 444k Lines of Code (LOC). Each bug has its corresponding report, test cases, and patch. BUGSJS has an extensive CLI that allows for easy access to the faulty and fixed versions of the programs, as well as the execution of the corresponding test cases.

% FixJS \cite{csuvik2022fixjs} is a dataset that includes bugs in Javascript functions. The data was collected from GitHub and had information on the faulty and fixed versions of the same program. The dataset contains over 300,000 samples, including details on the commit, the before/after states, and three source code representations.

% Table~\ref{tab:list-of-bug-datasets} included a list of existing bug datasets. According to our literature survey, most datasets  focus on C, Java, Python, and JavaScript bugs. There was no PHP bug dataset.

The existing work in analyzing program bugs has curated datasets focused on Java, C, Python, and JavaScript bugs. For example, Defects4J\cite{just2014defects4j} is a framework and database that offers genuine Java program bugs for reproducible research in software testing. It has 357 bugs from five open-source programs, each with a complete test suite that exposes the bug. It's expandable, and new bugs can be easily added to the database once a program is set up. Defects4J also includes a framework to access faulty and fixed program versions, their corresponding test suites, and a user-friendly interface for research in software testing. 

The Bugs.jar \cite{bugsjar} is an extensive data collection useful for researching automated Java program debugging, testing, and patching. It contains 1,158 bugs and patches from 8 open-source Java projects, representing eight important application categories.

BEARS is a project that creates a flexible benchmark for automatic repair studies in Java. It collects and stores bugs by identifying potential pairs of faulty and fixed program versions from open-source projects on GitHub. BEARS is publicly accessible and includes 251 reproducible bugs from 72 projects that use the Travis CI and Maven build environment.

The MANYBUGS and INTROCLASS datasets \cite{le2015manybugs} comprise 1,183 defects found in 15 C programs. These datasets help evaluate automatic repair algorithms and come with reproducibility and benchmark quality guarantees. ManyBugs contains bugs from well-known open-source projects, while IntroClass contains bugs from programming assignments done by a small group of students. The paper also presents experimental results for three repair methods: GenProg, AE, and TrpAutoRepair.

The datasets BUGSJS \cite{gyimesi2019bugsjs} and FixJS \cite{csuvik2022fixjs} are collections of JavaScript bugs. BUGSJS features 453 actual bugs that have been verified manually. These bugs are taken from 10 widely used server-side JavaScript programs, which collectively have 444,000 lines of code. Each bug comes with a report, test cases, and patch. BUGSJS also includes a user-friendly CLI that lets users conveniently access the faulty and fixed versions of the programs and execute the associated test cases. FixJS, on the other hand, gathers bugs from GitHub and provides information on the faulty and fixed versions of the same program. This dataset comprises over 300,000 samples and includes details on the commit, before/after states, and three source code representations.

Recently, Julian Aron Prenner et al. in \cite{prenner_robbes_2023}  present RunBugRun, a fully executable dataset of 450,000 small buggy/fixed program pairs originally submitted to programming competition websites written in eight different programming languages, namely C, C++, Java, Python, JavaScript, Ruby, Go and PHP. All the bugs in the RunBugRun dataset come with test cases. Further, the authors evaluate the dataset with two baselines and provide some statistical information. 

Table~\ref{tab:list-of-bug-datasets} shows a list of existing bug datasets. The Table indicates that most existing datasets focus on C, Java, Python, and JavaScript bugs, and a bug dataset for PHP programs has not been introduced. 

\begin{table}[!htb]
\centering
\caption{Bug dataset for different languages}
\begin{tabular}{|l|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{Tool} & C & Java & Python & JavaScript \\ \hline
Defects4J \cite{just2014defects4j}                 &   & \checkmark    &        &  \\ \hline
QuixBugs \cite{lin2017quixbugs}                  &   & \checkmark    & \checkmark      &    \\ \hline
BugsJS \cite{gyimesi2019bugsjs}                    &   &      &        & \checkmark  \\ \hline
ManyBugs, IntroClass \cite{le2015manybugs}      & \checkmark &      &        &    \\ \hline
Bugs.jar \cite{bugsjar}                  &   & \checkmark    &        &     \\ \hline
Bears \cite{madeiral2019bears}                     &   & \checkmark    &        &     \\ \hline
FixJs  \cite{csuvik2022fixjs}  &   &      &        & \checkmark   \\ \hline
\end{tabular}

\label{tab:list-of-bug-datasets}
\end{table}

% \noindent In addition to bug datasets, there are program repair tools, 

% RewardRepair \cite{ye2022neural} is a new repair model built on a mix of syntactic and semantic training objectives. This model combines semantic training based on program execution with token-level syntactic training. Researchers use program compilation and test execution-based loss functions to improve Neural Machine Translation (NMT)-based program repair. They use discriminators to compile and run test cases to generate patches and provide high-quality feedback about patch quality. The neural network weight is updated according to feedback. RewardRepair has three stages: syntactic training, semantic training, and inference. CoCoNuT \cite{lutellier2020coconut}, MegaDiff \cite{monperrus2021megadiff}, and CodeRep \cite{chen2018codrep} datasets are used for syntactic training since they only have buggy and patch codes. They used the Bears \cite{madeiral2019bears} dataset in semantic training since it has compiler configuration and test cases. For semantic training, they use four discriminative models: difference discriminator, compilability discriminator, plausibility discriminator, and regression discriminator executed serially to check patch quality.

% \begin{itemize}
%     \item Difference discriminator – This discriminator gives a penalty score if there is no change between buggy and fixed codes.
%     \item Compilability discriminator – use a compiler to check whether the patch is compilable. If compilable, assign a compilable reward.
%     \item Plausibility discriminator - Check whether patches pass human written test cases. If passed, a plausible reward is assigned.
%     \item Regression discriminator – This discriminator reduces the patches' behavioral changes.
% \end{itemize}

% Towards JavaScript program repair with Generative Pre-trained Transformer (GPT-2) \cite{lajko2022towards} paper, use a pre-trained transformer model called Generative Pre-trained Transformer (GPT)-2 on JavaScript bug fixing. It's an NLP model. It used the BugJs dataset to fine-tune and evaluate.  It shows overall accuracy of 17.25\%.

% SequenceR \cite{chen2019sequencer} paper introduces a program repair approach called sequence-to-sequence learning based on NMT. Focus on one-line bug fixing on Java programs. Used OpenNMT-py framework to build the model and evaluate on Defects4J benchmark. It generates 61 plausible and 18 identical patches for a human developer out of 75 one-line bugs.

% BIFI \cite{yasunaga2021break} is an unsupervised APR approach using unlabeled data to learn the bug fixer. It has two parts. Fixer, which can fix the buggy code, and breaker, which can break the good code and create a buggy code. The idea of BIFI is to apply the fixer to real bad codes and add the resulting fixed output to the training data. Then train the breaker those resulting paired data. Then generate the code errors using the breaker and train the fixer for those newly generated paired data. This cycle iterates multiple times, improving the fixer and breaker. If the training dataset is small, this method will become more effective.

% CURE \cite{jiang2021cure} is a new NMT-based APR technique with three significant improvements. The Pre-trained Programming language (PL) model is trained to predict the subsequent tokens in code sequences and learns to generate developer-like code. The code-aware beam-search strategy did more correct fixes by inducing more compilable patches and similar lengths to the buggy line. CURE used the byte-pair encoding sub-word tokenization technique to tokenize compound and rare words to address the Out of Vocabulary (OOV) problem.  Training data gathered from open-source java projects and CoCoNuT \cite{lutellier2020coconut} training data shared on GitHub. CURE uses word-level tokenization to separate code lines by spaces, camel case letters, underscores, strings, and numbers. Next, applying sub-word tokenization made better search space with more correct patches. CURE consists of two models, the PL model(GPT) and the CoCoNuT \cite{lutellier2020coconut}. CURE fixes 57 bugs in  the Defects4J \cite{just2014defects4j} and 26 in the QuixBugs \cite{lin2017quixbugs} benchmarks. Also, it fixes unique bugs in those two benchmarks. Fixes 13 more bugs in Defects4J compared to CoCoNuT \cite{lutellier2020coconut}.

% TFix \cite{berabi2021tfix} is a method that builds using a pre-trained text-to-text transformer called T5. This method fixes coding errors as a text-to-text prediction. When given a coding mistake as a text, TFix predicts a new text representation. They selected the T5 pre-trained model and then trained it to fine-tune it for code fixing. Identifying the code errors needs an error detector. Here they used ESlint since the target language is JavaScript. The error detector gives the error details. Using those error details, TFix creates a single piece of text to query the machine-learning model.

% DLFix \cite{li2020dlfix} contains two layers of Deep Learning (DL) models. A tree-based Recurrent Neural Network (RNN) serves as the first layer, which learns the context of bug fixes, and its result gives additional weighting as input for the second layer. And the second layer is used to learn the bug-fixing code transformation. The approach of DLFix is as follows,

% \begin{itemize}
%     \item Pre-processing – DLFix renames variables within a method of a project using Word2Vec on the sequence of code tokens to get their vector representation.
%     \item Context learning – The first layer of the two-layer learning model is dedicated to learning the context of the code fixes. Replace changes to the sub-tree with a summarized node. Unchanged Abstract Syntax Tree (AST) nodes from fix use as the context of the code fix.
%     \item Code transformation learning – Changed sub-tree before and after code fixes used to train the second layer(Transformation learning layer) to learn bug-fixing code transformation.
%     \item Program analysis filtering – Program analysis filter to check existence variables, methods, and class names to convert the keyword back to the right name.
%     \item Patch re-ranking - Given a list of candidate patches containing the ground-truth patch for a bug, build a Convolutional Neural Network (CNN) based binary classification approach and train it using the ground-truth patch as one positive example and the rest of the candidate patches as negative ones.
% \end{itemize}

% CoCoNuT \cite{lutellier2020coconut} APR tool is a Generate and Validate (G\&V) technique that combines CNN with new context-aware NMT architecture by using ensemble learning to overcome challenges and limitations in existing APR techniques. When using the G\&V method for APR, considerable human effort must be customized to work in different languages. The paper claimed that by using NMT, we could overcome those challenges. Also, NMT has challenges in context representing and capturing the diversity of bug fixes. Using context-aware NMT architecture and the advantage of hyperparameter tuning to build multiple models and use ensemble learning to combine models will help us overcome those challenges. It evaluated the CoCoNuT tool on six benchmarks in four programming languages (JavaScript, Java, C, Python). It could correctly fix 509 bugs, and 309 of them were never fixed by any of the existing tools.

% DrRepair \cite{yasunaga2020graph} introduces a novel APR approach using a program feedback graph, which connects symbols relevant to program repair in source code and diagnostic feedback and then applies a graph neural network on top to model the reasoning process—focused on C program compilation bug fixing.

% Automated Program Repair \cite{goues2019automated} In this paper, researchers discuss four practical use cases of APR. They were fixing bugs throughout development, repairing security vulnerabilities, intelligent tutoring, and self-healing of performance bottlenecks. An automated repair can provide hints for the programming assignments and can do the grading for those by comparing with the model solution, which is known as intelligent tutoring. Drones may encounter unexpected inputs because of the varying physical environment, which may cause to drain the battery. So automated repair can provide self-healing for that system. There are two central repairs, heuristic and constrained-based repair. There are some challenges in program repair. Need to ensure and develop quality repair, increase the scope of the problems that will be repaired, and integrate that repair into development.

% Automatic repair of OWASP Top 10 security vulnerabilities: A survey \cite{marchand2020automatic} This paper gives a survey report about existing security vulnerability repairing tools. In this paper, the authors classify existing APR methods according to which The Open Web Application Security Project (OWASP) top 10 categories they cover. Further, they analyze the two Java test suites (Juliet and VAKB -Vulnerability Assessment Knowledge Base) to analyze their coverage of OWASP top 10.

% Empirical Review of Java Program Repair Tools \cite{durieux2019empirical} There are 11 Java repair tools, 2141 bugs from 5 benchmarks, and 23,551 repair attempts performed in this study. Selected benchmarks contain Java language bugs, are peer-reviewed, and include at least one failing test case. They created an execution framework name “RepairThemAll” to run those repair tools with benchmarks. Defects4J \cite{just2014defects4j} benchmark patches the highest number of unique bugs, and repair tools over-fit Defects4J. Bugs.jar \cite{saha2018bugs} is the most non-patch generation benchmark. Repair tools need 13.5 minutes of average time to generate a patch, much smaller than the allocated budget(2 hours). Finally, this paper mainly introduces the benchmark over-fitting problem and the non-patch generation.

% Obstacles in Fully Automatic Program Repair: A survey \cite{mousavi2020obstacles} This paper reviews fully automatic program repair using the diffraction method. The authors discussed achieving “full automation” and the obstacles to achieving it, and the majorly concerned obstacle in this paper is overfitting. This paper discussed semantics- and heuristic-based, two automatic software repair techniques branches.

% RSRepair \cite{qi2014strength} is an APR tool based on a random search. RSRepair uses the same implementation function for fault localization and mutation in GenProg \cite{le2011genprog} and improves it. Improvements are GenProg has to run a fixed size of test cases for every candidate patch. But RSRepair immediately discards one candidate patch that failed to pass some test cases. In addition, to speed up the invalid patch identification process, they implemented a test case prioritization technique.

% Summary of A Critical Review of “Automatic Patch Generation Learned from Human-Written Patches” \cite{monperrus2014critical} is a survey paper by Martin Monperrus. In this paper, he gives a critical review of a paper that was published about the PAR approach. It is a template-based approach for fixing bugs in Java codes. Those templates typically fix common problems. In this paper, the authors explain vital factors they disagree with mentioned in the PAR paper and later give some essential ideas behind automatic software repair.

% Automated Repair of HTML Generation Errors in PHP Applications Using String Constraint Solving \cite{samimi2012automated}: This paper introduces two PHP and HTML error repairing tools in PHP applications. One is PHPQuickFix: which fixes simple bugs by statically analyzing individual prints. Another one is PHPRepair: which handles more general repairs using a dynamic approach. Based on a test suite. They implemented these two tools as Eclipse plugins. The method used is string constraint solving.

% Fix Me Up \cite{son2013fix} Is an access-control bug-repairing tool in PHP web applications based on static analysis and transformation approach. It uses an Access Control Template (ACT) to find faulty access control logic that some or all access check statements and fix those bugs by inserting missing statements.

% According to our literature survey, most of the existing APR tools focus on C, Java, JavaScript, and Python languages. Table~\ref{tab:list-of-apr-tools} included a list of APR tools categorization with languages. PHPQuickFix, and PHPRepair \cite{samimi2012automated} are HTML error-repairing tools for PHP applications. Fix Me Up \cite{son2013fix} is an access control bug-repairing tool for PHP applications. 

The existing advanced APR tools use learning-based methods that involve training machine learning models with a large corpus of code and natural language descriptions. These methods can generate semantically meaningful patches. However, most of the existing APR tools focus on C, Java, JavaScript, and Python languages. For example, SequenceR \cite{chen2019sequencer}, RewardRepair \cite{ye2022neural}, and CURE \cite{jiang2021cure} are APR tools developed for Java, whereas BIFI \cite{yasunaga2021break}, DrRepair \cite{yasunaga2020graph} and RSRepair \cite{qi2014strength} are developed for C programs. See Table~\ref{tab:list-of-apr-tools} shows a list of APR tools categorization based on the focused programming language.

However, no learning-based APR tools are available for PHP bugs, and the existing tools cannot repair logical bugs. Samimi et al. in \cite{samimi2012automated} introduce two PHP and HTML error-repairing tools for PHP applications. The first tool, PHPQuickFix, analyzes individual prints to fix basic bugs. The second tool, PHPRepair, uses a dynamic approach to handle more complex repairs. Fix Me Up \cite{son2013fix} is a tool designed to repair access-control bugs in PHP web applications. It works through static analysis and transformation, using an Access Control Template to identify flawed access control logic in access check statements. Once identified, Fix Me Up inserts missing statements to fix the bugs.

\begin{table}[!htb]
\centering
\caption{Existing APR tools categorization with languages}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{Tool}                                                                                                      & C & Java & Python & JavaScript & PHP \\ \hline
SequenceR \cite{chen2019sequencer}             &   & \checkmark &   &   &   \\ \hline
TFix \cite{berabi2021tfix}                  &   &   &   & \checkmark &   \\ \hline
Break-It-Fix-It \cite{yasunaga2021break}       & \checkmark &   & \checkmark &   &   \\ \hline
DrRepair \cite{yasunaga2020graph}              & \checkmark &   &   &   &   \\ \hline
RSRepair \cite{qi2014strength}              & \checkmark &   &   &   &   \\ \hline
RewardRepair \cite{ye2022neural}          &   & \checkmark &   &   &   \\ \hline
CURE  \cite{jiang2021cure}                 &   & \checkmark &   &   &   \\ \hline
% \begin{tabular}[c]{@{}l@{}}Towards JavaScript \\ program repair with \\ Generative Pre-trained \\ Transformer (GPT-2) \cite{lajko2022towards} \end{tabular} &   &      &        & \checkmark          &     \\ \hline
\begin{tabular}[c]{@{}l@{}}PHPQuickFix, \\ PHPRepair \cite{samimi2012automated} \end{tabular} &   &   &   &   & \checkmark \\ \hline
Fix Me Up \cite{son2013fix}             &   &   &   &   & \checkmark \\ \hline
\end{tabular}
\label{tab:list-of-apr-tools}
\end{table}

% We can identify two types of learning-based methods these existing APR tools followed. These are Transformer, Recurrent Neural Networks (RNN), or Long Short-Term Memory Networks (LSTM) Based Architecture. Figure~\ref{fig:apr-tools-categorization-method} shows existing learning-based APR tools categorization according to these methods. Among those approaches, transformer-based APR tools showed better results.

% \begin{figure}[!htb]
%   \includegraphics[width=0.5\textwidth]{./figures/Learning based APR Tools Categorization.JPG}
%   \caption{Learning-based APR tools categorization}
%   \label{fig:apr-tools-categorization-method}
% \end{figure}




==> sections-old/related_v2.tex <==
\section{Related Work}

Several curated datasets are available for analyzing program bugs, focusing on Java, C, Python, and JavaScript bugs. One example is Defects4J~\cite{just2014defects4j}, a framework, and database that provides real-world Java program bugs for reproducible research in software testing. It includes 357 bugs from 5 open-source programs, each with a complete test suite that exposes the bug. It's also expandable, and new bugs can be easily added to the database once a program is set up. Additionally, Defects4J includes a framework for accessing faulty and fixed program versions, their corresponding test suites, and a user-friendly interface for research in software testing. Another useful dataset is Bugs.jar~\cite{bugsjar}, which contains 1,158 bugs and patches from 8 open-source Java projects representing eight important application categories. Finally, BEARS~\cite{madeiral2019bears} is a flexible benchmark project for automatic repair studies in Java that collects and stores bugs by identifying potential pairs of faulty and fixed program versions from open-source projects on GitHub. BEARS is publicly accessible and includes 251 reproducible bugs from 72 projects that use the Travis CI and Maven build environment

The ManyBugs and IntroClass datasets \cite{le2015manybugs} comprise 1,183 defects found in 15 C programs. These datasets help evaluate automatic repair algorithms and come with reproducibility and benchmark quality guarantees. ManyBugs contains bugs from well-known open-source projects, while IntroClass contains bugs from programming assignments done by a small group of students. The paper \cite{le2015manybugs} also presents experimental results for three repair methods: GenProg, AE, and TrpAutoRepair.

The datasets BugsJS \cite{gyimesi2019bugsjs} and FixJS \cite{csuvik2022fixjs} are collections of JavaScript bugs. BugsJS features 453 actual bugs that have been verified manually. These bugs are taken from 10 widely used server-side JavaScript programs, which collectively have 444,000 lines of code. Each bug comes with a report, test cases, and patch. BugsJS also includes a user-friendly command line interface that lets users conveniently access the faulty and fixed versions of the programs and execute the associated test cases. FixJS, on the other hand, gathers bugs from GitHub and provides information on the faulty and fixed versions of the same program. This dataset comprises over 300,000 samples and includes details on the commit, before/after states, and three source code representations.

% Recently, Julian Aron Prenner et al. in \cite{prenner_robbes_2023}  present RunBugRun, a fully executable dataset of 450,000 small buggy/fixed program pairs originally submitted to programming competition websites written in eight different programming languages, namely C, C++, Java, Python, JavaScript, Ruby, Go and PHP. All the bugs in the RunBugRun dataset come with test cases. Further, the authors evaluate the dataset with two baselines and provide some statistical information. 

Table~\ref{tab:list-of-bug-datasets} shows a list of existing bug datasets. The Table indicates that most existing datasets focus on C, Java, Python, and JavaScript bugs, and a bug dataset for PHP programs has not been introduced. 

\begin{table}[!htb]
\centering
\caption{Most popularly cited benchmarks for general purpose program repair in the literature for different programming languages}
\begin{tabular}{|l|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{Tool} & C & Java & Python & JavaScript\\ \hline
Defects4J \cite{just2014defects4j}                 &   & \checkmark    &        &   \\ \hline
QuixBugs \cite{lin2017quixbugs}                  &   & \checkmark    & \checkmark      &    \\ \hline
BugsJS \cite{gyimesi2019bugsjs}                    &   &      &        & \checkmark  \\ \hline
ManyBugs, IntroClass \cite{le2015manybugs}      & \checkmark &      &        &    \\ \hline
Bugs.jar \cite{bugsjar}                  &   & \checkmark    &        &     \\ \hline
Bears \cite{madeiral2019bears}                     &   & \checkmark    &        &     \\ \hline
FixJs  \cite{csuvik2022fixjs}  &   &      &        & \checkmark   \\ \hline
\end{tabular}

\label{tab:list-of-bug-datasets}
\end{table}

A subset of program repair tools use learning-based methods that involve training machine learning models with a large corpus of code and natural language descriptions. These methods can generate semantically meaningful patches. However, most of the existing program repair tools focus on C, Java, JavaScript, and Python programming languages. For example, SequenceR \cite{chen2019sequencer}, RewardRepair \cite{ye2022neural}, and CURE \cite{jiang2021cure} are repair tools developed for Java, whereas BIFI \cite{yasunaga2021break}, DrRepair \cite{yasunaga2020graph} and RSRepair \cite{qi2014strength} are developed for C programs. %Table~\ref{tab:list-of-apr-tools} shows a list of APR tools categorization based on the focused programming language.

However, to the best of our knowledge there is no learning-based program repair tool available for PHP bugs, and the existing tools cannot repair logical bugs for PHP. Samimi et al. in \cite{samimi2012automated} introduce two PHP and HTML error-repairing tools for PHP applications. The first tool, PHPQuickFix, analyzes individual prints to fix basic bugs. The second tool, PHPRepair, uses a dynamic approach to handle more complex repairs. FixMeUp \cite{son2013fix} is a tool designed to repair access-control bugs in PHP web applications. It works through static analysis and transformation, using an Access Control Template to identify flawed access control logic in access check statements. Once identified, FixMeUp inserts missing statements to fix the bugs.

% \begin{table}[!htb]
% \centering
% \caption{Existing APR tools categorization with languages}
% \begin{tabular}{|l|c|c|c|c|c|}
% \hline
% \multicolumn{1}{|c|}{Tool}                                                                                                      & C & Java & Python & JavaScript & PHP \\ \hline
% SequenceR \cite{chen2019sequencer}             &   & \checkmark &   &   &   \\ \hline
% TFix \cite{berabi2021tfix}                  &   &   &   & \checkmark &   \\ \hline
% Break-It-Fix-It \cite{yasunaga2021break}       & \checkmark &   & \checkmark &   &   \\ \hline
% DrRepair \cite{yasunaga2020graph}              & \checkmark &   &   &   &   \\ \hline
% RSRepair \cite{qi2014strength}              & \checkmark &   &   &   &   \\ \hline
% RewardRepair \cite{ye2022neural}          &   & \checkmark &   &   &   \\ \hline
% CURE  \cite{jiang2021cure}                 &   & \checkmark &   &   &   \\ \hline
% % \begin{tabular}[c]{@{}l@{}}Towards JavaScript \\ program repair with \\ Generative Pre-trained \\ Transformer (GPT-2) \cite{lajko2022towards} \end{tabular} &   &      &        & \checkmark          &     \\ \hline
% \begin{tabular}[c]{@{}l@{}}PHPQuickFix, \\ PHPRepair \cite{samimi2012automated} \end{tabular} &   &   &   &   & \checkmark \\ \hline
% Fix Me Up \cite{son2013fix}             &   &   &   &   & \checkmark \\ \hline
% \end{tabular}
% \label{tab:list-of-apr-tools}
% \end{table}



==> sections-old/results.tex <==
\section{Results}

\subsection{Results of Large Language Models}

As mentioned earlier, we used two query types to evaluate LLMs. Each of those query types results is as follows.

\input{tables/table-llm-response}

\subsubsection{Query Type I}

In query type I, we input the buggy context and ask to fix the bug without specifying the buggy lines. In Table~\ref{tab:llm-test-results} has the results of each attempt under the query type 1. As we can see, all three attempts TextDavinci model perform better than ChatGPT. Altogether we got a total of 7 patches in the TextDavinci model and a total of 5 patches in the ChatGPT that passed all the test cases. So, the TextDavinci model performs better for the query type I (without specifying buggy lines) bug-fixing task.


\subsubsection{Results of the Query Type II}\

% In Query Type II, we specify the buggy lines in the input prompt and ask to fix the buggy lines. We analyze the model's response according to whether it was a "Giving Patch" or "Not Giving Patch." For some bugs, the model responses are like, "There is no bug in the given context." The model says there is no bug in the code. Those responses are counted under the "Not Giving Patch." The rest of the responses are counted under the "Giving Patch." Models give patches as PHP code or natural language explanation. Some responses model explain how to fix the bug without giving an exact PHP code. Those responses count under the "Natural Language." The rest of the responses are counted under the ”PHP Code.” Again we analyze how many patches could extract or not from the given PHP code patches. Table~\ref{tab:model-responses-results} included those details. Some patches include some noisy words before and after the patch. So we have to extract patches from those kinds of results. The "PHP Patch" consists of the number of patches that extract like that. The rest of the patches are counted under "PHP Patch with Noise." We did this categorization by manual investigation. 


For all 513 bugs, the TextDavinci model generates patches for almost every bug in all three rounds, but ChatGPT roughly generates patches for 62\% of the bugs as an average for three rounds. In every round, for more than 100 bugs, ChatGPT does not create patches, and for more than 70 bugs, ChatGPT generates some natural language explanations instead of patches. 

As we can see, the TextDavinci model can provide patches for almost all the bugs, but ChatGPT can't. As we identify the reason, some bugs have only line insertions. Our prompting doesn't give any buggy lines for this kind of bug. It put an empty string as the buggy lines. So ChatGPT couldn't identify the buggy lines in this kind of bug.

Our patch evaluation is done in two ways. One is we run only failing test cases on each patch. The second way is we run all related test cases on each patch. Table~\ref{tab:failing-testcase-results} includes results of the patches that passed failing test cases. Table~\ref{tab:all-related-testcase-results} contains results of the patches that passed all related test cases. Here First, Second, and Third are the three candidate patches. That columns show the number of validated patches in the corresponding patch generation round.

% \begin{table}[!htb]
% \centering
% \caption{Number of patches that can pass failing test cases}
% \begin{tabular}{|l|c|c|c|c|}
%     \hline
%     \textbf{Model} & \textbf{First} & \textbf{Second} & \textbf{Third} & \textbf{Total Unique Fixes} \\
%     \hline
%     TextDavinci & 43 & 46 & 39 & 61\\
%     \hline
%     ChatGPT & 16 & 20 & 17 & 29\\
%     \hline
%     \end{tabular}
% \begin{tablenotes}
%       \item \textbf{The abbreviations used are the following: First - First candidate patch, Second - Second candidate patch, Third - Third candidate patch}
% \end{tablenotes}
% \label{tab:failing-testcase-results}
% \end{table}

% \begin{table}[!htb]
% \centering
% \caption{Number of patches that can pass all test cases}
% \begin{tabular}{|l|c|c|c|c|}
%     \hline
%     \textbf{Model} & \textbf{First} & \textbf{Second} & \textbf{Third} & \textbf{Total Unique Fixes} \\
%     \hline
%     TextDavinci & 28 & 30 & 30 & 41\\
%     \hline
%     ChatGPT & 11 & 14 & 11 & 19\\
%     \hline
%     \end{tabular}
% \begin{tablenotes}
%       \item \textbf{The abbreviations used are the following: First - First candidate patch, Second - Second candidate patch, Third - Third candidate patch}
% \end{tablenotes}
% \label{tab:all-related-testcase-results}
% \end{table}

In all three rounds for all the criteria, TextDavinci models perform better than ChatGPT.

Table~\ref{tab:bug-fixes-line-changes} shows the patch categorization according to the number of lines included in the patches. Here we considered only patches that passed all the test cases.

\begin{table}[!htb]
\centering
\caption{Number of lines of the patch}
\begin{tabular}{|l|r|r|r|r|r|r|}
    \hline
    Model & {\begin{tabular}[c]{@{}c@{}}1 \\ Line\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}2 \\ Lines\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}3 \\ Lines\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}4 \\ Lines\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}10\\Lines\end{tabular}} & \textbf{Total} \\
    \hline
    TextDavinci & 31 & 4 & 5 & 1 & 0 & \textbf{41}\\
    \hline
    ChatGPT & 15 & 1 & 2 & 0 & 1 & \textbf{19}\\
    \hline
    \end{tabular}
\label{tab:bug-fixes-line-changes}
\end{table}

Both models are better for generating one-line patches. TextDavinci generated 31 one-line patches, but ChatGPT generated only 15 patches. ChatGPT could generate one 10-line patch, but TextDavinci couldn’t. 


Table~\ref{tab:bug-fixes-equivalence} shows how many patches are generated by two models, equal to the developer patch and semantically equal to the developer patch. Here we consider only patches that pass all the test cases. 

% \begin{table}[!htb]
% \centering
% \caption{Number of patches equals to developer patch}
% \begin{tabular}{|p{2cm}|ccc|ccc|ccc|c|c|}
% \hline
% \multirow{2}{*}{Model} & \multicolumn{3}{c|}{First}  & \multicolumn{3}{c|}{Second} & \multicolumn{3}{c|}{Third} \\ \cline{2-10}
%     & \multicolumn{1}{l|}P & \multicolumn{1}{l|}D & \multicolumn{1}{l|}S & \multicolumn{1}{l|}P & \multicolumn{1}{l|}D & \multicolumn{1}{l|}S & \multicolumn{1}{l|}P & \multicolumn{1}{l|}D & \multicolumn{1}{l|}S \\ \hline
% TextDavinci & \multicolumn{1}{c|}{28} & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{6} & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{11} & \multicolumn{1}{c|}{8} & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{12} & \multicolumn{1}{c|}{4} \\ \hline
% ChatGPT & \multicolumn{1}{c|}{11} & \multicolumn{1}{c|}{6} & \multicolumn{1}{c|}{3} & \multicolumn{1}{c|}{14} & \multicolumn{1}{c|}{7} & \multicolumn{1}{c|}{3} & \multicolumn{1}{c|}{11} & \multicolumn{1}{c|}{5} & \multicolumn{1}{c|}{2} \\ \hline
% \end{tabular}
% \begin{tablenotes}
%       \item \textbf{The abbreviations used are the following: First - First Candidate Patch, Second - Second Candidate Patch, Third - Third Candidate Patch, \\P-Plausible Patch, D-Similar to Developer Patch, S-Semantically Equivalent to Developer Patch}
% \end{tablenotes}
% \label{tab:bug-fixes-equivalence}
% \end{table}


\input{tables/table-llm-test-results}



In all three rounds for all the criteria, TextDavinci models perform better than ChatGPT.

Figure~\ref{fig:venn_digram} Venn diagram show the number of bugs fixed by both model and their intersection. According to that TextDavinci model has more unique fixes than the ChatGPT. This Venn diagram was drawn by considering all test cases' passed status.

\begin{figure}[!htb]
\centering
  \includegraphics[width=0.3\textwidth]{./figures/venn diagram.png}
  \caption{Uniquely repaired bugs by LLMs}
  \label{fig:venn_digram}
\end{figure}

Out of 513 bugs, TextDavinci was able to generate patches for 30 bugs that ChatGPT couldn’t. Also, ChatGPT generated patches for eight bugs that the TextDavinci model couldn’t generate. Both models commonly generated plausible patches (patches that passed all relevant test cases) for 11 bugs. Also, none of the models could generate plausible patches for 464 bugs in our test dataset.

Table~\ref{tab:model-patch-categorization} shows the model’s patch categorization. Here we considered only patches that passed all the test cases.

\begin{table}[!htb]
\centering
\caption{Models patch categorization}
\begin{tabular}{|l|r|r|r|}
    \hline
    Model & {\begin{tabular}[c]{@{}c@{}}Inserting \\ Statement\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}Deleting \\ Statement\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}Modifying \\ Statement\end{tabular}} \\
    \hline
    TextDavinci & 1 & 0 & 40 \\
    \hline
    ChatGPT & 0 & 0 & 19 \\
    \hline
\end{tabular}
\label{tab:model-patch-categorization}
\end{table}

TextDavinci model generated patches for 40 out of 41 bugs by modifying buggy lines, and only for one patch this model generated a new code line as a patch. But ChatGPT only generates patches by modifying buggy lines in all its plausible patches. None of the models could generate patches by deleting unnecessary lines.

\subsection{Results of Existing APR tools}

As mentioned, we ran all 513 bugs in  \bugsphp on both PHP-trained CURE and RewardRepair tools and generated 100 candidate patches from each tool. Table~\ref{tab:apr-tools-patch-results} shows the patch results of APR tools. RewardRepair can generate patches for 94 bugs to pass at least failing test cases, but CURE generates only 48 patches. RewardRepair generated 36 patches, which passed all the test cases, while CURE generated only 11 patches passing all the test cases. This shows the ability of the RewardRepair tool in PHP patch generation tasks.


\input{tables/table-apr-test-results}




Table~\ref{tab:bug-fixes-line-changes} shows the patch categorization according to the number of lines included in the patches. Here we considered only patches that passed all the test cases.

\begin{table}[!htb]
\centering
\caption{Number of lines of the patch}
\begin{tabular}{|l|r|r|r|r|}
    \hline
    Tool & {\begin{tabular}[c]{@{}c@{}}1 \\ Line\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}3 \\ Lines\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}4 \\ Lines\end{tabular}} & \textbf{Total} \\
    \hline
    CURE & 11 & 0 & 0 & \textbf{11}\\
    \hline
    RewardRepair & 29 & 5 & 2 & \textbf{36}\\
    \hline
    \end{tabular}
\label{tab:bug-fixes-line-changes}
\end{table}

Both models are better for generating one-line patches. RewardRepair generated 29 one-line patches, but CURE generated only 11 patches. RewardRepair could generate 3 and 4 lines  patches, but CURE couldn’t. 

Figure~\ref{fig:venn_digram_APR} Venn diagram show the number of bugs fixed by both APR tools and their intersection. According to that, the RewardRepair tool has more unique fixes than the CURE. This Venn diagram was drawn by considering all test cases' passed status.

\begin{figure}[!htb]
\centering
  \includegraphics[width=0.3\textwidth]{./figures/venn-diagram-APR-tools.png}
  \caption{Uniquely repaired bugs by APR tools}
  \label{fig:venn_digram_APR}
\end{figure}

Out of 513 bugs, RewardRepair was able to generate patches for 29 bugs that CURE couldn’t. Also, CURE generated patches for four bugs that the RewardRepair tool couldn’t generate. Both APR tools commonly generated plausible patches for seven bugs. Also, none of the APR tools could generate plausible patches for 473 bugs in our test dataset.

% Table~\ref{tab:model-patch-categorization} shows the APR tool's patch categorization. Here we considered only patches that passed all the test cases.

% \begin{table}[!htb]
% \centering
% \caption{APR tool patch categorization}
% \begin{tabular}{|l|r|r|r|}
%     \hline
%     Model & {\begin{tabular}[c]{@{}c@{}}Inserting \\ Statement\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}Deleting \\ Statement\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}Modifying \\ Statement\end{tabular}} \\
%     \hline
%     CURE & 1 & 1 & 9 \\
%     \hline
%     RewardRepair & 0 & 0 & 19 \\
%     \hline
% \end{tabular}
% \label{tab:model-patch-categorization}
% \end{table}

% TextDavinci model generated patches for 40 out of 41 bugs by modifying buggy lines, and only for one patch this model generated a new code line as a patch. But ChatGPT only generates patches by modifying buggy lines in all its correct patches. None of the models could generate patches by deleting unnecessary lines.

==> sections-old/results_v1.tex <==
\section{Experiment Results}
\subsection{Results of Large Language Models}

We first investigate the impact of providing a fix location in our prompt to the LLMs, with its capability to generate a successful patch. We generated two types of queries for the same bug and report the results for 3 repetitions in Table~\ref{tab:model-responses-results}. Columns ``Model'' shows the LLM model used for patch generation, while column ``Rep'' indicates the \textit{$i^{th}$} repetition. For each query type (Type-I and Type-II) we report the number of successful responses for which a candidate patch was extracted and the success rate as a percentage of total bugs. Sub columns ``CP'' and ``NP'' indicate the number of instances for which a patch was generated and not generated respectively. Sub colum ``SR'' computes the success rate for generating a patch as a percentage of the total number of prompts. 

\textit{TextDavinci} model is able to generate a candidate patch irrespective of providing a fix location in the prompt for all three rounds. However, \textit{ChatGPT} model perform better with query Type-II with a significant difference in their success rates. \textit{ChatGPT} model has an average success rate of 64\% in generating a candidate patch for query Type-I and 77\%  for query Type-II. In addition, \textit{ChatGPT} model generates an explanation in natural language instructing how to fix the bug when prompted with query Type-II. Overall, we see that the \textit{TextDavinci} model outperforms \textit{ChatGPT} model in terms of generating a candidate patch. 

\input{tables/table-llm-response}

% For query Type-I, the \textit{TextDavinci} model generates patches in all three repetitions, but ChatGPT roughly generates patches for 64\% of the bugs as an average for three rounds. As an average of more than 180 bugs, ChatGPT does not create patches. Table~\ref{tab:llm-test-results} has the results of each round under query type I. Altogether we got five unique patches in the TextDavinci model and four in the ChatGPT that passed all the test cases. So, the TextDavinci model performs better for the query type I (without specifying buggy lines) bug-fixing task.

% In query type II for all 513 bugs, the TextDavinci model generates patches for almost every bug in all three rounds, but ChatGPT roughly generates patches for 77\% of the bugs as an average for three rounds. As an average of nearly 120 bugs, ChatGPT does not create patches, and for more than 70 bugs, ChatGPT generates some natural language explanations instead of patches. 

For each successful extraction of a candidate patch, we apply the changes to the buggy program and validate the correctness using the developer test-suite. Table~\ref{tab:llm-test-results} summarize the results of the validation capturing the quality of the patches generated by LLMs. Column ``Model'' indicate the Large Language Model used to generate patches, while column ``Rep'' indicate the \textit{$i_{th}$} repetition. For each query type (Type-I and Type-II) we report the number of patches which are plausible and correct. Sub columns ``$N_V$'' indicates the number of bugs where at least one patch pass the failing test-cases, ``$N_P$'' indicates the number of bugs where at least one patch pass all test cases. We further compare plausible patches (i.e. patches passing all test cases) with the developer fix and determine if they are semantically equivalent or syntactically identical. Sub columns ``$N_E$'' indicates the number of bugs where a developer equivalent patch is found and ``$N_I$'' indicate number of bugs where an identical patch was found. 

\input{tables/table-llm-test-results-1}

Query Type-II has better performance in both models compared to Type-I as expected since we provide additional information in Type-II prompt. 
\textit{TextDavinci} model is able to generate a plausible patch for Type-II queries (i.e. passing all test cases) in \textbf{28} bugs on average, out of which at least \textbf{10} are identical to the developer fix. Meanwhile \textit{ChatGPT} model can only generate a plausible for \textbf{17} bugs on average and only \textbf{5} of them are identical to developer fix. 

% \begin{tcolorbox}[boxrule=1pt,left=1pt,right=1pt,top=1pt,bottom=1pt]
% \textbf{Finding \#1:}
% TextDavinci model is able to generate more number of plausible patches compared to ChatGPT model. Patches generated by TextDavinci is of higher quality than ChatGPT with \textbf{16} bugs on average generating patches semantically equivalent to developer fix. 
% \end{tcolorbox}

\begin{tcolorbox}[boxrule=1pt,left=1pt,right=1pt,top=1pt,bottom=1pt]
\textbf{Finding \#1:}
TextDavinci model can generate more plausible patches compared to the ChatGPT model. In addition, patches generated by TextDavinci are of higher quality than ChatGPT, with \textbf{16} bugs on average generating patches semantically equivalent to developer fixes. 
\end{tcolorbox}


Both TextDavinci and ChatGPT trained with massive data, but ChatGPT fine-tuned like a chatbot for conversations.  Since TextDavinci is trained for a diverse range of language related tasks TextDavinci performs well in patch generation as well. Even without giving a bug TextDavinci generates some patch while ChatGPT does not generate patches, We need to provide specific bug details to ChatGPT to generate a patch. Also ChatGPT try to give some natural language explanation for patch but TextDavinci always provide PHP patch cause to reduce performance of ChatGPT in APR tasks. 

\subsection{Results of Program Repair Models}
We collect the results of two state-of-the-art learning-based repair models CURE and RewardRepair and analyze its effectiveness in generating a correct patch for the 513 bugs in \bugsphp test dataset. Table~\ref{tab:apr-tools-patch-results} summarizes the results for each model. Column ``$N_C$'' indicate the number of bugs for which the repair model was able to generate a candidate patch. Columns ``$N_V$'' indicates the count of patches that pass the failing test-cases, ``$N_P$'' indicates the count of patches that pass all test cases. We further compare plausible patches (i.e. passing all test cases) with the developer fix and determine if they are semantically equivalent or syntactically identical. Columns ``$N_E$'' indicates the equivalent count and ``$N_I$'' indicate the identical count. 


\input{tables/table-apr-test-results}


\textit{RewardRepair} model can generate patches for 94 bugs which pass the least failing test cases, while \textit{CURE} can only generate such patches for 48 bugs. \textit{RewardRepair} model significantly outperforms \textit{CURE} model in all remaining aspect of generating plausible patches, developer equivalent patches and for \textbf{6} bugs generating an identical patch to the developer fix. 

\begin{tcolorbox}[boxrule=1pt,left=1pt,right=1pt,top=1pt,bottom=1pt]
\textbf{Finding \#2:}
RewardRepair model performs significantly better than CURE model in our experiments with PHP bugs trained with PHP developer fixes.
\end{tcolorbox}

The reason for have significant performance in Reward Repair than CURE. Reward Repair can generate more syntactically correct code than CURE. It means that RewardRepar can generate more compilable patches than CURE. RewardRepair author mentions this fact in their paper. Having a higher number of compilable patches can cause to have plausible patches among them.


\subsection{LLMs vs Repair Models}
In this section we perform a comparative analysis of the patches generated by LLMs and Repair Models to investigate the efficacy and limitations in each. First we check the unique number of bugs each model can fix. Figure~\ref{fig:unique-plausible} depicts the unique number of bugs each model can generate for PHP bugs in our \bugsphp dataset. In terms of plausible patches \textit{RewardRepair} model is able to generate \textbf{24} unique bugs while \textit{TextDavinci} is able to generate \textbf{19} unique bugs. Similarly \textit{CURE} model and \textit{ChatGPT} model is able to generate 3 and 5 unique bugs respectively. All four models can generate a plausible patch for one bug. 


\begin{figure}[h]
\centering
  \includegraphics[width=0.3\textwidth]{./figures/plausible-venn diagram.pdf}
  \caption{Venn diagram capturing the bugs commonly fixed by all models and the unique number of bugs each model is able to generate a plausible patch.}
  \label{fig:unique-plausible}
\end{figure}


Although generating a plausible patch is a significant performance indication provided that the test cases are in average spans from 100-1000, it does not indicate how many of such patches are correct patches. We also compare the number of bugs for which each model is able to generate a semantically equivalent patch with respect to the developer fix. Figure~\ref{fig:semantic-venn_digram} depicts the capabilities of each model in generating developer equivalent patches for the PHP bugs in our \bugsphp dataset. Accordingly, \textit{TextDavinci} model performs better with \textbf{11} bugs where a developer equivalent patch was generated while \textit{RewardRepair} is able to find the same for \textbf{8} unique bugs. In terms of high quality patches LLMs perform better compared to Repair models which has been trained specifically for the task of program repair. The reason for the significant different coulb be due to the fact LLMs have been trained with a large number developer fixes crawled from the internet compared to 500k we used in our training. However, interestingly Repair Models show comparative performance compared with LLM's although it used considerably small number of training data. 


\begin{figure}[h]
\centering
  \includegraphics[width=0.3\textwidth]{./figures/semantic-venn.pdf}
  \caption{Venn diagram capturing the bugs correctly fixed by all models and the unique number of bugs each model is able to generate a correct patch compared to developer fix.}
  \label{fig:semantic-venn_digram}
\end{figure}


\begin{tcolorbox}[boxrule=1pt,left=1pt,right=1pt,top=1pt,bottom=1pt]
\textbf{Finding \#3:}
RewardRepair model has comparative performances with TextDavinci model in generating high-quality patches for PHP bugs in our dataset.
\end{tcolorbox}


Table~\ref{tab:bug-fixes-line-changes-llms} shows the distribution of patches in each model with respect to the number of lines. Here we considered only the patches that passed all the test cases. \textit{TextDavinci} model generated 31 one-line patches, while \textit{RewardRepair} is able to generated 29 patches. Simiarly, \textit{ChatGPT} and \textit{CURE} could generate 15 and 11 single-line patches respectively. \textit{CURE} could only generate single-line patches while the rest can generate multi-line patches. \textit{TextDavinci} model performs better with respect to generating multi-line plausible patches. The ability to generate multi-line patch is more desirable in the context of program repair. 



\begin{table}[h]
\centering
\caption{Number of patches for each model in terms of complexity of the patch considering the number of line changes}
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Model}   & \multicolumn{1}{l|}{\textbf{1 line}} & \multicolumn{1}{l|}{\textbf{2 - 3 lines}} & \multicolumn{1}{l|}{\textbf{\textgreater 3 lines}} & \multicolumn{1}{l|}{\textbf{Total}} \\ \hline
TextDavinci  & 31                          & 9                                & 1                                         & 41                         \\ \hline
ChatGPT      & 15                          & 3                                & 1                                         & 19                         \\ \hline
CURE         & 11                          & 0                                & 0                                         & 11                         \\ \hline
RewardRepair & 29                          & 5                                & 2                                         & 36                         \\ \hline
\end{tabular}
\label{tab:bug-fixes-line-changes-llms}
\end{table}


We further investigate the complexities of the patches generated by each model for the bugs in our dataset \bugsphp. We list the unique patches generated by each tool which passes all test cases provided in the developer test suite. Listing~\ref{lst:textdavinci-example} and Listing~\ref{lst:rewardrepair-example} depicts the quality of two patches generated by \textit{TextDavinci} and \textit{RewardRepair} models respectively. Both patches are semantically equivalent to the developer patch and are non-trivial patches that fixes a logical error in PHP application. 


\begin{figure}[h]
\begin{subfigure}[t]{0.47\textwidth}
\begin{lstlisting}[numbers=none, frame=single, basicstyle=\scriptsize\ttfamily, language=PHP,escapechar=|]
-- return in_array($name, self::UNIQUE_HEADERS, true);
++ return in_array(strtolower($name), 
++ array_map('strtolower', self::UNIQUE_HEADERS), true);
\end{lstlisting}

\caption{model generated patch}
\label{lst:textdavinci-patch}
\end{subfigure}

\vspace{0.1in}

\begin{subfigure}[t]{0.47\textwidth}
\centering
\begin{lstlisting}[numbers=none, frame=single, basicstyle=\scriptsize\ttfamily, language=PHP,escapechar=|]
-- return in_array($name, self::UNIQUE_HEADERS, true);
++ return \in_array(strtolower($name), 
++ self::UNIQUE_HEADERS, true);

\end{lstlisting}
\caption{developer fix}
\label{lst:dev-fix-1}
\end{subfigure}

\caption{An example bug uniquely fixed by \textit{TextDavinci} model showing the developer fix and model generated fix}
\label{lst:textdavinci-example}
\vspace*{-0.2in}
\end{figure}




% \begin{figure}[h]
% \begin{subfigure}[t]{0.47\textwidth}
% \begin{lstlisting}[numbers=none, frame=single, basicstyle=\scriptsize\ttfamily, language=PHP,escapechar=|]
% -- if (null !== $value && $this !== $value && 
% --     !is_scalar($value)) {
% ++ if (null !== $value && $this !== $value &&
% ++     !is_scalar($value) && 
% ++     !$value instanceof Stringable) {
% \end{lstlisting}

% \caption{model generated patch}
% \label{lst:chatgpt-patch}
% \end{subfigure}

% \vspace{0.1in}

% \begin{subfigure}[t]{0.47\textwidth}
% \centering
% \begin{lstlisting}[numbers=none, frame=single, basicstyle=\scriptsize\ttfamily, language=PHP,escapechar=|]
% -- if (null !== $value && $this !== $value && 
% --     !is_scalar($value)) {
% ++ if (null !== $value && $this !== $value &&
% ++     !is_scalar($value) && 
% ++     !$value instanceof Stringable) {

% \end{lstlisting}
% \caption{developer fix}
% \label{lst:dev-fix-2}
% \end{subfigure}

% \caption{An example bug uniquely fixed by \textit{ChatGPT} model showing the developer fix and model generated fix}
% \vspace*{-0.2in}
% \end{figure}




\begin{figure}[h]
\begin{subfigure}[t]{0.47\textwidth}
\begin{lstlisting}[numbers=none, frame=single, basicstyle=\scriptsize\ttfamily, language=PHP,escapechar=|]
++ if  ($parsedEnv['path']!==  null)  {  
  $parsedEnv['path']  =  '/'  ===  $parsedEnv['path']?  
  null : substr($parsedEnv['path'],  1);  
++ }
\end{lstlisting}

\caption{model generated patch}
\label{lst:rewardrepair-patch}
\end{subfigure}

\vspace{0.1in}

\begin{subfigure}[t]{0.47\textwidth}
\centering
\begin{lstlisting}[numbers=none, frame=single, basicstyle=\scriptsize\ttfamily, language=PHP,escapechar=|]
++ if  (null !== $parsedEnv['path'])  {  
  $parsedEnv['path']  =  '/'  ===  $parsedEnv['path']?  
  null : substr($parsedEnv['path'],  1);  
++ }
\end{lstlisting}
\caption{developer fix}
\label{lst:dev-fix-2}
\end{subfigure}

\caption{An example bug uniquely fixed by \textit{RewardRepair} model showing the developer fix and model generated fix}
\label{lst:rewardrepair-example}
\vspace*{-0.2in}
\end{figure}


% \begin{figure}[h]
% \begin{subfigure}[t]{0.47\textwidth}
% \begin{lstlisting}[numbers=none, frame=single, basicstyle=\scriptsize\ttfamily, language=PHP,escapechar=|]
% -- if ($parent instanceof UrlRoutable && ($route->
% -- enforcesScopedBindings() || array_key_exists(
% -- $parameterName, $route->bindingFields()))) {
% ++ if( array_key_exists( static :: class , 
% ++ class_uses_recursive( $instance ) ) || array_key_exists
% ++ ( static :: class , class_uses_recursive( $instance ) ) 
% ++ ) {
% \end{lstlisting}

% \caption{model generated patch}
% \label{lst:chatgpt-patch}
% \end{subfigure}

% \vspace{0.1in}

% \begin{subfigure}[t]{0.47\textwidth}
% \centering
% \begin{lstlisting}[numbers=none, frame=single, basicstyle=\scriptsize\ttfamily, language=PHP,escapechar=|]
% ++ if  (null !== $parsedEnv['path'])  {  
%   $parsedEnv['path']  =  '/'  ===  $parsedEnv['path']?  
%   null : substr($parsedEnv['path'],  1);  
% ++ }
% \end{lstlisting}
% \caption{developer fix}
% \label{lst:dev-fix-2}
% \end{subfigure}

% \caption{An example bug uniquely fixed by \textit{CURE} model showing the developer fix and model generated fix}
% \vspace*{-0.2in}
% \end{figure}

% Listing~\ref{lst:input-promt-textdavinci} is the unique plausible patch generated by TextDavinci. Listing~\ref{lst:dev-model-patch-textdavinci} shows the corresponding developer and model's patch for that bug. Here model's patch is semantically equivalent to the developer patch. Listing~\ref{lst:input-promt-chatGPT} is the patch generated by ChatGPT. TextDavinci is also able to generate a plausible patch for this. Listing~\ref{lst:dev-model-patch-chatGPT} shows the corresponding developer and model's patch for that bug. Here model's patch is semantically equivalent to the developer patch.





% \begin{lstlisting}[numbers=none, frame=single, basicstyle=\scriptsize\ttfamily, language=PHP,caption=An example that is fixed by CURE, label={lst:input-promt-cure}]
% -- if ($parent instanceof UrlRoutable && ($route->
% -- enforcesScopedBindings() || array_key_exists(
% -- $parameterName, $route->bindingFields()))) {
% ++ if( array_key_exists( static :: class , 
% ++ class_uses_recursive( $instance ) ) || array_key_exists
% ++ ( static :: class , class_uses_recursive( $instance ) ) 
% ++ ) {
% \end{lstlisting}

% \begin{lstlisting}[numbers=none, frame=single, basicstyle=\scriptsize\ttfamily, language=PHP,escapechar=|,caption=Developer and Tools's patch of Listing~\ref{lst:input-promt-cure}, label={lst:dev-tool-patch-CURE}]
% Developer's Patch
% if ($parent instanceof UrlRoutable && ($route->enforcesScopedBindings() || $route->bindingFieldFor($parameterName) !== null)) {

% Tool's Patch
% if( array_key_exists( static :: class ,
%     class_uses_recursive( $instance ) ) || array_key_exists
%     ( static :: class , class_uses_recursive( $instance ) )
%     ) {
% \end{lstlisting}

% Listing~\ref{lst:input-promt-rewardrepair} is a unique plausible patch generated by the RewardRepair tool. Listing~\ref{lst:dev-model-patch-rewardrepair} shows the corresponding developer and tool's patch for that bug. Here tool's patch is semantically equivalent to the developer patch. Listing~\ref{lst:input-promt-cure} is the patch generated by the CURE tool. RewardRepair is also able to generate a plausible patch for this same bug. Listing~\ref{lst:dev-tool-patch-CURE} shows the corresponding developer and tool's patch for that bug. There is a significant difference between the developer and the tool's patch.









==> sections-old/training-data.tex <==
\section{Training Data Set Construction}
This section discusses the methodology of curating our dataset and analysis of our proposed benchmark \bugsphp.

We created our training dataset following similar criteria for subject selection and bug collection in bug dataset construction. In Subject selection, we used GitHub REST API\footnote{https://docs.github.com/en/rest?apiVersion=2022-11-28} to retrieve the GitHub repositories. Same way, the latest committed date greater than 2021, and sorted the list in descending order by stargazer count. then we select the first 5k repositories and remove the repositories used to bug dataset contraction.

In the bugs collection step, we collected the bug fix commits by checking \texttt{"fix"}, \texttt{"solve"}, \texttt{"bug"}, \texttt{"issue"}, \texttt{"problem"} or \texttt{"error"} keywords included in the commit message. Then we filter the bug fixes that have the number of files changes less than or equal to 3 and the number of line changes less than or equal to 50. Then we extract the changed files and label them as buggy and fixed. We collected 653,606 bugs from 4483 PHP applications. Finlay, we included a metafile that contains the commit id, repository, changed line numbers, etc for each data point.

==> tables/table-llm-response.tex <==

% \begin{table}[!htb]
% \caption{Model response breakdown}
% \begin{center}
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{Attempt} &
%   \multicolumn{1}{c|}{Model} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}GP\end{tabular}} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}E\end{tabular}} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}NGP\end{tabular}} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}NL\end{tabular}} \\ \hline
% \multirow{2}{*}{1} & {\begin{tabular}[c]{@{}c@{}}TextDavinci\end{tabular}} & 511 & 495 & 0   & 2  \\ \cline{2-6} 
%                    & ChatGPT          & 317 & 286 & 119 & 77 \\ \hline
% \multirow{2}{*}{2} & {\begin{tabular}[c]{@{}c@{}}TextDavinci\end{tabular}} & 512 & 506 & 0   & 1  \\ \cline{2-6} 
%                    & ChatGPT          & 320 & 291 & 118 & 75 \\ \hline
% \multirow{2}{*}{3} & {\begin{tabular}[c]{@{}c@{}}TextDavinci\end{tabular}} & 512 & 500 & 0   & 1  \\ \cline{2-6} 
%                    & ChatGPT          & 315 & 287 & 122 & 76 \\ \hline
% \end{tabular}
% \end{center}
% \begin{tablenotes}
%       \item \textbf{The abbreviations used are the following: GP-Giving Patch E-Extracted, NGP-Not Giving Patch, NL-Natural Language}
% \end{tablenotes}
% \label{tab:model-responses-results}
% \end{table}




% \begin{table}[!htb]
% \caption{Model response breakdown}
% \begin{center}
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% Attempt & Model & Query Type & Giving Patch & \begin{tabular}[c]{@{}c@{}}Not \\ Giving Patch\end{tabular} \\ \hline
% \multirow{4}{*}{1} & \multirow{2}{*}{TextDavinci} & 1 & 513 & 0   \\ \cline{3-5} 
%                    &                              & 2 & 513 & 0   \\ \cline{2-5} 
%                    & \multirow{2}{*}{ChatGPT}     & 1 & 336 & 177 \\ \cline{3-5} 
%                    &                              & 2 & 394 & 119 \\ \hline
% \multirow{4}{*}{2} & \multirow{2}{*}{TextDavinci} & 1 & 513 & 0   \\ \cline{3-5} 
%                    &                              & 2 & 513 & 0   \\ \cline{2-5} 
%                    & \multirow{2}{*}{ChatGPT}     & 1 & 325 & 188 \\ \cline{3-5} 
%                    &                              & 2 & 395 & 118 \\ \hline
% \multirow{4}{*}{3} & \multirow{2}{*}{TextDavinci} & 1 & 513 & 0   \\ \cline{3-5} 
%                    &                              & 2 & 513 & 0   \\ \cline{2-5} 
%                    & \multirow{2}{*}{ChatGPT}     & 1 & 325 & 188 \\ \cline{3-5} 
%                    &                              & 2 & 391 & 122 \\ \hline
% \end{tabular}
% \end{center}
% \label{tab:model-responses-results}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% \begin{table}[h]
% \caption{Model response breakdown}
% \begin{center}
% \begin{tabular}{|c|l|cc|cc|}
% \hline
% \multirow{2}{*}{Round} & \multicolumn{1}{c|}{\multirow{2}{*}{Model}} & \multicolumn{2}{c|}{Query Type I}                                                                                                          & \multicolumn{2}{c|}{Query Type II}                                                                                                         \\ \cline{3-6} 
%                        & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Giving \\ Patch\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Not Giving \\ Patch\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Giving\\  Patch\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Not Giving\\  Patch\end{tabular} \\ \hline
% \multirow{2}{*}{1}     & TextDavinci                                 & \multicolumn{1}{c|}{513}                                                     & 0                                                           & \multicolumn{1}{c|}{513}                                                     & 0                                                           \\ \cline{2-6} 
%                        & ChatGPT                                     & \multicolumn{1}{c|}{336}                                                     & 177                                                         & \multicolumn{1}{c|}{394}                                                     & 119                                                         \\ \hline
% \multirow{2}{*}{2}     & TextDavinci                                 & \multicolumn{1}{c|}{513}                                                     & 0                                                           & \multicolumn{1}{c|}{513}                                                     & 0                                                           \\ \cline{2-6} 
%                        & ChatGPT                                     & \multicolumn{1}{c|}{325}                                                     & 188                                                         & \multicolumn{1}{c|}{395}                                                     & 118                                                         \\ \hline
% \multirow{2}{*}{3}     & TextDavinci                                 & \multicolumn{1}{c|}{513}                                                     & 0                                                           & \multicolumn{1}{c|}{513}                                                     & 0                                                           \\ \cline{2-6} 
%                        & ChatGPT                                     & \multicolumn{1}{c|}{325}                                                     & 188                                                         & \multicolumn{1}{c|}{391}                                                     & 122                                                         \\ \hline
% \end{tabular}
% \end{center}
% \label{tab:model-responses-results}
% \end{table}


% \begin{table}[h]
% \caption{Model response breakdown}
% \begin{center}
% \begin{tabular}{|l|c|cc|cc|}
% \hline
% \multirow{2}{*}{Model} & \multicolumn{1}{c|}{\multirow{2}{*}{Repetition}} & \multicolumn{2}{c|}{Query Type-I}                                                                                                          & \multicolumn{2}{c|}{Query Type-II}                                                                                                         \\ \cline{3-6} 
%                        & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Candidate \\ Patch\end{tabular}} & \begin{tabular}[c]{@{}c@{}}No \\
%                        Patch\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Candidate \\ 
%                        Patch\end{tabular}} & \begin{tabular}[c]{@{}c@{}}No\\  Patch\end{tabular} \\ \hline
% \multirow{3}{*}{TextDavinci} & 1 & \multicolumn{1}{c|}{513}  & 0  & \multicolumn{1}{c|}{513} & 0   \\ \cline{2-6} 
% & 2 & \multicolumn{1}{c|}{513}  & 0  & \multicolumn{1}{c|}{513} & 0   \\ \cline{2-6} 
%  & 3   & \multicolumn{1}{c|}{513}  & 0  & \multicolumn{1}{c|}{513}  & 0   \\ \hline

% \multirow{3}{*}{ChatGPT} & 1 & \multicolumn{1}{c|}{336}  & 177 & \multicolumn{1}{c|}{394} & 119   \\ \cline{2-6} 
% & 2 & \multicolumn{1}{c|}{325}  & 188  & \multicolumn{1}{c|}{395} & 118   \\ \cline{2-6} 
%  & 3   & \multicolumn{1}{c|}{325}  & 188  & \multicolumn{1}{c|}{391}  & 122   \\ \hline
 
% \end{tabular}
% \end{center}
% \label{tab:model-responses-results}
% \end{table}


\begin{table}[!htb]
\begin{center}
\begin{tabular}{|l|c|ccc|ccc|}
\hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Rep}}} & \multicolumn{3}{c|}{\textbf{Query Type-I}}                                                                                                          & \multicolumn{3}{c|}{\textbf{Query Type-II}}                                                                                                        \\ \cline{3-8} 
                       & \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}CP\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}NP\end{tabular}} & \begin{tabular}[c]{@{}c@{}}SR\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}CP\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}NP\end{tabular}} & \begin{tabular}[c]{@{}c@{}}SR\end{tabular} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}TextDavinci\end{tabular}} & 1 & \multicolumn{1}{c|}{513}  & \multicolumn{1}{c|}{0} & 100 \% & \multicolumn{1}{c|}{513} & \multicolumn{1}{c|}{0}  & 100 \% \\ \cline{2-8} 
& 2 & \multicolumn{1}{c|}{513}  & \multicolumn{1}{c|}{0} & 100 \% & \multicolumn{1}{c|}{513} & \multicolumn{1}{c|}{0}  & 100 \% \\ \cline{2-8} 
 & 3   & \multicolumn{1}{c|}{513}  & \multicolumn{1}{c|}{0} & 100 \% & \multicolumn{1}{c|}{513}  & \multicolumn{1}{c|}{0} & 100 \%  \\ \hline

\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}ChatGPT\end{tabular}} & 1 & \multicolumn{1}{c|}{336}  & \multicolumn{1}{c|}{177} & 65.4 \% & \multicolumn{1}{c|}{394} & \multicolumn{1}{c|}{119} & 76.8 \%  \\ \cline{2-8} 
& 2 & \multicolumn{1}{c|}{325}  & \multicolumn{1}{c|}{188} & 63.3 \% & \multicolumn{1}{c|}{395} & \multicolumn{1}{c|}{118}  & 76.9 \% \\ \cline{2-8} 
 & 3   & \multicolumn{1}{c|}{325}  & \multicolumn{1}{c|}{188} & 63.3 \% & \multicolumn{1}{c|}{391}  & \multicolumn{1}{c|}{122} & 76.2 \%  \\ \hline
 
\end{tabular}
\end{center}


\begin{tablenotes}
\centering
\item {CP: number of candidate patches, NP: number of responses with no patch, SR: success rate (percentage of successful candidate patch generation)}
\end{tablenotes}
\caption{Success rate for each model for different prompts}

\label{tab:model-responses-results}
\end{table}





==> tables/table-llm-test-results-1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h!]
\centering
\resizebox{0.95\columnwidth{}}{!}{%
\begin{tabular}{|c|c|cccc|cccc|}
\hline
\multirow{2}{*}{\textbf{Model}}       & \multirow{2}{*}{\textbf{Rep}} & \multicolumn{4}{c|}{\textbf {Query Type-I}}                                                                                                                                                   & \multicolumn{4}{c|}{\textbf {Query Type-II} }                                                                                                                                                                      \\ \cline{3-10} 
                             &                        & \multicolumn{1}{c|}{$N_V$} & \multicolumn{1}{c|}{$N_P$} & \multicolumn{1}{c|}{$N_E$} & $N_I$ & \multicolumn{1}{c|}{$N_V$} & \multicolumn{1}{c|}{$N_P$} & \multicolumn{1}{c|}{$N_E$} & \multicolumn{1}{l|}{$N_I$} \\ \hline
\multirow{3}{*}{TextDavinci} & 1                      & \multicolumn{1}{c|}{4}                  & \multicolumn{1}{c|}{3}              & \multicolumn{1}{c|}{3}                                                                  & 1         & \multicolumn{1}{c|}{43}                 & \multicolumn{1}{c|}{28}             & \multicolumn{1}{c|}{16}                                                                 & 10                             \\ \cline{2-10} 
                             & 2                      & \multicolumn{1}{c|}{7}                  & \multicolumn{1}{c|}{5}              & \multicolumn{1}{c|}{2}                                                                  & 1         & \multicolumn{1}{c|}{46}                 & \multicolumn{1}{c|}{30}             & \multicolumn{1}{c|}{19}                                                                 & 11                             \\ \cline{2-10} 
                             & 3                      & \multicolumn{1}{c|}{3}                  & \multicolumn{1}{c|}{2}              & \multicolumn{1}{c|}{1}                                                                  & 0         & \multicolumn{1}{c|}{39}                 & \multicolumn{1}{c|}{30}             & \multicolumn{1}{c|}{16}                                                                 & 12                             \\ \hline
\multirow{3}{*}{ChatGPT}     & 1                      & \multicolumn{1}{c|}{3}                  & \multicolumn{1}{c|}{3}              & \multicolumn{1}{c|}{0}                                                                  & 0         & \multicolumn{1}{c|}{16}                 & \multicolumn{1}{c|}{11}             & \multicolumn{1}{c|}{9}                                                                  & 6                              \\ \cline{2-10} 
                             & 2                      & \multicolumn{1}{c|}{2}                  & \multicolumn{1}{c|}{1}              & \multicolumn{1}{c|}{1}                                                                  & 1         & \multicolumn{1}{c|}{20}                 & \multicolumn{1}{c|}{14}             & \multicolumn{1}{c|}{10}                                                                 & 9                              \\ \cline{2-10} 
                             & 3                      & \multicolumn{1}{c|}{0}                  & \multicolumn{1}{c|}{0}              & \multicolumn{1}{c|}{0}                                                                  & 0         & \multicolumn{1}{c|}{17}                 & \multicolumn{1}{c|}{11}             & \multicolumn{1}{c|}{7}                                                                  & 5                              \\ \hline
\end{tabular}
%
}
\begin{tablenotes}
\item {$N_V$: \# instances at least one patch pass failing test cases, $N_P$: \# instances at least one patch pass all test cases, $N_E$: \# instances a semantically equivalent patch is found, $N_I$: \# instances a identical patch is found}

\end{tablenotes}
\caption{Quality of the patches generated by each model}
\label{tab:llm-test-results}

\end{table}

==> tables/table-llm-test-results.tex <==
% \begin{table*}[]
% \centering
% \caption{Number of patches pass test cases, semantically equals and equals to developer patch}
% \begin{tabular}{|p{2cm}|cccc|cccc|cc|c|c|}
% \hline
% \multirow{3}{*}{Model} & \multicolumn{4}{c|}{First}  & \multicolumn{4}{c|}{Second} & \multicolumn{4}{c|}{Third} \\ \cline{2-13}
%     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Failing \\ test \\ cases\end{tabular}}  
%     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}All \\ test \\ cases\end{tabular}}
%     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Semantically \\ equivalent\end{tabular}}
%     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Identical\end{tabular}}
%     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Failing \\ test \\ cases\end{tabular}}
%     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}All \\ test \\ cases\end{tabular}}
%     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Semantically \\ equivalent\end{tabular}}
%     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Identical\end{tabular}}
%     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Failing \\ test \\ cases\end{tabular}}
%     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}All \\ test \\ cases\end{tabular}}
%     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Semantically \\ equivalent\end{tabular}}
%     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Identical\end{tabular}}
%     \\ \hline
% TextDavinci & \multicolumn{1}{c|}{43} & \multicolumn{1}{c|}{28} & \multicolumn{1}{c|}{16} & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{46} & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{19} & \multicolumn{1}{c|}{11} & \multicolumn{1}{c|}{39}  & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{16} & \multicolumn{1}{c|}{12} \\ \hline
% ChatGPT & \multicolumn{1}{c|}{16} & \multicolumn{1}{c|}{11} & \multicolumn{1}{c|}{9} & \multicolumn{1}{c|}{6} & \multicolumn{1}{c|}{20} & \multicolumn{1}{c|}{14} & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{7} & \multicolumn{1}{c|}{17}  & \multicolumn{1}{c|}{11} & \multicolumn{1}{c|}{7} & \multicolumn{1}{c|}{5} \\ \hline
% \end{tabular}
% \label{tab:llm-test-results}
% \end{table*}






\begin{table*}[]
\centering
\caption{Overall result of the LLM evaluations}
\begin{tabular}{|c|c|cccc|cccc|cccc|}
\hline
\multirow{2}{*}{Model} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Query \\ Type\end{tabular}} &
  \multicolumn{4}{c|}{First Round} &
  \multicolumn{4}{c|}{Second Round} &
  \multicolumn{4}{c|}{Third Round}\\ \cline{3-14} 
 &
   &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Failing \\ test \\ cases\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}All \\ test \\ cases\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Semanti-\\ cally \\ equivalent\end{tabular}} &
  {\begin{tabular}[c]{@{}c@{}}Identical\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Failing \\ test \\ cases\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}All \\ test \\ cases\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Semanti-\\ cally \\ equivalent\end{tabular}} &
  {\begin{tabular}[c]{@{}c@{}}Identical\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Failing \\ test \\ cases\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}All \\ test \\ cases\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Semanti-\\ cally \\ equivalent\end{tabular}} &
  {\begin{tabular}[c]{@{}c@{}}Identical\end{tabular}} \\ \hline
\multirow{2}{*}{TextDavinci} &
  1 &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  1 &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{5} &
  \multicolumn{1}{c|}{2} &
  1 &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{2} &
  \multicolumn{1}{c|}{1} &
  0 \\ \cline{2-14} 
 &
  2 &
  \multicolumn{1}{c|}{43} &
  \multicolumn{1}{c|}{28} &
  \multicolumn{1}{c|}{16} &
  10 &
  \multicolumn{1}{c|}{46} &
  \multicolumn{1}{c|}{30} &
  \multicolumn{1}{c|}{19} &
  11 &
  \multicolumn{1}{c|}{39} &
  \multicolumn{1}{c|}{30} &
  \multicolumn{1}{c|}{16} &
  12 \\ \hline
\multirow{2}{*}{ChatGPT} &
  1 &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{0} &
  0 &
  \multicolumn{1}{c|}{2} &
  \multicolumn{1}{c|}{1} &
  \multicolumn{1}{c|}{1} &
  1 &
  \multicolumn{1}{c|}{0} &
  \multicolumn{1}{c|}{0} &
  \multicolumn{1}{c|}{0} &
  0 \\ \cline{2-14} 
 &
  2 &
  \multicolumn{1}{c|}{16} &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{9} &
  6 &
  \multicolumn{1}{c|}{20} &
  \multicolumn{1}{c|}{14} &
  \multicolumn{1}{c|}{10} &
  9 &
  \multicolumn{1}{c|}{17} &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{7} &
  5 \\ \hline
\end{tabular}
\label{tab:llm-test-results-1}
\end{table*}

==> tables/table-subjects-old.tex <==

\begin{table*}[t]
\centering
\caption{Subjects included in BugsPHP}
\begin{tabular}{|ll|llll|l|lll|l|}
\hline
\multicolumn{2}{|c|}{Program}                                                                                                  & \multicolumn{4}{c|}{Stats}                                                                        & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Tests \\ Cases\end{tabular}} & \multicolumn{3}{c|}{Code Coverage (\%)}                                                                                                                                                                       & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Final \\ Number \\ Of Bugs\end{tabular}}} \\ \cline{1-6} \cline{8-10}
\multicolumn{1}{|l|}{Name}                  & Description                                                                      & \multicolumn{1}{l|}{LOC(PHP)} & \multicolumn{1}{l|}{Stars} & \multicolumn{1}{l|}{Commits} & Forks &                                                                         & \multicolumn{1}{c|}{Lines} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Functions \\ and \\ Methods\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Classes \\ and \\ Traits\end{tabular}} & \multicolumn{1}{c|}{}                                                                                    \\ \hline
\multicolumn{1}{|l|}{Carbon}                 & \begin{tabular}[c]{@{}l@{}}API extension for DateTime\end{tabular}                                                                    & \multicolumn{1}{l|}{316k}     & \multicolumn{1}{l|}{16.1k} & \multicolumn{1}{l|}{3434}    & 12k   & 5898                                                                    & \multicolumn{1}{l|}{99.98} & \multicolumn{1}{l|}{99.75}                                                               & 98.25                                                                                 & 11                                                                                                       \\ \hline
\multicolumn{1}{|l|}{easywechat}            & \begin{tabular}[c]{@{}l@{}}Interface for integrating WeChat's\\ official API into PHP applications\end{tabular}                                                                     & \multicolumn{1}{l|}{14k}      & \multicolumn{1}{l|}{10k} & \multicolumn{1}{l|}{2179}    & 24k   & 178                                                                     & \multicolumn{1}{l|}{56.02} & \multicolumn{1}{l|}{50}                                                                  & 20.25                                                                                 & 9                                                                                                        \\ \hline
\multicolumn{1}{|l|}{symfony}               & Application framework                                                            & \multicolumn{1}{l|}{1579k}    & \multicolumn{1}{l|}{28.2k} & \multicolumn{1}{l|}{63973}   & 90k   & 41083                                                                   & \multicolumn{1}{l|}{80.66} & \multicolumn{1}{l|}{65.67}                                                               & 36.09                                                                                 & 188                                                                                                      \\ \hline
\multicolumn{1}{|l|}{PHP-Parser}            & \begin{tabular}[c]{@{}l@{}}Static code analysis and\\ manipulation \end{tabular}                                                                      & \multicolumn{1}{l|}{30k}      & \multicolumn{1}{l|}{16.1k} & \multicolumn{1}{l|}{1426}    & 914   & 1691                                                                    & \multicolumn{1}{l|}{92.69} & \multicolumn{1}{l|}{91.29}                                                               & 85.9                                                                                  & 3                                                                                                        \\ \hline
\multicolumn{1}{|l|}{framework}             & \begin{tabular}[c]{@{}l@{}}Web application framework\end{tabular}             & \multicolumn{1}{l|}{355k}     & \multicolumn{1}{l|}{29.3k} & \multicolumn{1}{l|}{35451}   & 99k   & 8425                                                                    & \multicolumn{1}{l|}{74.91} & \multicolumn{1}{l|}{69.09}                                                               & 32.28                                                                                 & 94                                                                                                       \\ \hline
\multicolumn{1}{|l|}{monolog}               & PHP logging library                                                              & \multicolumn{1}{l|}{27k}      & \multicolumn{1}{l|}{20.3k} & \multicolumn{1}{l|}{2696}    & 19k   & 1139                                                                    & \multicolumn{1}{l|}{63.98} & \multicolumn{1}{l|}{52.97}                                                               & 23.85                                                                                 & 7                                                                                                        \\ \hline
\multicolumn{1}{|l|}{composer}              & \begin{tabular}[c]{@{}l@{}}PHP dependency manager\end{tabular}                & \multicolumn{1}{l|}{107k}     & \multicolumn{1}{l|}{27.6k} & \multicolumn{1}{l|}{12065}   & 65k   & 2240                                                                    & \multicolumn{1}{l|}{63.34} & \multicolumn{1}{l|}{49.35}                                                               & 14.53                                                                                 & 18                                                                                                       \\ \hline
\multicolumn{1}{|l|}{orm}                   & Object-relational mapper                                                                     & \multicolumn{1}{l|}{187k}     & \multicolumn{1}{l|}{9.6k}  & \multicolumn{1}{l|}{13124}   & 25k   & 3706                                                                    & \multicolumn{1}{l|}{84.27} & \multicolumn{1}{l|}{68.01}                                                               & 45.09                                                                                 & 15                                                                                                       \\ \hline
\multicolumn{1}{|l|}{laravel-permission}    & \begin{tabular}[c]{@{}l@{}}Manage user permissions and\\ roles in a database\end{tabular}                                                                      & \multicolumn{1}{l|}{8k}       & \multicolumn{1}{l|}{11.2k} & \multicolumn{1}{l|}{1359}    & 17k   & 432                                                                     & \multicolumn{1}{l|}{93.72} & \multicolumn{1}{l|}{80.29}                                                               & 53.85                                                                                 & 6                                                                                                        \\ \hline
\multicolumn{1}{|l|}{PhpSpreadsheet}        & \begin{tabular}[c]{@{}l@{}}Pure PHP library for reading and\\ writing spreadsheet files\end{tabular}                                                                     & \multicolumn{1}{l|}{251k}     & \multicolumn{1}{l|}{12.1k} & \multicolumn{1}{l|}{4003}    & 30k   & 14071                                                                   & \multicolumn{1}{l|}{80.01} & \multicolumn{1}{l|}{77.21}                                                               & 52.25                                                                                 & 12                                                                                                       \\ \hline
\multicolumn{1}{|l|}{magento2}              & \begin{tabular}[c]{@{}l@{}}Open-source e-commerce\\ platform\end{tabular}       & \multicolumn{1}{l|}{2854k}    & \multicolumn{1}{l|}{10.6k} & \multicolumn{1}{l|}{135360}  & 92k   & 16224                                                                   & \multicolumn{1}{l|}{46.15} & \multicolumn{1}{l|}{37.66}                                                               & 29.52                                                                                 & 23                                                                                                       \\ \hline
\multicolumn{1}{|l|}{PHP-CS-Fixer}          & PHP coding standards fixer                                                                      & \multicolumn{1}{l|}{225k}     & \multicolumn{1}{l|}{11.9k} & \multicolumn{1}{l|}{8897}    & 15k   & 31774                                                                   & \multicolumn{1}{l|}{93.97} & \multicolumn{1}{l|}{87.45}                                                               & 64.85                                                                                 & 82                                                                                                       \\ \hline
\multicolumn{1}{|l|}{cakephp}               & \begin{tabular}[c]{@{}l@{}}Open-source web application\\ framework\end{tabular} & \multicolumn{1}{l|}{358k}     & \multicolumn{1}{l|}{8.6k}  & \multicolumn{1}{l|}{44636}   & 35k   & 8322                                                                    & \multicolumn{1}{l|}{84.69} & \multicolumn{1}{l|}{73.59}                                                               & 36.92                                                                                 & 33                                                                                                       \\ \hline
\multicolumn{1}{|l|}{dbal}                  & Database abstraction layer                                                                     & \multicolumn{1}{l|}{81k}      & \multicolumn{1}{l|}{9k}  & \multicolumn{1}{l|}{10941}   & 12k   & 4122                                                                    & \multicolumn{1}{l|}{65.52} & \multicolumn{1}{l|}{55.72}                                                               & 29.28                                                                                 & 9                                                                                                        \\ \hline
\multicolumn{1}{|l|}{google-api-php-client} & \begin{tabular}[c]{@{}l@{}}PHP client library for accessing\\ Google APIs\end{tabular}                                                                      & \multicolumn{1}{l|}{11k}      & \multicolumn{1}{l|}{8.5k}  & \multicolumn{1}{l|}{1807}    & 35k   & 228                                                                     & \multicolumn{1}{l|}{66.6}  & \multicolumn{1}{l|}{55.56}                                                               & 11.76                                                                                 & 3                                                                                                        \\ \hline
\end{tabular}
\label{tab:table-subjects}
\end{table*}
